Rigidity hierarchy in random point fields: random polynomials and determinantal processes

In certain point processes, the configuration of points outside a bounded domain determines, with probability 1, certain statistical features of the points within the domain. This notion, called rigidity, was introduced in a work of Ghosh and Peres. In this paper, rigidity and the related notion of tolerance are examined systematically and point processes with rigidity of various degrees are introduced. Natural classes of point processes such as determinantal point processes, zero sets of Gaussian entire functions and perturbed lattices are examined from the point of view of rigidity, and general conditions are provided for them to exhibit specified nature of spatially rigid behaviour. In particular, we examine the rigidity of determinantal point processes in terms of their kernel, and demonstrate that a necessary condition for determinantal processes to exhibit rigidity is that their kernel must be a projection. We introduce a one parameter family of point processes which exhibit arbitrarily high levels of rigidity (depending on the choice of parameter value), answering a natural question on point processes with higher levels of rigidity (beyond the known examples of rigidity of local mass and center of mass). Our one parameter family is also related to a natural extension of the standard planar Gaussian analytic function process and their zero sets.

==> Revised manuscript/biblio.tex <==
 \begin{thebibliography}{9}

\bibitem[And]{And}
Anderson, J.W., \emph{Hyperbolic geometry}, Springer Science \& Business Media, 2006.

\bibitem[AGL]{AGL}
Adhikari, K.,  Ghosh, S. and Lebowitz, J.L., \emph{Fluctuation and Entropy in Spectrally Constrained random fields}, Communications in Mathematical Physics (2021): 1-32.

\bibitem[BBK]{bbkbook}
Baccelli, Francois and Blaszczyszyn, Bartlomiej and Karray, Mohamed, \emph{Random Measures, Point Processes, and Stochastic Geometry}, Inria, \href{https://hal.inria.fr/hal-02460214/file/PointProcesses45.pdf}{Available online}, 2020.

\bibitem[BQ]{buf-1}
Bufetov, A. I. and  Qiu, Y., \emph{Determinantal point processes associated with Hilbert spaces of holomorphic functions}, Communications in Mathematical Physics 351, no. 1 (2017): 1-44.

\bibitem[BDQ]{buf-2}
Bufetov, A.I., Dabrowski, Y.,  and Qiu, Y., \emph{Linear rigidity of stationary stochastic processes}, Ergodic Theory and Dynamical Systems 38, no. 7 (2018): 2493-2507.

\bibitem[Buf-3]{buf-3}
Bufetov, A.I., \emph{Rigidity of Determinantal Point Processes with the Airy, the Bessel and the Gamma Kernel}, Bulletin of Mathematical Sciences 6, no. 1 (2016): 163-172.

\bibitem[BQS]{BQS}
Bufetov, A. I.,  Qiu,  Y., and Shamov, A., \emph{Kernels of conditional determinantal measures and the Lyons–Peres completeness conjecture}, Journal of the European Mathematical Society 23, no. 5 (2021): 1477-1519.

\bibitem[DaV]{DV}
Daley, D. J. and Vere Jones, D. \emph{An Introduction to the Theory of Point Processes (Vols. I \& II)}, Springer, 1997.

\bibitem[DeHLM]{DHLM}
Dereudre, D., Hardy, A., Leble, T. and Maida, M. \emph{DLR equations and rigidity for the Sine-beta process}, Communications on Pure and Applied Mathematics 74, no. 1 (2021): 172-222..

\bibitem[Du]{Durrett}
Durrett, R., \emph{Probability: theory and examples}, Vol. 49. Cambridge university press, 2019.

\bibitem[DM]{DymMackean}
Dym, H. and  McKean, H. P., \emph{Gaussian processes, function theory, and the inverse spectral problem}, Probability and Mathematical Statistics, Vol. 31. Academic Press.

\bibitem[Fe]{Fe}
Feldheim, N., \emph{Zeroes of Gaussian analytic functions with translation-invariant distribution}, Israel Journal of Mathematics 195, no. 1 (2013): 317-345.

\bibitem[Ge]{Ge}
H.-O. Georgii, \emph{Canonical and grand canonical Gibbs states for continuum systems}, Communications in Mathematical Physics 48, no. 1 (1976): 31-51.

\bibitem[G-I]{G-1}
Ghosh, S., \emph{Determinantal processes and completeness of random exponentials: the critical case}, Probability Theory and Related Fields 163, no. 3-4 (2015): 643-665.

% \bibitem[G-II]{G12-2}
% S. Ghosh, \emph{ Rigidity and Tolerance in Gaussian zeroes and Ginibre eigenvalues: quantitative estimates}, http://arxiv.org/abs/1211.3506.

\bibitem[G-II]{G-2}
Ghosh, S., \emph{Palm measures and rigidity phenomena in point processes}, Electronic Communications in Probability 21 (2016).

\bibitem[Gh-III]{G-3}
Ghosh, S., \emph{Quantitative estimates for rigidity and tolerance in generalised Gaussian analytic function zeros and related processes}, in preparation.

\bibitem[GhKr]{GhK}
Ghosh, S., and Krishnapur, M., \emph{Rigidity hierarchy in random point fields: random polynomials and determinantal processes}, arXiv preprint arXiv:1510.08814 (2015).

\bibitem[GhL]{GhL}
Ghosh, S., and Lebowitz, J.L., \emph{Generalized stealthy hyperuniform processes: Maximal rigidity and the bounded holes conjecture}, Communications in Mathematical Physics 363, no. 1 (2018): 97-110.


\bibitem[GP]{GP}
Ghosh, S.  and Peres, Y.,  \emph{Rigidity and Tolerance in point processes: Gaussian zeroes and Ginibre eigenvalues}, http://arxiv.org/abs/1211.2381, Duke Mathematical Journal 166, no. 10 (2017): 1789-1858.

\bibitem[GKP]{GKP}
Ghosh,  S., Krishnapur, M. and Peres, Y., \emph{Continuum Percolation for Gaussian zeroes and Ginibre eigenvalues}, http://arxiv.org/abs/1211.2514v1.


\bibitem[Gin]{Gin}
Ginibre, J., \emph{Statistical ensembles of complex, quaternion, and real matrices}, Journal of Mathematical Physics, (1965).


\bibitem[Go]{Go}
Goldman, A., The Palm measure and the Voronoi tessellation for the Ginibre process. Ann.
Appl. Probab. 20 (2010), 1, 90–128.

\bibitem[HiShTr]{HST}
Hiraoka, Y.,  Shirai, T.  and Trinh, K.D., \emph{Limit theorems for persistence diagrams}, The Annals of Applied Probability 28, no. 5 (2018): 2740-2780.

\bibitem[HS]{HS}
Holroyd, A. E. and Soo, T., \emph{Insertion and deletion tolerance of point processes}, Electron. J. Probab. 18, (2013), no. 74.

\bibitem[HKPV]{HKPV}
Hough, J. B., Krishnapur, M., Peres, Y. and Vir\'{a}g, B., \emph{Zeros of Gaussian Analytic Functions and Determinantal Point Processes}, Providence, RI, American Mathematical Society, (2009).

% \bibitem[Kr]{Kr}
% M. Krishnapur, \emph{Zeros of Random Analytic Functions}, PhD Thesis, University of California, Berkeley [arXiv.math.PR/0607504], 2006.

\bibitem[Ka]{Ka}
Kallenberg, O.,  \emph{Random Measures}, Akademie-Verlag $\cdot$ Berlin and Academic Press, 1983.

\bibitem[KiNi]{KiNi}
Kiro, A., and Nishry, A., \emph{Rigidity for zero sets of Gaussian entire functions}, Electronic Communications in Probability 24 (2019).

\bibitem[Lob]{Lob}
Lobachevskii, N.I., \emph{Pangeometry}, Vol. 4. European Mathematical Society, 2010.

\bibitem[Ly-I]{Ly}
Lyons, R.,  \emph{Determinantal Probability Measures}, Publ. Math. Inst. Hautes Etudes Sci., 98, 167-212, 2003.

\bibitem[Ly-II]{Lyons-ICM}
Lyons, R., \emph{Determinantal probability: basic properties and conjectures}, Proc. International Congress of Mathematicians 2014, Seoul, Korea, vol. IV, 137--161.


\bibitem[LySt]{LySt}
Lyons, R. and Steif, J.,  \emph{Stationary determinantal processes: Phase multiplicity, Bernoullicity, entropy, and domination}, Duke Math. J., Volume 120, Number 3 (2003), 515--575.

\bibitem[NS-I]{NS}
Nazarov, F. and Sodin, M., \emph{Random Complex Zeroes and Random Nodal Lines}, Proceedings of the International Congress of Mathematicians, Vol. III, 1450--1484, 2010.

\bibitem[NS-II]{NS1}
Nazarov, F. and Sodin, M., \emph{Fluctuations in Random Complex Zeroes: Asymptotic Normality Revisited}, Int. Math. Res. Not., Vol. 2011, No. 24, 5720--5759, 2011.

\bibitem[NSV]{NSV}
Nazarov, F., Sodin, M. and  Volberg, A., \emph{Transportation to random zeroes by the gradient flow. Geometric and Functional Analysis}, Vol 17-3, 887--935, 2007.

\bibitem[Os]{Os}
Osada, H.,  \emph{Interacting Brownian motions in infinite dimensions with logarithmic interaction potentials}, Annals of Probability, Vol.41, 2013.

\bibitem[OsSh]{OsSh}
Osada,  H. and Shirai, T., \emph{Absolute continuity and singularity of Palm measures of the Ginibre point process}, Probability Theory and Related Fields 165, no. 3 (2016): 725-770.

\bibitem[PS]{PS}
Peres, Y.  and Sly, A., \emph{Rigidity and tolerance for perturbed lattices}, arXiv preprint arXiv:1409.4490

\bibitem[Qi]{Qi}
Qiu, Y. \emph{Rigid stationary determinantal processes in non-Archimedean fields}, Bernoulli 25, no. 1 (2019): 75-88.

\bibitem[ST1]{ST1}
Sodin, M. and Tsirelson,  B., \emph{Random complex zeroes. I. Asymptotic normality}, Israel J. Math. {\bf 144} (2004), 125-149.

\bibitem[Sosh]{soshnikov}
Soshnikov, A., \emph{Determinantal random point fields},  Uspekhi Mat. Nauk {\bf 55}, (2000), no. 5(335), 107--160; translation in
Russian Math. Surveys {\bf 55} (2000), no. 5, 923-975

\bibitem[ShTa]{shiraitakahashi}
Shirai, T. and Takahashi, Y., \emph{Random point fields associated with certain Fredholm determinants I: fermion, Poisson and boson point processes}, Journal of Functional Analysis
 {\bf 205}, Issue 2, (2003), 414--463

\bibitem[Ter]{Terras}
Terras, A., \emph{Harmonic analysis on symmetric spaces -- Euclidean space, the sphere, and the Poincare upper half-plane}, Springer Science \& Business Media, 2013.

\bibitem[Tri]{Tripathi}
Tripathi, R.,  \emph{Determinantal Processes and Stochastic Domination}, arXiv preprint arXiv:2009.09141 (2020).


\end{thebibliography}


==> Revised manuscript/hierarchy.tex <==
 \section{Rigidity of $\a$-GAFs: Proof of Theorem~\ref{hierig}}
 Let $\fa$ be the $\a$-Gaussian analytic function (abbreviated as $\a$-GAF) defined by \[ \fa(z)= \sum_{j=0}^{\infty} \frac{\xi_j}{\jh} z^j. \] In this section, $\ze_{\a}$ will denote the point process of zeroes of $\fa$. Our goal  is to establish that  $\ze_\a$ exhibits rigidity of the first $k_{\a}$ moments in any bounded domain where $\frac{1}{k_{\a}}<\a \le \frac{1}{k_{\a}-1}$. We formulate this assertion in the form of the following Lemma.
 
 \begin{lemma}
\label{rigidity}
 Let $D\subset \C$ be a bounded open set, and let $\mathcal{S}_{D^c}$ denote the space of locally finite point configurations on $D^c$. For each $0 \le k \le \lfloor 1/\a \rfloor$,  there is a map $S_k : \mathcal{S}_{D^c} \to \C$ such that the moment $\sum_{z \in \ze_\a \cap D} z^k = S_k(\ze_\a \cap D^c)$ a.s.
 \end{lemma}

Observe that Lemma \ref{rigidity} will imply Theorem \ref{hierig}, so henceforth we focus on proving Lemma \ref{rigidity}.

% In section~\ref{sec:rigiditygaf} we prove the desired degree of rigidity by  estimating the variance of certain linear statistics of $\ze_{\a}$. In section~\ref{sec:tolerancegaf} the tolerance behaviour is discussed. Theorem \ref{hierig} follows from Theorems \ref{rigidity} and \ref{tolerance}.

% \subsection{Rigidity of $\a$-GAF: variance of linear statistics}\label{sec:rigiditygaf}
As in nearly all proofs of rigidity, we would be interested in proving upper bounds on the variance of appropriate linear statistics of the point process of zeroes. We formulate this in the form of a lemma on the variance growth of linear statistics.

\begin{lemma} \label{lem:varlinstat}
Let $\ph$ be a $C_c^{\infty}$ function on $\C$ such that \begin{inparaenum}[(a)] \item $|\Delta \ph|$ is radial and \item $\Delta \ph$ vanishes in a neighbourhood of the origin. \end{inparaenum}
Let $L>0$, and define $\ph_L(z)=\ph(z/L)$. Then we have 
\[\var\l(\int \ph_L \ d\ze_\a\r) \le C_{\ph,\a} \int_0^{\infty} \!\!\! \int_0^{\infty} |\L \ph(r) \L \ph(s) | \exp(-\a L^{\frac{2}{\a}}(r^{\frac{1}{\a}}-s^{\frac{1}{\a}})^2)L^{-\frac{1}{\a}}(rs)^{1-\frac{1}{2\a}}dr ds. \] 
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:varlinstat}]
 The random analytic function $\fa$ is a complex Gaussian field on $\C$ whose covariance kernel of which is given by
 \begin{equation} \label{eq:series_exp}
 K_{\a}(z,w):=\E[\fa(z)\overline{\fa(w)}]=\sum_{j=0}^{\infty} \frac{(z\ol{w})^j}{\ja}.
 \end{equation}
 The normalized random function $\hat{\fa}(z):=\fa(z)/\sqrt{K_{\a}(z,z)}$ has covariance
 \[\t_{\a}(z,w):=\E[\hat{\fa}(z)\overline{\fa(w)}]=\frac{K_{\a}(z,w)}{\sqrt{K_{\a}(z,z)K_{\a}(w,w)}}.\]
The variance of linear statistics will be expressed in terms of  the quantity
 \begin{align*}
% \t_{\a}(z,w)&:=\frac{K(z,w)}{\sqrt{K(z,z)K(w,w)}}, \\
 \psi_{\a}(z,w)&:=\E[\log|\hat{\fa}(z)|\cdot \log|\hat{\fa}(w)|] = \sum_{j=1}^{\infty} \frac{|\t_{\a}(z,w)|^{2j}}{4 j^2}.
 \end{align*}
It may be shown (c.f. Lemma \ref{lem:variance} at the end of this section)  that
% is known (see \cite{HKPV}, combine equation (3.5.2) and Lemma~3.5.2 in chapter 3) that
\[
\var\l(\int \ph_L \ d\ze_\a\r) = \frac{1}{4 \pi^2} \int\!\!\! \int \L \ph_L(z) \L \ph_L(w) \psi_{\a}(z,w) dm(z)dm(w);
\]
Here and everywhere in the paper, we use $dm(z)$ to denote Lebesgue measure.

Since $|\t_{\a}(z,w)| \le 1$, we have the  comparison $|\t_{\a}(z,w)|^2 \le \psi_{\a}(z,w) \le 2 |\t_{\a}(z,w)|^2$ (because $\sum j^{-2}\le 2$). This implies that
\begin{align}
\var\l(\int \ph_L \ d\ze_\a \r) &\le \frac{2}{4 \pi^2}  \int\!\!\! \int |\L \ph_L(z) \L \ph_L(w)|\cdot |\t_{\a}(z,w)|^2 dm(z)dm(w) \nonumber \\
&= \frac{2}{4 \pi^2}  \int \!\!\! \int |\L \ph(z) \L \ph(w)|\cdot |\t_{\a}(Lz,Lw)|^2 dm(z)dm(w). \label{eq:bdforlinearstatvar}
 \end{align}
In the last step we made a simple change of variables.

Recall that we are considering  functions $\ph$ for which \begin{inparaenum}[(a)] \item $|\Delta \ph|$ is radial and \item $\Delta \ph$ vanishes in a neighbourhood of the origin. \end{inparaenum}    Further, recall the definition of $K_\a(z,w)$, and notice that $K_\a(z,z)$ and $\theta_\a(w,w)$ are also radial functions. Now consider integrating over the angular components of $z$ and $w$ (expressed in polar co-ordinates) on the right hand side of \eqref{eq:bdforlinearstatvar}. In other words, we write $z=re^{i \mu}$ and $w= s e^{i \nu}$, and we first perform the integration on the right hand side of \eqref{eq:bdforlinearstatvar} with respect to the variables $\mu$ and $\nu$. Due to the radial nature of the functions $\ph$ and $K_\a(z,z), K_\a(w,w)$ above, we may deduce that 
\begin{align*}
& \var\l(\int \ph_L \ d\ze_\a \r)  \\ \le & \frac{2}{4 \pi^2} 
  \int \!\!\! \int \frac{|\L \ph(r) \L \ph(s)|} {|K_{\a}(Lre^{i\mu},Lre^{i\mu})|^2 |K_{\a}(Lse^{i\nu},Lse^{i\nu})|^2} \cdot \l( \int \int |K_\a(Lre^{i\mu},Lse^{i\nu})|^2 d\mu d\nu   \r)  rdr sds. \numberthis \label{eq:angular}
\end{align*}  
We perform the integration over the angular variables $\mu,\nu$ in \eqref{eq:angular} by expanding $K_\a(Lre^{i\mu},Lse^{i\nu})$ in its series expansion \eqref{eq:series_exp}.
 
  Set \[g(t,\beta)= \sum_{k=0}^{\infty} \frac{t^{k}}{(k!)^{\beta}},\]
  and denote $a_k= \frac{t^{k}}{(k!)^{\beta}}$.  
Thus, from \eqref{eq:angular}, via integration over angular variables as above, we may arrive at
  \begin{align*}
 \var\l(\int \ph_L \ d\ze_\a \r) &\le 2  \int_0^{\infty} \!\!\! \int_0^{\infty} |\L \ph(r) \L \ph(s) | \frac{g(L^4r^2s^2,2\a)}{g(L^2r^2,\a)g(L^2s^2,\a)} rs dr ds.
 \end{align*}
 
 The ratio of two successive terms in the expansion of $g(t,\beta)$ is \[\frac{a_{k+1}}{a_k}=\frac{t}{(k+1)^{\beta}}.\] This implies that $a_k$ is maximised when $t=k^{\beta}$, in other words the maximiser is $k_* = t^{1/\beta} $ (strictly speaking $\lfloor t^{1/\beta}\rfloor$, but for ease of notation we ignore the symbol for integer part). The maximal term, via Stirling's approximation for the factorial, is \[ a_{k_*}= \exp\l(t^{1/\beta}\log t - \beta \frac{(t^{1/\beta} + \frac{1}{2}) \log t}{\beta} + \beta t^{1/\beta} \r) = t^{-\frac12}e^{\beta t^{1/\beta}} .\]

 For a positive integer $j$, we have \[a_{k_*+j}=\frac{t^{k_*+j}}{[(k_*+j)!]^{\beta}}= a_{k_*} \frac{t^j}{k_* ^{j \beta}} \prod_{i=1}^j\l( 1+ \frac{i}{k_*} \r)^{-\beta} \le a_{k_*} \prod_{i=1}^j\l( 1+ \frac{i}{k_*} \r)^{-\beta}.  \]
 Each term $(1+\frac{i}{k_{*}})^{-\beta}$ in the product is less than $1$. Further, for $i>\frac12 k_{*}$ this term is at most $(2/3)^{\beta}$. For  $1\le i\le \frac12 k_{*}$ by virtue of the inequality $e^{x/2}\le 1+x\le e^{x}$ for $0<x<\frac12$, the same term is between $e^{-\beta i/k_{*}}$ and $e^{-\beta i/2k_{*}}$. Putting all this together, we have
 \begin{align*}
  \frac{a_{k_{*}+j}}{a_{k_{*}}} \le  \l(\frac{2}{3}\r)^{j-\frac12 k_{*}} \mb{ if }j>\frac12 k_{*}, \\
e^{-\beta j^{2}/2k_{*}}  \le \frac{a_{k_{*}+j}}{a_{k_{*}}} \le e^{-\beta j^{2}/4k_{*}} \mb{ if }j\le \frac12 k_{*}.
 \end{align*}
Similarly,  $a_{k_{*}-j}=a_{k_{*}}\prod_{i=0}^{j-1}(1-\frac{i}{k_{*}})^{\beta}$ from which by analogous steps (use $e^{-2x}\le 1-x\le e^{-x}$ for $0<x<\frac12$) we get
\begin{align*}
  \frac{a_{k_{*}-j}}{a_{k_{*}}} \le  \l(\frac{1}{2}\r)^{j-\frac12 k_{*}} \mb{ if }j>\frac12 k_{*}, \\
e^{-\beta j^{2}/k_{*}}  \le \frac{a_{k_{*}+j}}{a_{k_{*}}} \le e^{-\beta j^{2}/2k_{*}} \mb{ if }j\le \frac12 k_{*}.
 \end{align*}
 Thus, for $j \ge \sqrt{k_*/c\beta}$, the quantity $a_{k_* \pm j}/a_{k_*}$ decays exponentially. The upshot of this is that $g(t,\beta)/a_{k_*}\sqrt{k_*}$ is bounded between positive quantities that depend only on $\beta$. Therefore, the ratio between the quantitites
 \begin{align*}
 \frac{g(L^4r^2s^2,2\a)}{g(L^2r^2,\a)g(L^2s^2,\a)}\end{align*}
  and
   \begin{align*}&&\frac{\l(\frac{e^{2\a(L^4r^2s^2)^{1/2\a}}}{\sqrt{L^4r^2s^2}}(L^4r^2s^2)^{1/4\a}\r)}{\l(\frac{e^{\a(L^2r^2)^{1/\a}}}{\sqrt{L^2r^2}} \cdot (L^2r^2)^{1/2\a}\frac{e^{\a(L^2s^2)^{1/\a}}}{\sqrt{L^2s^2}} \cdot (L^2s^2)^{1/2\a}\r)}  =\frac{\exp(-\a L^{2/\a}(r^{1/\a}-s^{1/\a})^2)}{L^{1/\a}r^{1/2\a}s^{1/2\a}} \end{align*}
%  \begin{align*}&&\l(\frac{e^{2\a(L^4r^2s^2)^{1/2\a}}}{\sqrt{L^4r^2s^2}}(L^4r^2s^2)^{1/4\a}\r)\l(\frac{e^{\a(L^2r^2)^{1/a}}}{\sqrt{L^2r^2}} \cdot (L^2r^2)^{1/2\a}\frac{e^{\a(L^2s^2)^{1/a}}}{\sqrt{L^2s^2}} \cdot (L^2s^2)^{1/2\a}\r)^{-1} \\ && =\exp(-\a L^{2/\a}(r^{1/\a}-s^{1/\a})^2)L^{-1/\a}r^{-1/2\a}s^{-1/2\a} \end{align*}
  is bounded between two constants $c_{\beta}$ and $C_{\beta}$.

 As a result,
 \begin{align}
 &\int_0^{\infty}\!\!\! \int_0^{\infty} |\L \ph(r) \L \ph(s) | \frac{g(L^4r^2s^2,2\a)}{g(L^2r^2,\a)g(L^2s^2,\a)} rs dr ds \label{eq:varianceboundalphagaf} \\
 &  \le C_{\beta} \int_0^{\infty} \!\!\! \int_0^{\infty} |\L \ph(r) \L \ph(s) | \exp(-\a L^{2/\a}(r^{1/\a}-s^{1/\a})^2)L^{-1/\a}r^{1-1/2\a}s^{1-1/2\a} dr ds,
\nonumber
 \end{align}
%  where the notation $\asymp$ means that ratio of the quantities on either side is bounded between universal constants.
The last integral is well defined since $\L \ph (r) \equiv 0$ for $r$ close to $0$. 

This completes the proof of Lemma \ref{lem:varlinstat}.
\end{proof}

% Recall that the bound in \eqref{eq:varianceboundalphagaf} is applicable to any $\ph$ satisfying
%\begin{enumerate}[(a)] \item $|\Delta \ph|$ is a radial function and \item $\Delta \ph$ vanishes in a neighbourhood of the origin. \end{enumerate}

We now move on to complete the proof Lemma \ref{rigidity} (and hence  the proof of Theorem \ref{hierig}).

\begin{proof}[Proof of Lemma \ref{rigidity}]
We apply the bound to  a specific family of radial functions. Given any $r_{0}>1$ and any $\eps>0$, let $\ph_{\eps}$ be a radial function such that
\begin{enumerate}
\item $\ph_{\eps}(r)=1$ for $r<2r_{0}$ and $\ph_{\eps}(r)=0$ for $r>2r_{0}e^{2/\eps}$,
\item $|\ph_\eps'(r)|\le \frac{\eps}{2r}$ and $|\ph_\eps''(r)|\le\frac{\eps}{2r^2}$ for all $r$.
\end{enumerate}

Such a function can be constructed by starting with the harmonic function $(\log|z|-\log a)/(\log b-\log a)$ for some $2r_{0}<a<b<2r_{0}e$ and  convolving it with  the indicator function of a disk $D(0,\delta)$ for a small enough $\del>0$.

Consider the function $\Phi^\eps(z)=z^k\ph_\eps(z)$. Observe that $\Phi^\eps$ satisfies the conditions (a) and (b) above. As a result,  $\Phi^\eps$ satisfies the inequality \eqref{eq:varianceboundalphagaf}. Hence we have
\begin{equation} \label{eq:varianceboundalphagaf_intermediate}
\mathrm{Var}\l( \int L^k \Phi^\eps_L d \F_\a \r) \le L^{2k - \frac{2}{\a}} \int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr + K(\Phi^\eps)L^{2k}e^{-cL^{2/\a}},
\end{equation}
where $K(\Phi^\eps)$ is a positive quantity that depends only on $\Phi^\eps$ (and is independent of $L$).
We briefly mention here as to how we obtain the above inequality. To this end, on the right hand side of \eqref{eq:varianceboundalphagaf} we carry out integration with respect to the variable $s$. This integration can be decomposed into two regimes of the variable $s$ : namely, $\{s : r^{1/\a}-s^{1/\a} \le 1  \}$ and $\{s : r^{1/\a}-s^{1/\a} > 1  \}$. The two terms on the right hand side of \eqref{eq:varianceboundalphagaf_intermediate} are obtained from these two regimes of integration respectively.


Observe that $ 2k - 2/\a \le 0 $, so $ L^{2k - \frac{2}{\a}} \le 1$.

We now claim that $ \int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr = O(\eps)$. To see this, applying Leibniz rule to compute the Laplacian $|\Delta \Phi^\eps (r)|$ is supported on the set $2r_0 \le r \le 2r_0\exp(2/\eps)$ , and is $O(\eps r^{k-2})$ on this interval. This implies that
\[\int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr \le C_1 \eps^2 \int_{2r_0}^{2r_0\exp(2/\eps)} r^{2k-4+3-\frac{2}{\a}} dr \le C_2 \eps^2 \int_{2r_0}^{2r_0\exp(2/\eps)} \frac{dr}{r} \le C_3 \eps. \]

Now, given $\delta>0$, first choose $\eps$ such that  $\int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr \le \delta/2$; based on that choose $L$ large enough such that $K(\Phi^\eps)L^{2k}e^{-cL^{2/\a}} \le \delta/2$. 
% and \eqref{twoscales-1}. Consequently, it can be seen that the function $\Psi^N:=\frac{1}{N}\sum_{j=1}^N 2^{jk}\Phi_{2^j}$ has the property $\var\l(\int \Psi^N d\ze_\a \r) \to 0$ as $N \to \infty$.
%  By Borel Cantelli Lemma, this implies that there is a subsequence $\{N_j\}$ such that $\int \Psi^N d\ze_\a - \E\l[ \int \Psi^{N_j} d\ze_\a \r] \to 0$ a.s. as $j \to \infty$.
% Clearly $2^{jk}\Phi_{2^j} \equiv z^k$ on $D$, and hence $\Psi^N \equiv z^k$ on $\D$.
This enables us to invoke Theorem 6.1 from \cite{GP} (using the function $L^k\Phi_L^\eps(z)$ as defined above; for a statement see Theorem \ref{thm:GP} in Section \ref{sec:thiswillberewritten} ) and conclude that there is a measurable function $S_k:\mathcal{S}_{D^c} \to \C$ such that $\sum_{z \in \ze_\a \cap D} z^k = S_k(\ze_\a \cap D^c)$ a.s. This completes the proof of  Lemma \ref{rigidity} (and hence the proof of Theorem \ref{hierig}).
\end{proof}

We end this section with a technical lemma that provides us with an expression for $\var\l(\int \ph_L \ d\ze_\a\r)$.

\begin{lemma} \label{lem:variance}
Let $\ph$ be a $C_c^2$ function and $L>0$. Then we have
\[
\var\l(\int \ph_L \ d\ze_\a\r) = \frac{1}{4 \pi^2}  \int\!\!\! \int \L \ph_L(z) \L \ph_L(w) \psi_{\a}(z,w) dm(z)dm(w).
\]
\end{lemma}

\begin{proof}
We consider the centered random variable 
\[ \left( \int \ph_L \ d\ze_\a \right) - \E \left[\int \ph_L \ d\ze_\a \right].  \]
We may write, using the Edelman-Kostlan formula (c.f. Eq. (2.4.8) in \cite{HKPV} Chap 2; see also Eq. (3.5.2) in \cite{HKPV} Chap. 3), that 
\begin{equation} 
\left( \int \ph_L \ d\ze_\a \right) - \E \left[\int \ph_L \ d\ze_\a \right] = \frac{1}{2\pi}\int \L \phi_L(z) \log |\hat{\fa}(z)| dm(z).
\end{equation}
Thus, 
\begin{align*} 
& \var\l(\int \ph_L \ d\ze_\a\r)  \\ 
=  & \var\l(\frac{1}{2\pi}\int \L \phi_L(z) \log |\hat{\fa}(z)| dm(z)\r) \\
= & \frac{1}{4\pi^2} \int \int \L \phi_L(z) \L \ph_L(w) \mathrm{Cov}\l( \log |\hat{\fa}(z)|, \log |\hat{\fa}(w)| \r) dm(z). \numberthis \label{eq:intermediate}
\end{align*}
We now use the following result ( Lemma~3.5.2  in \cite{HKPV}) : if $a,b$ are complex Gaussians with $\E[|a|^2]=\E[|b|^2]=1$ and $\E[a \overline{b}]=\theta$, then 
  \[    \mathrm{Cov}\l( \log |a|, \log |b| \r)   =   \sum_{m=1}^\infty \frac{|\theta|^{2m}}{4m^2}.  \] Applying this to \eqref{eq:intermediate}, we obtain the desired result.
\end{proof}

%\[\ph_{1,\eps}(r)=\begin{cases}
%                          1 & \text{ for $0\le r \le 2r_0$}, \\
%                           -\frac{\eps}{2} \log r + \frac{\eps}{2} \log 2r_0 +1  & \text{ for $2r_0 \le r \le 2r_0\exp(2/\eps)$}, \\
%                           0 & \text{ for $r \ge 2r_0\exp(2/\eps)$ }.
%                          \end{cases}
%\]

%%%Let us first to the integration with respect to $s$. It suffices to focus on $s$ such that $s^{1/\a}=r^{1/\a}\pm 100L^{-1/\a}$ (because this is essentially integration against a Gaussian distribution in $s^{1/\a}$ with standard deviation $L^{-1/\a}$). By a binomial expansion (and again using the fact that we can take $r$ to be bounded away from 0), this implies that \[s= r \pm 200 \a r^{1-1/\a} L^{-1/\a}.\] Then for this range of $s$ (setting $s=r$), the integrand roughly equals $\L \ph(r)^2 r^{2-1/\a} L^{-1/\a}$. Integrating over the interval of $s$ gives a contribution of $\a r^{1-1/\a}L^{-1/\a}$. The remaining contribution, from outside this range, can be bounded above by $K(\ph)e^{-cL^{2/\a}}$.  Thus, the integral to be estimated reduces to
%%% \begin{equation} \label{bound} CL^{-2/\a} \int_0^{\infty} (\L\ph(r))^2 r^{3-2/\a} dr +  K(\ph)e^{-cL^{2/\a}} .\end{equation}
%%% Note that this gives the correct order of the variance (in $L$) as well as the right dependence on $\ph$ for the standard planar GAF (which corresponds to $\a=1$).
%%%
%%% Observe that the above argument can be carried out as soon as the following two conditions are satisfied :
%%% \begin{itemize}
%%% \item (i) The function $| \L \ph  |$ is a radial function
%%% \item  (ii) $ \L \ph  \equiv 0$ in a neighbourhood of the origin.
%%% \end{itemize}
%%%%
%%%%  Also observe that for $\a >0$, outside a given neighbourhood $U$ of the origin, we have the inequality, $r^{2-1/2\a}  \le c(U) r^2 $. As a result, if we consider functions $\phi$ such that $\L \phi \equiv 0$ on a neighbourhood $U$ of the origin, then We have the inequallity
%%%%  \begin{equation} \label{bound} \var\l(\int \ph_L d\ze_\a\r) \le C(U)  L^{-1/\a} \int_0^{\infty} (\L\ph(r))^2  r^2 dr.
%%%%   \end{equation}
%%%%
%%%% By polarization, we conclude that for any two functions $\ph$ and $\psi$ such that $|\L \ph|$ and $|\L \psi|$ are radial functions supported outside a neighbourhood $U$ of the origin, we have
%%%% \begin{equation}
%%%% \label{covar}
%%%% \mathrm{Cov} \l(  \int \ph_L d\ze_\a , \int \psi_L d\ze_\a \r) \le C(U) L^{-1/\a} \int_0^{\infty} \Delta \ph(r) \L \psi (r) r^2 dr.
%%%% \end{equation}
%%%%  This further implies that, for $\Gamma>0$, we have
%%%%  \begin{equation}
%%%% \label{twoscales-1}
%%%% \mathrm{Cov} \l(  \int \ph_L d\ze_\a , \int \psi_{\Gamma L} d\ze_\a \r) \le C(U) L^{-1/\a} \Gamma^{-2} \int_0^{\infty} \Delta \ph(r) \L \psi (r/\Gamma) r^2 dr.
%%%% \end{equation}
%%%%  The import of the above equations is that, when $\Gamma \to \infty$ with $L$ held fixed, the quantity
%%%% $ \mathrm{Cov} \l(  \int \ph_L d\ze_\a , \int \psi_{\Gamma L} d\ze_\a \r) \to 0$.

%%%Now we are ready to prove the following theorem:
%%%\begin{theorem}
%%%\label{rigidity}
%%% Let $D\subset \C$ be a bounded open set, and let $\mathcal{S}_{D^c}$ denote the space of locally finite point configurations on $D^c$. For each $0 \le k \le \lfloor 1/\a \rfloor$,  there is a map $S_k : \mathcal{S}_{D^c} \to \C$ such that the moment $\sum_{z \in \ze_\a \cap D} z^k = S_k(\ze_\a \cap D^c)$ a.s.
%%% \end{theorem}
%%%
%%%\begin{proof}
%%%First, observe that it is enough to prove the theorem for the case of a disk $D$; let its radius be $r_0$. Fix a $0 \le k \le \lfloor 1/2\a \rfloor$. Given a small $\delta>0$, let $\eps>0$ be a small positive number whose choice would be described below. We consider a  radial function $\ph_{1,\eps}$ satisfying the following conditions:
%%%\[\ph_{1,\eps}(r)=\begin{cases}
%%%                          1 & \text{ for $0\le r \le 2r_0$}, \\
%%%                           -\frac{\eps}{2} \log r + \frac{\eps}{2} \log 2r_0 +1  & \text{ for $2r_0 \le r \le 2r_0\exp(2/\eps)$}, \\
%%%                           0 & \text{ for $r \ge 2r_0\exp(2/\eps)$ }.
%%%                          \end{cases}
%%%\]
%%%Observe that $\ph_{1,\eps}'(r)=-\eps/2r$ and $\ph_{1,\eps}''(r)=\eps/2r^2$ for $2r_0 \le r \le 2r_0\exp(2/\eps)$; these derivatives being 0 outside the said region. We then ``smooth'' the function $\ph_{1,\eps}$ at $2r_0$ and $2r_0\exp(2/\eps)$ such that the resulting function $\ph_\eps$ is $C_c^2$ and satisfies $|\ph_\eps'(r)|\le \eps/2r$ and $|\ph_\eps''(r)|\le\eps/2r^2$ for all $r$.

%%%Consider the function $\Phi^\eps(z)=z^k\ph_\eps(z)$. Observe that $\Phi^\eps$ satisfies the conditions (i) and (ii) above. As a result,  $\Phi^\eps$ satisfies the inequality \eqref{bound}. Hence we have
%%%\[\mathrm{Var}\l( \int L^k \Phi^\eps_L d \F_\a \r) \le L^{2k - \frac{2}{\a}} \int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr + K(\Phi^\eps)L^{2k}e^{-cL^{2/\a}}.\]
%%%Observe that $ 2k - 2/\a \le 0 $, so $ L^{2k - \frac{2}{\a}} \le 1$.

%%%We claim that $ \int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr = O(\eps)$. To see this, applying Leibniz rule to compute the Laplacian $|\Delta \Phi^\eps (r)|$ is supported on the set $2r_0 \le r \le 2r_0\exp(2/\eps)$ , and is $O(\eps r^{k-2})$ on this interval. This implies that
%%%\[\int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr \le C_1 \eps^2 \int_{2r_0}^{2r_0\exp(2/\eps)} r^{2k-4+3-\frac{2}{\a}} dr \le C_2 \eps^2 \int_{2r_0}^{2r_0\exp(2/\eps)} \frac{dr}{r} \le C_3 \eps. \]

%%%Now, given $\delta>0$, first choose $\eps$ such that  $\int |\Delta \Phi^\eps (r)|^2 r^{3-\frac{2}{\a}} dr \le \delta/2$; based on that choose $L$ large enough such that $K(\Phi^\eps)L^{2k}e^{-cL^{2/\a}} \le \delta/2$.
%%%% and \eqref{twoscales-1}. Consequently, it can be seen that the function $\Psi^N:=\frac{1}{N}\sum_{j=1}^N 2^{jk}\Phi_{2^j}$ has the property $\var\l(\int \Psi^N d\ze_\a \r) \to 0$ as $N \to \infty$.
%%%%  By Borel Cantelli Lemma, this implies that there is a subsequence $\{N_j\}$ such that $\int \Psi^N d\ze_\a - \E\l[ \int \Psi^{N_j} d\ze_\a \r] \to 0$ a.s. as $j \to \infty$.
%%%% Clearly $2^{jk}\Phi_{2^j} \equiv z^k$ on $D$, and hence $\Psi^N \equiv z^k$ on $\D$.
%%%This enables us to invoke Theorem 6.1 from \cite{GP} (using the function $L^k\Phi_L^\eps(z)$ as defined above) and conclude that there is a measurable function $S_k:\mathcal{S}_{D^c} \to \C$ such that $\sum_{z \in \ze_\a \cap D} z^k = S_k(\ze_\a \cap D^c)$ a.s.
%%%% , hence \[\int_D \Psi^N d\ze_\a = \sum_{z \in \ze_\a \cap D} z^k.\] But \[\int \Psi^N d\ze_\a =\int_D \Psi^N d\ze_\a + \int_{D^c} \Psi^N d\ze_\a .\] In view of this, we have a.s.
%%%% \[\sum_{z \in \ze_\a \cap D} z^k = \int_D \Psi^N d\ze_\a = \lim_{j \to \infty} \l(  \E\l[ \int \Psi^{N_j} d\ze_\a \r]  -  \int_{D^c} \Psi^{N_j} d\ze_\a \r), \] as desired.

%%% \end{proof}

%\subsection{Tolerance of $\a$-GAF zeroes}\label{sec:tolerancegaf}
%Our goal in this section is to prove:
%\begin{theorem}
% \label{tolerance}
%Let $D\subset \C$ be a bounded open set, and let $\mathcal{S}_{\D^c}$ denote the space of locally finite point configurations on $\D^c$. For each $0 \le k \le \lfloor 1/\a \rfloor=r$,  let $s_k:=\sum_{z \in \ze_\a \cap D} z^k = S_k(\ze_\a \cap D^c)$, and let $\ul{s}:=(s_1,\cdots,s_r)$. Define \[\Sigma_{s_0,\us}:\{\uz \in D^{s_0}: \sum_{j=1}^{s_0} \z_j^k=s_k, 1 \le k \le r \},\] where we write $\uz:=(\z_1,\cdots,\z_{s_0})$. Then the conditional distribution of $(\ze_\a)_\inn$ given $(\ze_\a)_\out$ is mutually absolutely conitnuous with the Lebesgue measure on $\Sigma_{s_0,\uz}$.
%\end{theorem}
%
%% It remains to show that the conditional distribution of the points inside $\D$ is mutually absolutely continuous with respect to the Lebesgue measure on the constrained submanifold with the first $r$ moments held fixed. For brevity, we refer to this phenomenon as ``tolerance''.
%Clearly, Theorem \ref{tolerance}, together with Theorem \ref{rigidity}, completes the proof of Theorem \ref{hierig}.
%
%The proof of Theorem \ref{tolerance} can be accomplished by applying Theorem 7.2 from \cite{GP}. This can be done by closely following the approach for establishing tolerance for the planar GAF as in \cite{GP}; most of the argument  either does not depend on the specific value of $\a$, or the method of proof carries over from $\a=1/2$ (which is the case dealt with in \cite{GP}) to general $\a$ with minor modifications. As such, we will not provide the details of the proof here, and refer the interested reader to the supplementary note \cite{GK} that provides the full argument for general $\a$.

% \begin{thebibliography}{9}
%  \bibitem[GP]{GP}
% S. Ghosh, Y. Peres, \emph{Rigidity and Tolerance in point processes: Gaussian zeroes and Ginibre eigenvalues}, Duke Mathematical Journal, to appear.
%
% \end{thebibliography}




% \end{document}


==> Revised manuscript/introduction.tex <==


 \section{Introduction}
 \label{introduction}
 The study of rigidity phenomena in random point sets has attracted a fair amount of attention in the recent past. To put it informally, ``rigidity'' refers to a phenomenon where, for a bounded domain $\D$ in the ambient space, the points of the set outside $\D$ determine, almost surely, certain properties of the points inside. In other words, we consider spatial conditioning in the random point set, and ``rigidity'' broadly refers to singularities appearing in the conditional distribution of the points inside $\D$ given the locations of those outside.
 
 We take this opportunity to provide a rigorous formulation of the phenomenon of ``rigidity'', on similar lines to \cite{GP}. Let us first describe the set-up in which we will work, and introduce some fundamental notions. A (simple) point process $\Pi$ is a random locally finite point configuration on some metric space $\Xi$ that is equipped with a regular Borel measure $\mu$. A point process can equivalently be looked upon as a random counting measure, with atoms corresponding to the points. For more details on point processes, we refer the reader to \cite{DV} and \cite{Ka}. The space $\S$ of locally finite point configurations on $\Xi$ is a Polish space, and a point process $\Pi$ on $\Xi$ can be thought of as a probability measure on $\S$.  Let $\D \subset \Xi$ be a bounded open set. The decomposition $\Xi=\D \cup \D^c$ induces a factorization $\S=\S_{\inn} \times \S_{\out}$, where $\S_{\inn}$ and $\S_{\out}$ are respectively the spaces of  finite point configurations on $\D$ and locally finite point configurations on $\D^c$.  This immediately leads to the natural decomposition $\Upsilon=(\Upsilon_{\inn},\Upsilon_{\out})$ for any $\Upsilon \in \S$, and  consequently a decomposition of the point process $\Pi$ as $\Pi=(\Pi_{\inn},\Pi_{\out})$. 

 We are now ready to formulate a rigorous definition of rigidity as follows. 
 \begin{definition}
 \label{defrig}
A measurable function $f_{\inn} : \S_{\inn} \rightarrow \C $ is said to be \textbf{rigid} with respect to the point process $X$ on $\S$ if there is a measurable function  $f_{\out}:\S_{\out} \rightarrow \C$ such that a.s. we have $f_{\inn}(X_{\inn})=f_{\out}(X_{\out})$.
\end{definition}
 
 Of course, the phenomenon of rigidity is the most interesting in the case of point processes that have infinitely many points. For finite processes (of a given size), the points outside a domain $\D$ will determine the number of points inside $\D$, and in the usual case of the points having a joint density, these points inside $\D$ could be in almost any configuration in $\D$. However, such simplistic behaviour cannot be expected, and indeed, is not true for point processes of infinite size. 
 
 The most common point process of infinite size, used as a model for many real world phenomena, is the Poisson point process. The most significant property of the Poisson process is the statistical independence of points in disjoint domains, and this property ensures that there is no ``rigidity'' of any sort for the Poisson process. However, for processes with non-trivial spatial correlation, the exploration of rigidity phenomena remains an interesting question. Among the most important natural examples of point processes of this kind are the bulk scaling limits of various random matrix ensembles, e.g. the sine kernel process in one dimension, or the Ginibre ensemble in two dimensions. Other significant ensembles include the zeroes of the standard planar Gaussian Analytic Function, abbreviated as the (standard planar) GAF on the complex plane, and the zeroes of the standard GAF on the hyperbolic plane. 
 
 The underlying randomness in most of these processes comes from independent Gaussian random variables, and inspite of the non-trivial spatial correlations, it would be natural to expect a fair amount of regularity or smoothness in the conditional distributions (under spatial conditioning). For example, one might expect that the conditional distribution of the points inside a given domain $\D$ would be, a.s., mutually absolutely continuous with respect to a Poisson process on $\D$. However, it turns out that in many of these processes, such anticipated regularity is not true. On the contrary, the conditional distribution of the points inside $\D$ is highlly sinngular, in the sense that the support of the conditional measure is a singular subset of the ambient domain.
  
 In \cite{GP}, the authors studied rigidity phenomena with regard to the Ginibre ensemble and the standard planar GAF zero process. The Ginibre ensemble is the weak limit of the eigenvalues of non-Hermitian (complex) Gaussian random matrices. The standard planar GAF is the Gaussian power series \[f(z)=\sum_{k=0}^\infty \frac{\xi_k}{\sqrt{k!}}z^k,\] and the GAF zero process is the point process of zeroes of this random analytic function. For more details on these ensembles, we refer the reader to \cite{HKPV}.
 
 The study of rigidity phenomena in point processes has received some attention in the recent past; we mention here some of the works relevant to our study. In \cite{G-1}, it was shown that the sine kernel process (which arises as the bulk limit of Hermitian random matrix ensembles) exhibits rigidity in the number of points in a domain. Similar results were also established for a wide range of translation invariant determinantal point processes on $\Z$ (introduced by Lyons and Steif \cite{LySt}) that correspond to function spaces characterised by vanishing Fourier transform outside a given set. In \cite{OsSh}, Osada and Shirai showed that for the Ginibre ensemble, the Palm measures with respect to different point sets are mutually absolutely continuous if the conditioning set of points have the same cardinality, and are mutually absolutely continuous otherwise. Such dichotomy is similar in spirit to, and is, in fact, closely related with the rigidity phenomena under our consideration. For more on this theme, we refer the reader to the upcoming article \cite{G-2}. 
 
 Rigidity phenomena have also been exploited to answer questions on point processes and stochastic geometry which are interesting in their own right. In \cite{G-1}, rigidity of the sine kernel process was exploited to answer a completeness question related to exponential functions coming from the point process. In \cite{GKP}, the authors used an understanding of the rigidity behaviour of the Ginibre ensemble and the standard planar GAF zero process obtained in 
 \cite{GP} in order to study continuum percolation on these models. In particular, they showed the  existence of a non-trivial critical radius for percolation, and established the uniqueness of the infinite cluster in the supercritical regime. In \cite{Os}, an understanding of  quasi-Gibbs property, which has a somewhat similar  flavour to rigidity and tolerance, was used to define an infinite particle SDE for invariant dynamics on the Ginibre process. To execute a similar programme for invariant dynamics on the standard planar GAF zero process involves new challenges involving the higher level of rigidity in GAF, and is a topic of current research.
  
 In \cite{GP}, the authors showed that in the Ginibre ensemble, the points outside any bounded open set $\D$ determine a.s. the number of points inside $\D$, and in the GAF zero process, the points outside $\D$ determine the number and the sum of the points inside. If we think of the points as a particle system, then this can be described by saying that in the Ginibre ensemble, there is local conservation of mass, while in the standard planar GAF zero process, the mass as well as the centre of mass are locally conserved. Moreover, they showed that these are the ``only'' conservation laws in these ensembles, in a natural sense. To be precise, we quote the relevant theorems from \cite{GP}.
 
 In Theorems \ref{gin-1}-\ref{gaf-2} we denote the Ginibre ensemble by $\G$ and the GAF zero ensemble by $\F$. As before, $\D$ is a bounded open set in $\C$. 

 In the case of the Ginibre ensemble, we prove that a.s.  the points outside $\D$ determine the number of points inside $\D$, and ``nothing more''. 

\begin{theorem}
 \label{gin-1}
For the Ginibre ensemble, there is a measurable function $N:\S_{\out} \to \nat$ such that a.s. \[ \mathrm{ \ Number \ of \ points \ in \ } \G_{\inn} = N(\G_{\out})\hspace{3 pt}.\]
\end{theorem}

Since a.s. the length of $\uz$ equals $N(\G_{\out})$, we can assume that each measure $\rho(\uout,\cdot)$ is supported on $\D^{N({\uout})}$.


\begin{theorem}
\label{gin-2}
For the Ginibre ensemble, $\P$-a.s. the measure $\rho({\G_{\out}},\cdot)$ and the Lebesgue measure $\el$ on $\D^{N(\G_{\out})}$ are mutually absolutely continuous.
\end{theorem}

In the case of the GAF zero process, we prove that the points outside $\D$ determine the number as well as the centre of mass (or equivalently, the sum) of the points inside $\D$, and ``nothing more''. 

\begin{theorem}
 \label{gaf-1}
For the GAF zero ensemble, \newline
\noindent
(i)There is a measurable function $N:\S_{\out} \to \nat$ such that a.s.  \[ \mathrm{ \ Number \ of \ points \ in \ } \F_{\inn} = N(\F_{\out}).\]
(ii)There is a measurable function $S:\S_{\out} \to \C$ such that a.s.  \[ \mathrm{ \ Sum \ of \ the \ points \ in \ } \F_{\inn} = S(\F_{\out}).\]
\end{theorem}

For a possible value $\uout$ of $\F_{\out}$, define the set of admissible vectors of inside points (obtained by considering all possible orderings of such inside point configurations) \[ \Sigma_{S({\uout})} := \{ \uz \in \D^{N({\uout})} : \sum_{j=1}^{N({\uout})} \z_j = S({\uout}) \}\] where $\uz=(\z_1,\cdots,\z_{N({\uout})})$.

Since a.s. the length of $\uz$ equals $N({\uout})$, we can assume that each measure $\rho(\uout,\cdot)$ gives us the distribution of a random vector in  $\D^{N({\uout})}$ supported on $\Sigma_{S({\uout})}$.

\begin{theorem}
\label{gaf-2}
For the GAF zero ensemble, $\P$-a.s. the measure $\rho(\F_{\out},\cdot)$ and the Lebesgue measure $\els$ on $\Sigma_{S(\F_{\out})}$ are mutually absolutely continuous.
\end{theorem}

Theorems \ref{gin-2} and \ref{gaf-2} lead to a natural definition of ``tolerance'' for point processes. Heuristically, this corresponds to the regularity of the spatially conditional measures, modulo local rigidity constraints. Before making a formal definition, let us recall the definition of linear statistics: 
\begin{definition}
 \label{linstat}
Let $\Pi$ be a point proces on $\Xi$ and $\ph:\Xi \to \C$ be a measurable function. Then the linear statistics $\La(\ph)[\Pi]$ of $\Pi$ is defined to be the random variable \[\La(\ph)[\Pi]:=\int_\Xi \ph(z) d[\Pi](z).\] 
\end{definition}


\begin{definition}
 \label{tolerance}
 Let $\Pi$ be a point process on a Riemannian manifold $\Xi$ with volume measure $\mu$. Let $\D \subset \Xi$ be a bounded open set, and let $\La(\Phi_0),\La(\Phi_1),\cdots,\La(\Phi_t)$ be rigid linear statistics of the point process $\Pi_\inn$ on $\D$, with $\Phi_0 \equiv 1$ and $\Phi_1,\cdots,\Phi_t:\D \rightarrow \C$ smooth functions. 
 
 For an integer $m \ge 0$  and $\us:=(s_1,\cdots,s_t) \subset \C^t$, consider the submanifold of $\D^m$ \[\Sigma_{m,\us}:=\{ \uz=(\zeta_1,\cdots,\zeta_m) \in \D^m : \La(\Phi_j)[\delta_{\uz}]=s_j; 1 \le j \le t  \},\] where $\delta_{\uz}$ is the counting measure corresponding to the point set $\{\zeta_i\}_{i=1}^m$.
 
 Then $\Pi$ is said to be tolerant subject to  $\La(\Phi_0),\La(\Phi_1),\cdots,\La(\Phi_t)$ if the conditional distribution $\l(\Pi_\inn | \Pi_\out=\o \r)$ is mutually absolutely continuous with the point process of $\La(\Phi_0)[\Pi_\inn]=N(\o)$ points sampled independently from the submanifold $\Sigma_{N(\o),\us}$ (where $s_i=\La(\Phi_i)[\Pi_\inn]=S_i(\o), 1\le i \le t$) equipped with the restriction of the volume measure $\mu^{\otimes N(\o)}$.
\end{definition}

\begin{remark}
 One can generalise the above notion of tolerance by demanding constraints on more general functionals than linear statistics. For example, for a fixed positive integer $k$, one can consider a smooth function $\Psi:\D^k \to \C$ and demand that the functional $\La^{(k)}(\Psi):=\int \int \Psi d[\Pi_\inn]^{\otimes k}$ is rigid.  
\end{remark}

Theorems \ref{gin-2} and \ref{gaf-2} can be phrased in terms tolerance as defined above. E.g., Theorem \ref{gin-2} can be rephrased by saying that for any bounded open set $\D$, the Ginibre ensemble  is tolerant subject to the number of points in $\D$.

In view of these results, it is natural to ask whether there are point processes which exhibit higher levels of rigidity, in the sense that higher moments of the points inside $\D$ are also conserved. In a technical sense, we can formulate this question as follows.
 
\begin{definition}
 \label{hie}
 We say that a point process $\Pi$ on $\C$ is rigid at level $k$ if the following conditions hold for every bounded open set $\D \subset \C$:
 \begin{itemize}
  \item The linear statistics of $\Pi_\inn$ given by $\{\La(z^{j})\}_{j=0}^{k-1}$ are rigid.
  \item $\Pi$ is tolerant subject to $\{\La(z^{j})\}_{j=0}^{k-1}$.
 \end{itemize}
\end{definition}

In terms of the last definition, we can say that the Ginibre ensemble is rigid at level 1 and the standard planar GAF zero process is rigid at level 2.
 
Of course, we would like to consider ``natural'' models of point processes exhibiting higher levels of rigidity. As in, the models should not be toy examples engineered to precisely conform to such notions of rigid behaviour. One potential source of such toy models could be lattice perturbations, with the perturbations constrained so as to obtain rigidity at the desired level. However, even to obtain ``toy'' examples seems to be rather difficult, and we are not aware of any such models.
 
 In this paper, we answer the above question by introducing a family of point processes, indexed by a parameter $\a>0$, such that for different values of $\a$  there is a different rigidity behaviour. These are also Gaussian analytic functions, albeit with different scaling behaviour of the coefficients from the standard one. In fact, we show that there is a monotonicity in the rigid behaviour with respect to the parameter $\a$: for $\frac{1}{k} < \a \le \frac{1}{k-1}$ (where $k \ge 0$ is an integer), the resulting point process is rigid at level $k$. For the special case $\a=1/2$, we recover the standard planar GAF. We call this family of Gaussian analytic functions as $\a$-GAF, which we formally define as follows:
 
 \begin{definition}
  For a real number $\a>0$, we define the $\a$-GAF \[f_\a(z)=\sum_{k=0}^\infty \frac{\xi_k}{(k!)^{\a/2}}z^k.\]
 \end{definition}

 This enables us to state
 \begin{theorem}
  \label{hierig}
  The $\a$-GAF zero process is rigid at level $k \ge 1$ whenever $\a \in (\frac{1}{k} , \frac{1}{k-1}]$. 
 \end{theorem}

%  It is natural to ask whether one can study continuum percolation on the $\a$-GAF zero processes on similar lines to \cite{GKP}. Letus mention prove existence of a (non-trivial) critical radius for continuum percolation on the $\a$-GAF zero process, and whether it is possible to establish uniqueness of the infinite cluster in the supercritical regime 
 
 Another natural question which arises with regard to rigidity phenomena is the following. In a determinantal point process (henceforth abbreviated as d.p.p.) with a kernel $K$ and a background measure $\mu$, all information about the process is contained, in principle, in the pair $(K,\mu)$. So, it is natural to ask whether it is possible to read off information about the rigidity behaviour of determinantal processes by looking at their kernel. We provide a partial answer to this question by specifying conditions on the pair $(K,\mu)$ which mandate a certain rigidity behaviour of the determinantal process.
 
 To state this result, recall that the necessary and sufficient condition (due to Machchi and Soshnikov) for the pair $(K,\mu)$ to be the kernel and background measure of a determinantal point process is that $K$ gives rise to a non-negative contraction when looked upon in the natural way as the kernel of an integral operator acting on $L^2(\mu)$. Then we have the following connection between rigidity and the kernel:
 
 \begin{theorem}
  \label{detrig}
  Let $\Pi$ be a determinantal point process with kernel $K$ and background measure $\mu$. Then $\Pi$ exhibits rigidity in the number of points in a domain only if $K$ is a projection operator on $L^2(\mu)$.
 \end{theorem}

 It is an interesting question to ask whether converse of Theorem \ref{detrig} is true. In other words, if the kernel $K$ yields a projection operator on $L^2(\mu)$, then is the resulting determinantal process rigid (in terms of the number of points in a domain). However, such a statement is not true in complete generality. A counter-example is provided by the zeroes of the hyperbolic Gaussian analytic function of intensity 1. It is a determinantal point process whose kernel is the projection on to the Bargmann spacee of $L^2$ analytic functions on the unit disk. It has been shown to be insertion and deletion tolerant in \cite{HS}; in particular, it does not exhibit rigidity of the number of points in any domain. However, this is an example where the ambient space (the hyperbolic plane) is non-Euclidean, in particular it is non-amenable. This still leaves open the question of whether a determinantal point process on a Euclidean space given by a projection kernel is necessarily rigid (in terms of the number of points), or more generally, what can be said about the rigidity  properties of such point processes. 
 
 In Section \ref{radialmeasures}, we consider determinantal point processes on $\C$ with a sesqui-holomorphic kernel $K(z,w)$ (that is holomorphic in $z$ and conjugate-holomorphic in $w$).  Further, we will assume that $\gamma$ is a radial measure with $\mu$ being the measure on the non-negative real line induced by $|Z|^2$ (where $Z  \sim \gamma$), that $\mu$ has all moments finite, and let \[c_j^{-1}= \int_0^\infty r^j d\mu(r).\] We will focus on the case where the kernel has the structure \[K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j .\] The last identity implies that $K$ is a reproducing kernel, projecting on to the subspace of $L^2(\gamma)$ gererated by the polynomials.   

 This is an interesting family of d.p.p.-s (parametrized by the measure $\gamma$), encompassing the zeroes of the hyperbolic GAF with unit intensity on one hand (where $\gamma$ is the uniform measure on the unit disk), and the Ginibre ensemble on the the other (where $\gamma$ equals the standard Gaussian measure on the complex plane). It is known that the rigidity properties of these two ensembles are very different - while the hyperbolic GAF is tolerant to insertion and deletion of points (\cite{HS}), the Ginibre ensemble exhibits rigidity at level 1. 
 
 We investiage this family of d.p.p.-s with respect to rigidity behavious. Interestingly, a rough dichotomy emerges - when $\gamma$ is compactly supported (along with some additional conditions), the d.p.p. does not exhibit rigidity, whereas, when $\gamma$ belongs to a fairly wide class of measures that have unbounded support (that includes the Gaussian and related measures), the d.p.p. is rigid at level 1. Technically, these conditions on the measures can be articulated in terms of the various moments of $\mu$.
 
 Before stating the theorems, we introduce some further notations. Let $\Gamma_j$ be the size biasing of $\mu$ of the order $j$; in other words, $\Gamma_j$ has a density which is proportional to $r^jd\mu(r)$. Let \[\mu_j:=\E[\Gamma_j]=c_j/c_{j+1},\] \[\sigma_j:=\E\l[\l(\frac{\Gamma_j}{\mu_j}-1\r)^2\r]=\l(\frac{\mu_{j+1}}{\mu_j}-1\r)\] and  \[\nu_j := \E\l[  \l(\frac{\Gamma_j}{\mu_j}-1\r)^4\r]= \l( \frac{\mu_{j+3}\mu_{j+2}\mu_{j+1}}{\mu_j} - 4 \frac{\mu_{j+2} \mu_{j+1}}{\mu_j^2} + 6 \frac{\mu_{j+1}}{\mu_j} -3 \r).\]
 
 In the setting described above, we can state the following theorems:
 \begin{theorem}
 \label{compact}
Suppose that $\sum_{j=1}^{\infty}\sigma_j < \infty$. Then the process $\mathbb{X}$ does not exhibit rigidity of numbers.
\end{theorem}
 
 and 
 
 \begin{theorem}
 \label{dpprt}
Let the measure $\mu$ be such that it satisfies the following growth conditions:
\begin{itemize}
 \item $\sum_{j=1}^{\infty}\nu_j<\infty. $
 \item $\sum_{j=1}^{k} \mu_j^4 \nu_j= o(\mu_k^4).  $
\end{itemize}
Then the determinantal point process $\mathbb{X}$ is rigid with respect to the number of points in a bounded domain. 
If, in addition, we have the measure $\gamma$ absolutely continuous w.r.t. the Lebesgue measure on $\C$, and that for some integer $a \ge 1$ 
\begin{itemize}
 \item $\sum_{j=1}^{\infty}\mu_j^{-a}<\infty$, 
\end{itemize}
then the point process  $\mathbb{X}$ is in fact rigid at level 1.
\end{theorem}

\begin{remark}
 The assumption of absolute continuity on the measure $\gamma$ is somewhat superfluous, and is there purely to invoke the definition of tolerance, which rules out arbitrary measures. However, for rigidity at level 1, one can adopt a slightly wider notion of tolerance, by demanding that the point process inside a bounded open $\D$ is mutually absolutely continuous with respect to the point process of $N(\D)$ intependent points sampled from $d\gamma^{\otimes N(\D)}$. The proof of tolerance shows that this more general notion of tolerance is also valid in the case at hand. 
\end{remark}


A key class of measures $\mu$ which satisfies the conditions in Theorem \ref{compact} is the one where we have the following asymptotic expansion for $m_j$:
\[ \mu_j=A+\frac{B}{j} + O(1/j^2) .\]
Included in this class of measures are all measures $\mu$ such that $\mu$ is compactly supported and has a positive density in a neighbourhood of the maximal end of its support, which incorporates the important case of uniform measures on disks.

An important class of measures which satisfies the criteria in Theorem \ref{dpprt} are those which exhibit the following asymptotics, for some constants $C,A,\a$: \[\mu_j:=\E[\Gamma_j]=Cj^\a\l(1+\frac{A}{j} + O(\frac{1}{j^2})\r).\]
In other words, we stipulate a power law for the means of the size biased measures $\Gamma_j$. This covers the case of all measures of the form $d\mu(r)=r^\beta e^{-r^\gamma}dr$, which includes the Ginibre ensemble. 

While Theorems \ref{compact} and \ref{dpprt} encompass the known and important examples of relevant d.p.p.-s, it would be definitely very interesting to sharpen the dichotomy presentes in these two theorems. In particular, would it be possible to extend this dichotomy and establish that it is indeed the compactness or the non-compactness of the measure $\gamma$ that determines the rigidity behaviour of the d.p.p.

An interesting point process on $\R$ for which rigidity phenomena has been considered is the case of the sine kernel process. Indeed, it has been shown in \cite{G-I} that this point process has rigidity of the number points. It turns out that this is the only rigid statistic for the sine process, in other words, the sine process is rigid of order 1. The proof of tolerance, subject to the constraint on the number of points, is on similar lines to the proof of tolerance for the Ginibre ensemble in \cite{GP} and the proof of tolerance in Theorem \ref{dpprt}. Accordingly, we will address the proof in the supplementary note \cite{}. For now, we simply record the fact as:
\begin{theorem}
 \label{sintol}
 The sine kernel process on $\R$ is rigid at level 1.
\end{theorem}


Finally, in Section \ref{lattice}, we consider the  point process obtained by Gaussian perturbations of $\Z$. For an i.i.d. perturbation of $\Z$, it can be shown that the resulting point process is rigid at level 1; for this the perturbing variable does not need to be Gaussian, finite variance is enough. This is similar to the situation for i.i.d. lattice perturbations of $\Z^2$. On the other hand, for i.i.d. perturbations in dimensions $d \ge 3$, it is known (\cite{PS}) that there is a phase transition in the variance of the perturbing Gaussian: there is a critical $\sigma_c$ such that for variance bigger than $\sigma_c^2$, the process is insertion tolerant (to be defined below), while for variance less than $\sigma_c^2$ it is rigid (at level 1). We call a point process $\X$ on a Euclidean space insertion tolerant, if, given any bounded domain $D$ and the point configuration  $ \X$ we can introduce a new point in $D$ and still remain in the support of $\X$.  In particular, this implies that there is no rigidity of numbers in $\X$.

In dimension 1, when the tails of the Gaussians become progressively heavier, the rigidity phenomena presents an interesting study. If we posit a power law growth for the variances of the perturbations, we obtain a phase transition in the rigidity behaviour of Gaussian perturbations of $\Z$ as follows:

\begin{theorem}
 \label{power}
 Consider the point process $\X$ on $\R$ which is the random point set given by $\{k+Z_k: k \in \Z, Z_k \text{ independent } N(0,\sigma_\beta(k)) \}$, where $\sigma_\beta(k) = |k|^\beta$. Then $\X$ is insertion tolerant if $\beta>1/2$, and is rigid (at level 1) if $\beta \le 1/2$.
\end{theorem}




==> Revised manuscript/introduction3.tex <==


\section{Introduction}
 \label{introduction}

\subsection{Background} \label{sec:background}
A simple point process on $\R^{d}$ is a random locally finite subset of $\R^d$. To be precise, let $\mathcal{S}$ denote the space of locally finite point sets in $\R^d$. By identifying a set with its counting measure, $\mathcal S$ becomes an open subset of $\mathcal M_p$, the space of all integer-valued locally finite Borel measures on $\R^d$. Equipped with the vague topology, $\mathcal M_p$ turns out to be a Polish space. A random variable taking values in $\mathcal M_p$ (with probability $1$)  is called a point process, and a random measure that  takes values in $\mathcal S$ (with probability $1$) is called a simple point process. A slightly more general definition is given in Section~\ref{sec:setup}.  For more detailed discussion, we refer the interested reader to Chapter~1 of \cite{bbkbook} or the extensive works \cite{DV}, \cite{Ka}.  
 
The most well-studied models among point processes on Euclidean spaces are the Poisson point processes. In a Poisson process, for any Borel subset $D\subseteq \R^{d}$, the configuration of points of the point process that fall inside $D$ and the configuration of points that fall inside $D^{c}$ are independent. For a general point process such independence is no longer valid, and in fact, the study of spatial conditioning in such processes becomes a an important and highly non-trivial question. An extensive literature on the topic has developed over the years, including on tractable generalisations of independence such as Gibbs-type properties \cite{Ge}. 

In the work \cite{GP}, a surprising phenomenon that is in a sense diametrically opposite to independence was shown to occur in certain point processes -- namely, some features of the configuration of points inside $D$ (eg., the number of points that fall in $D$) may be determined, almost surely, by the configuration of points in $D^{c}$. This phenomenon was referred to as {\em rigidity} in \cite{GP}. In other words, some statistic $X$ that is a measurable function of the points in $D$ may also be shown to be a measurable function of the points in $D^c$ (in which case $X$ is said to be rigid). The precise definitions of rigidity and related concepts will be given later in the article; for the present introductory discussions we will content ourselves with the idea as explained above.

 It was shown in \cite{GP} that for the infinite Ginibre ensemble (recalled more precisely in Result~\ref{res:ginibre}) on $\R^{2}$, the number of points inside a bounded region $D$ is determined by the configuration of points outside $D$ (i.e., by the configuration of points in $D^c$). It was also shown that for the zeroes of the canonical Gaussian entire function (see Result~\ref{res:GEF}), the number of points as well as the center of mass of the points in a bounded region are determined by the configuration of points outside. In both cases it was shown, in a precise sense, that nothing more than this can be determined by the configuration outside.

The goal of this paper is to systematically explore the extent of rigidity in several natural point processes. In Section \ref{sec:setup}, we give definitions of rigidity and tolerance following \cite{GP}, but in a more general setting. In Section \ref{sec:models}, we recall the known examples and related results in the literature. Further, we mention certain applications to the study of point processes to which these notions have been crucial. In Section~\ref{sec:ourresults} we state the new results of this paper. In subsequent sections we give proofs of these results.


\subsection{ Setup and fundamental notions}  \label{sec:setup}
In this section, we give definitions of rigidity and tolerance following \cite{GP}, albeit in a more general setting. 

The definition of point process on $\R^d$ recalled in the introduction generalizes in a straightforward way to point processes on any locally compact, second countable Hausdorff space (or l.c.s.h space in short).  Let  $\Xi$ be a l.c.s.h. space. Let $\mathcal M$ denote the space of Radon measures on $\Xi$, a Polish space with the topology of vague convergence. Let $\mathcal M_{p}\subseteq \mathcal M$ denote the closed subset  of integer-valued Radon measures on $\Xi$, and let $\S\subseteq \mathcal M_{p}$ denote the relatively open subset  of counting measures of locally finite subsets of $\Xi$.  As Borel subsets of $\mathcal M$, both $\mathcal M_p$ and $\mathcal S$ inherit Borel sigma-algebras. A random variable $\Pi$ defined on some probability space $(\Omega,\mathcal F,\P)$ is called a {\em random measure} if it takes values  in $\mathcal M$, a {\em point process} if it takes values (with probability 1) in $\mathcal M_p$ and a {\em simple point process} if it takes values (w.p. 1) in $\S$.  For more details on point processes, we refer the reader to \cite{bbkbook} (Chapter~1), \cite{DV}, \cite{Ka}.

If $D\subseteq \Xi$ is a Borel set, let $\S_{D}=\{\theta \in \S \suchthat \theta(D^{c})=0\}$. For a point process $\Pi$ on $\Xi$, let $\Pi_{D}$ denote the restriction of $\Pi$ to $D$, i.e., the point process on $\Xi$ satisfying $\Pi_{D}(A)=\Pi(A\cap D)$.  Let $\sigma\{\Pi_{D}\}$ denote the sigma-algebra generated by $\Pi_{D}$. Random variables measurable with respect to $\sigma\{\Pi_{D}\}$ are precisely those of the form $f(\Pi_{D})$ where $f:\S_{D}\mapsto \R$ is  measurable. 

The key  object in our study is the sigma-algebra $\Rig_{D}:=\overline{\sigma(\Pi_{D})}\cap \overline{\sigma(\Pi_{D^{c}})}$ where $\overline{\mathcal F}$ denotes the completion of a sigma-algebra $\mathcal F$. If $Y$ is an $\Rig_{D}$-measurable random variable, then there exist measurable functions $f_{\inn}:\S_{D}\mapsto \R$ and
$f_{\out}:\S_{D^{c}}\mapsto \R$ such that $Y=f_{\inn}(\Pi_{D})$ $a.s.$ and $Y=f_{\out}(\Pi_{D^{c}})$ $a.s.$ Thus, $\Rig_{D}$-measurable random variables are precisely those features of $\Pi_{D}$  which can be inferred exactly (with probability one), from a knowledge of the configuration $\Pi_{D^{c}}$.
\begin{definition}[Rigidity]
%Let $\Pi$ be a simple point process on a locally compact space $\Xi$ and let $D\subseteq \Xi$ be a Borel set.
A measurable function $f:\S_{D}\mapsto \R$ is said to be rigid for the pair $(\Pi,D)$ if $f(\Pi_{D})$ is $\Rig_{D}$-measurable.
\end{definition}
Clearly, this is interesting only if $f(\Pi_{D})$ is not a constant. In that case,  $\Rig_{D}$ contains events with non-trivial probability.

 The most basic feature of interest is the number of points in $D$, i.e., $N_{D}:\S_{D}\to \R$ defined as $N_{D}(\Pi)=\Pi(D)$. If $N_{D}$ is rigid for all pre-compact $D\subseteq \Xi$, then we say that $\Pi$ exhibits {\em rigidity of numbers}.

Once we establish that there are rigid functions, the natural question is, how many? This is captured by the following definition. We write  $\sigma\{Y_{i}\suchthat i\in I\}$ for the sigma-algebra generated by  $Y_{i}$, $i\in I$.
\begin{definition}[Tolerance]\label{def:tolerance} Let $f_{1},\ldots ,f_{m}:\S_{D}\mapsto \R$ be measurable functions. We say that the pair $(\Pi,D)$ is tolerant subject to $\{f_{1},\ldots ,f_{m}\}$ if $\sigma\{f_{1}(\Pi_{D}),\ldots ,f_{m}(\Pi_{D})\}$ and $\Rig_{D}$ are equal up to $\P$-null sets.
\end{definition}
The definition entails that each $f_{i}$ is rigid for $(\Pi,D)$ and for every $A\in \Rig_{D}$, there is a $B\in \sigma\{f_{1}(\Pi_{D}),\ldots ,f_{m}(\Pi_{D})\}$ such that $\P(A\Delta B)=0$. Of course, we may allow $m=\infty$ and make the same definition. This definition captures the idea that nothing more than $f_{i}(\Pi_{D})$, $i\le m$, can be determined by the outside configuration $\Pi_{D^{c}}$. Or more precisely, any feature of the point process inside $D$ that can be determined by the outside configuration is equal (almost surely) to a function of these $m$ features.

However, there are other ways to capture the same idea. In most of the cases that we encounter, the following stronger form of tolerance holds.
\begin{definition}[Tolerance - strong form] \label{def:tolerancestrong2}
In the language of Definition~\ref{def:tolerance}, we say that $(\Pi,D)$ is strongly tolerant  subject to $\{f_{1},f_{2},\ldots ,f_{m}\}$ if, almost surely, the conditional distribution of $\Pi_{D}$ given $\Pi_{D^{c}}$ is mutually absolutely continuous to the conditional distribution of $\Pi_{D}$ given $\sigma\{f_{1}(\Pi_{D}),\ldots ,f_{m}(\Pi_{D})\}$.
\end{definition}
There are other possible definitions of tolerance that lie between these two. In section~\ref{sec:thiswillberewritten} we discuss these and also explain the relationship between tolerance and strong tolerance. In particular, it is shown that strong tolerance implies tolerance, as the name suggests.
%The reader more interested in the results may read the rest of the paper accepting strong tolerance as the ``right definition''.

In general, the extent of rigidity could depend not only on the underlying point process but also on the sub-domain $D$. In almost all cases considered in this paper, the point process is on $\R^{2}$ and the extent of rigidity is the same for all bounded subsets $D$.   An exception is in non-projection determinantal processes of Theorem~\ref{detrig}, see Remark~\ref{rem:inclusion}.
% Hence we make the following definition.


%If $\Pi$ is a point process on $\R^{2}\cong \C$ with finite number of points (i.e., $  \Pi(\C)<\infty$ $a.s.$),  define $M_{k}(\Pi)=\int_{\C}z^{k}d\Pi(z)$ for $k\in \N$. For a general point process $M_{k}(\Pi_{D})$ makes sense for any bounded Borel set $D$.  Especially significant is $M_{0}(\Pi_{D})$, the number of points of $\Pi$ in $D$. which we also denote by $N_{D}$.
%\begin{definition} A simple point process $\Pi$ on the complex plane $\C$ is said to be rigid at level $k$ if the following conditions are satisfied.
%\begin{enumerate}
%\item For any bounded open set $D$, the pair $(\Pi,D)$ is strongly tolerant subject to $\{M_{0},\ldots ,M_{k-1}\}$,
%\item  Given $M_{j}(\Pi_{D})=m_{j}$ for $0\le j\le k-1$, the conditional distribution of $\Pi_{D}$ is mutually absolutely continuous to Lebesgue measure on the manifold
%\[
%\{(z_{1},\ldots ,z_{m_{0}})\in D^{m_{0}} \ : \ z_{1}^{j}+\ldots +z_{m_{0}}^{j}=m_{j}\mb{ for }1\le j \le k-1\}.
%\]
%This should hold for (almost) every $m_{0}\in \N$, $m_{1},\ldots ,m_{k-1}\in \mathbb C$.
%\end{enumerate}
%\end{definition}
%Clearly, analogous definitions can be made with any functions $\phi_{j}:\C\mapsto \R$ by defining tolerance subject to the linear statistics $\Lambda_{j}(\Pi_{D})=\int_{D} \phi_{j}(x)d\Pi(x)$, $0\le j\le k$. Such definitions can be extended beyond the complex plane. Even on the complex plane, one could consider non-holomorphic moments $M_{j,k}(\Pi_{D}):=\int_{D} z^{j}\bar{z}^{k}d\Pi_{D}(z)$, and for point processes that do not have joint intensities with respect to Lebesgue measure (for instance, point processes on $\Z^{2}$), etc. While the concepts of rigidity and tolerance and rigidity of numbers as given in the first three definitions are somehow fundamental, the definition of ``rigid up to level $k$''  in the last definition is deliberately made specific to the plane, and for the sake of conciseness in the statement of our results.

\subsection{Existing literature on rigidity and tolerance}  \label{sec:models}
In this section, we discuss significant strands of results available in the literature related to the topic of rigidity and tolerance, and applications thereof.
\subsubsection{Known models of rigidity and tolerance}
We begin with surveying available results on rigidity and tolerance phenomena for standard point processes.
A Poisson process has no rigidity. In other words, $\Rig_{D}$ is trivial for any $D$. It is interesting and non-trivial that there are point processes with any rigidity at all. We quote three sample results. The first two are from \cite{GP}  while the last is from \cite{G-1}.
%Result~\ref{res:ginibre} and Result~\ref{res:GEF} are from \cite{GP} while Result~\ref{res:sinekernel} is from \cite{G-1}.

{\it  Infinite Ginibre ensemble in the complex plane}: This is the determinantal point process defined by the kernel $e^{z\bar{w}}$ with respect to the measure $\frac{1}{\pi}e^{-\frac12 |z|^{2}}$ on the complex plane. For the definition of a determinantal point process, we refer the reader to \cite{soshnikov} or chapter 4 of \cite{HKPV} (we give a brief description in Section~\ref{sec:ourresults}). The infinite Ginibre ensemble is a translation and rotation invariant simple point process on the plane.
\begin{result}[\cite{GP}] \label{res:ginibre}The infinite Ginibre ensemble exhibits rigidity of numbers. Furthermore, the infinite Ginibre ensemble is strongly tolerant subject to the number of points for any bounded domain $D \subset \R^2$.\emph{}
%conditional on the number of points in a bounded domain $D$ being $m \ge 0$, the points of the process inside $D$ are mutually absolutely continuous with respect to the Lebesgue measure on $D^m$.
\end{result}
 Informally, the result says that for any bounded set $D$, from the  knowledge of $\Pi_{D^{c}}$, it is possible to determine the number of points in $\Pi_{D}$, but nothing more can be determined.

{\it Zero set of the canonical Gaussian entire function}: Let $\Pi$ be the zero set of the  random entire function $\sum_{n=0}^{\infty}\xi_{n}\frac{z^{n}}{\sqrt{n!}}$ where $\xi_{n}$ are i.i.d. standard complex Gaussian random variables (each $\xi_{n}$ has density $\frac1\pi e^{-|z|^{2}}$). Then, $\Pi$ is a translation and rotation invariant simple point process on the plane (see \cite{ST1} for details); for more on translation invariant zero sets of Gaussian analytic functions, see e.g. \cite{Fe}.

\begin{result}[\cite{GP}] \label{res:GEF} The zero set of the Gaussian entire function exhibits rigidity of the number and the center of mass of the points in any bounded domain $D \subset \R^2$.  Furthermore, for any bounded domain $D \subset \R^2$, this zero process is strongly tolerant subject to the number and the center of mass of the points.\emph{}
\end{result}
Informally, this means that for any bounded set $D$, from the knowledge of $\Pi_{D^{c}}$, it is possible to determine the number of points in $\Pi_{D}$ and the center of mass of these points, but nothing more.

{\it Sine-kernel determinantal point process on $\R$}: This is the determinantal point process with kernel $\frac{\sin(x-y)}{x-y}$ with respect to the Lebesgue measure on $\R$. This is a translation invariant simple point process (see section~2 of \cite{soshnikov}) that arises in the study of Hermitian random matrices.

\begin{result}(\cite{G-1}) \label{res:sinekernel} The sine-kernel determinantal point process exhibits rigidity of numbers.
\end{result}
A similar result was shown for a wide class of translation  invariant determinantal point processes on the real line. These determinantal processes (see Soshnikov~\cite{soshnikov} and Lyons and Steif~\cite{LySt}) have kernels of the form  $\hat{g}(x-y)$ where $g$ is the indicator of a subset of $\R^d$ having finite positive Lebesgue measure, see \cite{G-1} for details. 
%$\hat{g}(x-y)$ where $g\in L^{2}(\R)$  and $0\le g\le 1$; 
Number rigidity for sine beta processes was proved in \cite{DHLM}.

Bufetov~\cite{buf-3} demonstrated rigidity of numbers for determinantal point processes  with Airy, Bessel and Gamma kernels. These point processes are not translation invariant. In addition, Bufetov and Qiu~\cite{buf-1}, have shown rigidity for a class of determinantal processes in the plane. Their result has an overlap with, but does not subsume, Theorems~\ref{compact} and \ref{dpprt} that we prove in this paper. In addition, it is worth mentioning that in \cite{buf-2}, Bufetov, Dabrowski and Qiu study one-sided rigidity. In our terminology, this corresponds to taking $\Xi=\R$ and $D=[a,\infty)$. This result may be the only known result that proves rigidity for unbounded sets, although one may mention that analogous results (theorems of Szeg\"{o} and Kolmogorov on the complete predictability of a Gaussian process from its past) are known in the theory of Gaussian processes, see~ \cite{DymMackean}. Rigidity phenomena have subsequently been considered widely general set-ups, mostly in the case of determinantal processes, see e.g. Qiu (\cite{Qi})  and Hiraoka, Shirai and Trinh (\cite{HST}).

%{\color{blue}
%It is worth remarking that in all three results above, tolerance was shown in the following stronger form.
%\begin{definition}[Tolerance - strong form]
% \label{tolerancestrong2}
%Let $\Pi$ be a point process on $\Xi$ and let $D\subseteq \Xi$. Let $f_{i}:\S_{D}\to \R$ for $1\le i\le m$ be $\Rig_{D}$-measurable. We say that $(\Pi,D)$ is strongly tolerant  subject to $\{f_{1},f_{2},\ldots ,f_{m}\}$ if, almost surely, the conditional distribution of $\Pi_{D}$ given $\Pi_{D^{c}}$ is mutually absolutely continuous to the conditional distribution of $\Pi_{D}$ given $\sigma\{f_{1}(\Pi_{D}),\ldots ,f_{m}(\Pi_{D})\}$.
%\end{definition}
%In section~\ref{sec:thiswillberewritten} we explain the relationship between tolerance and strong tolerance. In particular, strong tolerance implies tolerance, as the name suggests.
%}

%
%{\color{blue}\begin{definition}[Tolerance - strong form]
% \label{tolerance}
% Let $\Pi$ be a point process on  $\R^{d}$ and let $\Phi_1,\ldots ,\Phi_{k}:\R^{d}\to \R$ be smooth functions and let $\Phi_{0}$ be the constant function $1$. Let $D \subset \Xi$ be a bounded open set. For $\Phi:\R^{d}\to \R$, let $\La(\Phi):\S_{D}\to \R$ be the linear statistic defined as $\La(\Phi)[\Pi]:=\int_D \Phi(z) d\Pi(z)$.
%
%  For integer $m \ge 0$  and $\us:=(s_1,\cdots,s_k) \in \C^k$, consider  the  submanifold of $D^m$ defined as
%\[
% \Sigma_{m,\us}:=\{ \uz=(\zeta_1,\cdots,\zeta_m) \in D^m : \La(\Phi_j)[\delta_{\uz}]=s_j \mb{ for } 1 \le j \le t  \},
% \]
% where $\delta_{\uz}=\sum_{i=1}^{m}\delta_{\zeta_{i}}$ is the counting measure corresponding to the point set $\{\zeta_i,\ldots ,\zeta_{m}\}$.
%
% We say that $\Pi$ is strongly tolerant subject to  $\{\La(\Phi_0),\La(\Phi_1),\cdots,\La(\Phi_k)\}$ if
% \begin{inparaenum}[(a)]
% \item $\La(\Phi_{j})$, $0\le j\le k$, are rigid for $(\Pi,D)$ and
% \item the conditional distribution of $\Pi_D$ given  $\Pi_{D^{c}}$ is mutually absolutely continuous to the point process of $\La(\Phi_0)[\Pi_D]=N(\o)$  points sampled independently from Lebesgue measure on the submanifold $\Sigma_{N(\o),\us}$ .
% \end{inparaenum}
%\end{definition}
%The reason for restricting to point processes on $\R^{d}$ is that there is a natural measure on $\Sigma_{m,\us}$. If $\Xi$ is a Riemannian manifold, it carries a natural volume measure and the same definition can be made. Even more generally, if $\Xi$ is a locally compact space endowed with a  Radon measure $\mu$ and $D$ has compact closure, then we can normalize $\mu\big|_{D}$ to a probability measure on $D$. Let  $U_{1},\ldots ,U_{m}$ be sampled independently from this probability measure. The regular conditional distribution of $(U_{1},\ldots ,U_{m})$ given that $(U_{1},\ldots ,U_{m})\in \Sigma_{m,\us}$ exists and defines the measure on $\Sigma_{m,\us}$ which can be used to define strong form of tolerance.}



\subsubsection{Related literature} In \cite{OsSh}, Osada and Shirai showed that for the Ginibre ensemble, the Palm measures with respect to different point sets are mutually absolutely continuous if the conditioning set of points have the same cardinality, and are mutually absolutely continuous otherwise. Such dichotomy is similar in spirit to, and is, in fact, closely related with the rigidity phenomena under our consideration. There has been recent interest in examining the extent to which rigidity can occur in stochastic systems, including applications to spectrally constrained random systems, \textit{stealthy} models, and maximal rigidity; see e.g. the recent works \cite{GhL, AGL} and also the paper \cite{KiNi} that are pursuant to an earlier arxiv version of our present paper \cite{GhK}. For connections between the strength of rigidity in a point process and its \textit{Palm measures}, we refer the reader to \cite{G-2}. In the more general area of spatial conditioning in point processes, important progress has been obtained recently in \cite{BQS} in the setting of determinantal processes, which also establishes the Lyons-Peres completeness conjecture. 
%For more on this theme, we refer the reader to the upcoming article \cite{G-2}.



\subsubsection{Applications to other aspects of point processes:} The study of rigidity, although natural, is not an end in itself. Rigidity phenomena have  been exploited to answer questions on point processes and stochastic geometry that are interesting in their own right.

In \cite{G-1}, rigidity of the sine kernel process (Result~\ref{res:sinekernel}) was exploited to answer a completeness question related to exponential functions coming from the point process. In \cite{GKP}, the authors used an understanding of the rigidity behaviour of the Ginibre ensemble and the zero set of the Gaussian entire function   (Result~\ref{res:ginibre} and Result~\ref{res:GEF}) in order to study continuum percolation on these models. In particular, they showed the  existence of a non-trivial critical radius for percolation, and established the uniqueness of the infinite cluster in the supercritical regime.

In \cite{Os}, an understanding of  quasi-Gibbs property, which has a somewhat similar  flavour to rigidity and tolerance, was used to define an infinite particle SDE for invariant dynamics on the Ginibre process. To execute a similar programme for invariant dynamics on the zero set of the Gaussian entire function, one faces new challenges involving the higher level of rigidity in Result~\ref{res:GEF}, and it is a topic of current research.

\section{Our results}\label{sec:ourresults}
Now we present our results along with some remarks on our motivations and on what more could be true but are not known.

\subsection{Point processes with higher levels of rigidity and $\a$-GAFs} \label{sec:higher_rig}
The Results~\ref{res:ginibre} and \ref{res:GEF} demonstrate point process that are rigid only with respect to the local mass or local mass and center of mass respectively. The primary  question that we explore in this section is whether there are there natural point processes that exhibit higher levels of rigidity.  This could, for example, entail that for some $k\ge 3$ and any bounded set $D$, the $k$-th moment (i.e., the sum of $k$th powers) of the points of the process that fall in $D$ can be determined by the outside configuration $\Pi_{D^{c}}$.

We answer this natural  question in the affirmative, by constructing zero sets of Gaussian entire functions with arbitrarily high degrees of rigidity. To this end, we first define $\a$-Gaussian analytic functions (\textit{abbrv.} $\a$-GAF).

\begin{definition}
  For a real number $\a>0$,  the $\a$-GAF is the random entire function  \[f_\a(z):=\sum_{k=0}^\infty \frac{\xi_k}{(k!)^{\a/2}}z^k\]
  where $\xi_{k}$ are i.i.d. standard complex Gaussian random variables.
 \end{definition}
For $\a=1$, we are reduced to the canonical planar Gaussian entire function whose zero set is a translation-invariant point process (see Proposition~2.3.4. in \cite{HKPV}). For any $\a\not=1$, the zero set of $\a$-GAFs is not translation-invariant in the plane. Figure~\ref{fig:alphagafzerosets} demonstrates how the parameter $\alpha$ affects the distribution of the zeroes.


% aware of any translation invariant point processes that is rigid at level $3$ or more,  but the following theorem at least gives natural enough point processes with arbitrarily high levels of rigidity.

% In this paper, we answer the above question by introducing a family of point processes, indexed by a parameter $\a>0$, such that for different values of $\a$  there is a different rigidity behaviour. These are also Gaussian analytic functions, albeit with different scaling behaviour of the coefficients from the standard one. In fact, we show that there is a monotonicity in the rigid behaviour with respect to the parameter $\a$: for $\frac{1}{k} < \a \le \frac{1}{k-1}$ (where $k \ge 0$ is an integer), the resulting point process is rigid at level $k$. For the special case $\a=1/2$, we recover the standard planar GAF. We call this family of Gaussian analytic functions as $\a$-GAF, which we formally define as follows:
For stating our main theorem of this section, we recall that the (holomorphic) $p$-th moment (or the moment of order $p$, for any integer $p \ge 0$) of a (finite) point set $\{z_1,\cdots,z_m\} \subset \R^2=\C$ is given by $z_1^p + \cdots +z_m^p$, where the $z_i$ are treated as complex numbers. By the first $p$ moments of such a point set, we imply the set of its moments of order $\{0,1,\ldots,p-1\}$.

 \begin{theorem}
  \label{hierig}
  The zero set of the $\a$-GAF exhibits rigidity of the first $k$ moments of its points in any bounded domain $D \subset \R^2$ whenever $\a \in (\frac{1}{k} , \frac{1}{k-1}]$.
 \end{theorem}

In the forthcoming paper \cite{G-3}, we investigate and answer in the affirmative the question of the strong tolerance of the $\a$-GAF zeros given the first $k$ moments of its points in a bounded domain (where $\a \in (\frac{1}{k} , \frac{1}{k-1}]$, as in the statement of Theorem \ref{hierig}).

\subsection{Rigidity of determinantal point processes} \label{sec:DPP}
Result~\ref{res:ginibre} and Result~\ref{res:sinekernel} exhibit determinantal point processes on $\R^{2}$ and on $\R$ that exhibit rigidity of numbers, and strongly tolerant given the number of points (i.e., for any bounded set $D$, the number of points of the process that fall inside $D$  is determined by the outside configuration $\Pi_{D^{c}}$, but nothing more). The natural question that arises pertains to the rigidity and tolerance properties exhibited a general determinantal point process. To articulate our result, we first recall the precise notion of a determinantal point process.

A determinantal point process (henceforth abbreviated as d.p.p.) on $\Xi$ with a Hermitian kernel $K:\Xi\times \Xi\to \C$ (Hermitian means that $K(x,y)=\overline{K(y,x)}$) and a (Radon) measure $\mu$, is a point process whose joint intensities (also called correlation functions)  with respect to $\mu$ are given by
\begin{align*}
\rho_{k}(x_{1},\ldots ,x_{k}) = \det\l(K(x_{i},x_{j})\r)_{i,j\le k}
\end{align*}
for any $k\ge 1$ and any $x_{1},\ldots ,x_{k}\in \Xi$. We refer to \cite{HKPV}, chapters 1 and 4, for more details of these notions.  All information about a determinantal process is in the kernel $K$, once the  measure $\mu$ is fixed. For $D\subseteq \Xi$, we define the integral operator $\mathcal K_{D}:L^{2}(D,\mu)\mapsto L^{2}(D,\mu)$ by
\[
(\mathcal K_{D} f)(x)=\int_{D}K(x,y)f(y)d\mu(y).
\]
We say that the kernel $K$ is locally of trace-class if for every $D\subseteq \C$ that is pre-compact, the operator $\mathcal K_{D}$ is of trace-class. We write $\mathcal K$ for $\mathcal K_{\Xi}$.

It is well known that the kernel and background measure completely determine the distribution of a determinantal point process (Lemma~4.2.6 in \cite{HKPV}). Hence in principle, the rigidity properties of a determinantal process are encoded in its kernel and background measure, possibly in a highly indirect and complicated manner. 

A natural problem, therefore, is to understand the rigidity and tolerance behaviour of a determinatal point process in the form of a simple criterion expressed in terms of the kernel.  We provide a partial answer to this question by specifying conditions on the pair $(K,\mu)$ that mandate a certain rigidity behaviour of the determinantal process. More specifically, we investigate conditions under which a determinantal process has rigidity of numbers. Recall that this means that for any $D\subseteq \Xi$ whose closure is compact, the counting function $N_{D}:\S_{D}\mapsto \R$, is rigid.

To state our  result, we recall the following result of Machchi and Soshnikov (see Theorem~3 in Soshnikov~\cite{soshnikov}): Let $K$ be locally of trace-class and Hermitian. Then, a determinantal point process with the pair $(K,\mu)$ exists if and only if $0\le \mathcal K\le I$. Equivalently, the spectrum of $\mathcal K$ is contained in $[0,1]$. Clearly $\mathcal K$ defines a projection operator if and only if its spectrum is contained in $\{0,1\}$.
%In that case, we say that the determinantal point process is a projection determinantal process.

Now we are ready to state a necessary condition for a determinantal point process to exhibit rigidity of numbers.
 \begin{theorem}
  \label{detrig}
  Let $\Pi$ be a determinantal point process with kernel $K$ and background measure $\mu$. Then $\Pi$ exhibits rigidity of numbers only if the integral operator $\mathcal K$ associated to $K$ is a projection operator.
  \end{theorem}

\begin{remark} \label{rem:inclusion} 
The statement of Theorem \ref{detrig} primarily entails the contrapositive of being number rigid, in the sense that, if $\mathcal K$ is not a projection operator, then there exists a  precompact Borel set $D$ (possibly depending on $\mathcal K$) such that the point count in $D$ (i.e., $N_D(\Pi)$) is not rigid. However, it may be easily  seen that, if the point count in a domain $D_1$ (i.e., $N_{D_1}(\Pi)$)  is not rigid, then the same will hold true for the point count $N_{D_2}(\Pi)$ for any domain $D_2$ such that $D_1 \subseteq D_2$ (for a detailed argument, see Lemma \ref{lem:inclusion} in Section \ref{sec:thiswillberewritten}). 

However, it is not true in general that  rigidity of numbers holds for all bounded sets.  For example, let  $D_0$ be a bounded open set in $\R^d$, and suppose that $\mathcal K_{D_0}$ is a projection  of finite rank $n$ and that $\mathcal K_{D_0^c}$ is not a projection. Examples are easy to construct, for example by taking  finite rank projection operators $\mathcal K_1$ and $\mathcal K_2$ on $L^2(D_0)$ and $L^2(\D_0^c)$ respectively, and setting $\mathcal K=\mathcal K_1\oplus \frac12 \mathcal K_2$ (the direct sum; in terms of the associated kernels, $K=K_1$ one $D_0$ and $K=\frac12 K_2$ on $D_0^c$). Then $\mathcal K$ is a not a projection, and the corresponding DPP does fail to have number rigidity for some $D$. However, $\Pi$ has exactly $n$ points in $D_0$ and hence for any $D\subseteq D_0$, we do have number rigidity, since $N_D(\Pi)=n-N_{D^c\cap D_0}(\Pi)$, which is measurable w.r.t. $\sigma(\Pi_{D^c})$. 
\end{remark}


It is an interesting question as to whether, conversely, every projection determinantal point process exhibits rigidity of numbers. This is certainly true for  the infinite Ginibre ensemble (Result~\ref{res:ginibre}) and for the sine-kernel process on the line (Result~\ref{res:sinekernel}), but is not true in complete generality.

A counter-example is provided by the  Bergman determinantal point process, which is a determinantal process on the unit disk $\mathbb D=\{z\in \mathbb C \! : \! |z|<1\}$ whose kernel is the Bergman kernel $K(z,w)=(1-z\bar{w})^{-2}$ and  $d\mu(z)=\pi^{-1}dm(z)$ is the normalized Lebesgue measure on the unit disk. The corresponding operator is the projection from $L^{2}(\mu)$ onto the subspace of square integrable holomorphic functions. Holroyd and Soo~\cite{HS} have shown that this determinantal process is  insertion tolerant and deletion tolerant\footnote{A point process $\Pi$ on $\R^{d}$ is said to be insertion tolerant  if for any set subset  $A\subseteq\R^{d}$ with positive, finite Lebesgue measure, if a point $U$ is sampled uniformly from $A$ and added to $\Pi$, the distribution of the resulting point process $\Pi+\del_{U}$, is absolutely continuous to the distribution of $\Pi$. Poisson process is an obvious example. Evidently, an insertion tolerant point process does not have rigidity of numbers.}. Consequently it does not display rigidity of numbers.



However, this is an example where the ambient space (the hyperbolic plane) exhibits non-Euclidean geometry (in particular, it displays hyperbolic or Lobachevskian geometry \cite{Terras,And,Lob}). This still leaves open the question of whether a translation-invariant determinantal point process on a $\R^{d}$ given by a projection kernel  necessarily exhibits rigidity of numbers, or more generally, what can be said about the rigidity  properties of such point processes. We do not have a complete answer to this question, but in this work we are able to prove rigidity of numbers (or the lack of it) for a significant class of determinantal point processes in the plane. This is taken up for consideration in the next section.

\subsection{Radial determinantal processes on the plane} \label{sec:radial}
 Let $\gamma$ be a radially symmetric probability measure on the complex plane such that $c_{j}^{-1}:=\int_0^\infty |z|^{2j} d\gamma(z)<\infty$ for all $j$. Then $\{\sqrt{c_{j}}z^{j} \! : \! j\ge 0\}$ is an orthonormal set in $L^{2}(\gamma)$. It is an orthonormal basis for the subspace of holomorphic functions in $L^{2}(\gamma)$ and the projection operator onto this closed subspace is given by the kernel $K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j$.  By the result of Machchi and Soshnikov quoted earlier, there is a unique  determinantal process with kernel $K$ and measure $\gamma$. These processes include the infinite Ginibre ensemble (when $\gamma$ is standard complex Gaussian measure on the plane) and the Bergman determinantal process (when $\gamma$ is normalized uniform measure on the unit disk).


 Before stating the main result in this section, we introduce the following quantities.
 %Let $\Gamma_j$ be the size biasing of $\mu$ of the order $j$; in other words, $\Gamma_j$ has a density which is proportional to $r^jd\mu(r)$. Let
% \[\mu_j:=\E[\Gamma_j]=c_j/c_{j+1},\] \[\sigma_j:=\E\l[\l(\frac{\Gamma_j}{\mu_j}-1\r)^2\r]=\l(\frac{\mu_{j+1}}{\mu_j}-1\r)\] and  \[\nu_j := \E\l[  \l(\frac{\Gamma_j}{\mu_j}-1\r)^4\r]= \l( \frac{\mu_{j+3}\mu_{j+2}\mu_{j+1}}{\mu_j} - 4 \frac{\mu_{j+2} \mu_{j+1}}{\mu_j^2} + 6 \frac{\mu_{j+1}}{\mu_j} -3 \r).\]
 \begin{align*}
 \mu_j:=\frac{c_j}{c_{j+1}}, &\qquad \sigma_j:=\frac{\mu_{j+1}}{\mu_j}-1, \qquad
 \nu_j := \; \frac{\mu_{j+3}\mu_{j+2}\mu_{j+1}}{\mu_j^3} - 4 \frac{\mu_{j+2} \mu_{j+1}}{\mu_j^2} + 6 \frac{\mu_{j+1}}{\mu_j} -3.
 \end{align*}
 In the setting described so far, we prove the following theorems.
 \begin{theorem}
 \label{compact} Let $\Pi$ be the determinantal point process  on $\C$ with kernel $K$ with respect to the radial background measure $\gamma$. If $\sum_{j=1}^{\infty}\sigma_j < \infty$, then the process $\Pi$ does not exhibit rigidity of numbers.
\end{theorem}
 \begin{theorem}
 \label{dpprt}
 Let $\Pi$ be the determinantal point process on $\C$ with kernel $K$ with respect to the radial background measure $\gamma$. Assume that \begin{inparaenum}[(1)] \item $\mu_j \to \infty$ as $j \to \infty$, \item $\sum_{j=1}^{\infty}\nu_j<\infty$ and \item$\sum_{j=1}^{k} \mu_j^4 \nu_j= o(\mu_k^4)$ as $k \to \infty$.  \end{inparaenum}  Then $\Pi$ exhibits rigidity of numbers.
\\
%\indent Suppose that in addition to the previous conditions,  the measure $\mu$ is  absolutely continuous w.r.t. the Lebesgue measure on $\C$, and that for some integer $a \ge 1$ we have $\sum_{j=1}^{\infty}\mu_j^{-a}<\infty$. Then, for any bounded domain $D$, the point process $\Pi$ exhibits rigidity of the particle number in $D$, and is strongly tolerant given this particle number.
\end{theorem}
The condition $\sum_{j}\sigma_{j}<\infty$ in Theorem~\ref{compact} is satisfied if $\mu_j=A+Bj^{-1}+ O(j^{-2})$. The conditions in Theorem~\ref{dpprt} are satisfied if $\mu_j=Cj^a(1+A j^{-1} + O(j^{-2}))$. The latter is certainly the case if $\mu$ has density proportional to $|z|^{\alpha}e^{-|z|^{\beta}}$. This includes the infinite Ginibre ensemble with $\alpha=0$ and $\beta=2$.

We believe that the additional moment assumption $\sum_{j=1}^{\infty}\mu_j^{-a}<\infty$ for some integer $a \ge 1$ would suffice to establish strong tolerance for the process $\Pi$ in Theorem \ref{dpprt} for any bounded domain $D$ subject to its particle number. However, the rigorous demonstration of such a result would take us too far afield with regard to techniques and methods, and it would be appropriate to leave such considerations for a different occasion.

%\begin{remark} We believe that the additional moment assumption $\sum_{j=1}^{\infty}\mu_j^{-a}<\infty$ for some integer $a \ge 1$ would suffice to establish strong tolerance for the process $\Pi$ in Theorem \ref{dpprt} for any bounded domain $D$ subject to its particle number. However, the rigorous demonstration of such a result would take us too far afield with regard to techniques and methods, and such considerations may be deferred for a different venue.
%\end{remark}


 %is enough to establish that the inverse power sums \[\l( \sum_{z \in \Pi_n \cap \D^c} \frac{1}{z^k} \r)\] is bounded above in expectation.
%Exploiting this fact, and employing the techniques introduced in \cite{GP} to deal with the Ginibre ensemble, it can be shown that $\Pi$ is rigid of order 1.

%The assumption of absolute continuity on the measure $\gamma$ is made because we defined rigidity at level $k$ with respect to Lebesgue measure on the plane. In general, strong tolerance holds, and in fact  the conditional distribution (given $\Pi_{D^{c}}$) of the vector of $N(D)$ points inside the disk, when put in a uniform random order, is  mutually absolutely continuous to $\gamma^{\otimes N(D)}$. The proof goes through with minor changes.


While Theorems \ref{compact} and \ref{dpprt} cover a good class of radially symmetric determinantal processes, it would be definitely very interesting to sharpen the dichotomy present in these two theorems. In particular, it be of great interest to extend this dichotomy and establish that it is the compactness or the non-compactness of the support of the measure $\mu$ that determines the rigidity behaviour of the determinantal process (e.g. as in Theorems \ref{compact} and \ref{dpprt}).


\subsection{Perturbed lattice models} \label{sec:perturbed_lattice}
 A perturbed lattice  is the point process $\sum_{k\in \Z^d}\delta_{k+\xi_{k}}$, whose points are $\{k+\xi_{k}\! : \! k\in \Z^{d}\}$ where $\xi_{k}$ are independent $\R^{d}$-valued random vectors. Thus, heuristically speaking, by a perturbed lattice we mean a point process obtained by perturbing the points of a lattice by independent random variables. 

In one dimension, if the perturbations are i.i.d., non-degenerate and have finite variance, then it can be shown that the resulting point process exhibits rigidity of numbers, and is strongly tolerant given the particle number for any bounded domain.  For i.i.d. lattice perturbations of $\Z^2$, the situation is similar these results are due to Holroyd and Soo \cite{HS}. Remarkably, for i.i.d.  perturbations by isotropic Gaussians in dimensions $d \ge 3$, it is known (\cite{PS}) that there is a phase transition in the variance of the perturbing Gaussian. Then, there is a critical $\sigma_c$ such that if the variance of the perturbing Gaussians is more than $\sigma_c^2$, then the point process is deletion tolerant\footnote{A point process $\Pi$ is said to be deletion tolerant if for any randomly chosen point $Z$ of $\Pi$, the distribution  of the point process $\Pi-\del_{Z}$ got by deleting the point at $Z$, is absolutely continuous to the distribution of $\Pi$.}, while for  perturbations with variance less than $\sigma_c^2$ it exhibits rigidity of numbers.

In this work we investigate the setting of dimension $1$ and Gaussian perturbations, but where the perturbations are no longer identically distributed.  The following theorem entails that if we posit a power law growth for the variances of the perturbations, the model undergoes a phase transition in the rigidity behaviour as follows.

\begin{theorem}
 \label{power}
Consider the point process $\X=\sum_{k\in \Z}\delta_{k+Z_k}$ on $\R$, where $Z_k\sim N(0,\sigma_\beta(k))$ are independent and $\sigma_\beta(k) = |k|^\beta$. Then,
  \begin{enumerate}
  \item For $\beta>1/2$, $\X$ does not exhibit rigidity of numbers. 
  \item For $\beta \le 1/2$, $\X$ exhibits rigidity of the number of points in any bounded domain  and strong tolerance given this  number.
  \end{enumerate}
\end{theorem}
% The reader interested in the proofs of Theorems stated in this section may skip the next section which is about various possible definitions of tolerance and their inter-relationships.





% =============
% The study of rigidity phenomena in random point sets has attracted a fair amount of attention in the recent past. To put it informally, ``rigidity'' refers to a phenomenon where, for a bounded domain $\D$ in the ambient space, the points of the set outside $\D$ determine, almost surely, certain properties of the points inside. In other words, we consider spatial conditioning in the random point set, and ``rigidity'' broadly refers to singularities appearing in the conditional distribution of the points inside $\D$ given the locations of those outside.
%
% We take this opportunity to provide a rigorous formulation of the phenomenon of ``rigidity'', on similar lines to \cite{GP}. Let us first describe the set-up in which we will work, and introduce some fundamental notions. A (simple) point process $\Pi$ is a random locally finite point configuration on some metric space $\Xi$ that is equipped with a regular Borel measure $\mu$. A point process can equivalently be looked upon as a random counting measure, with atoms corresponding to the points. For more details on point processes, we refer the reader to \cite{DV} and \cite{Ka}. The space $\S$ of locally finite point configurations on $\Xi$ is a Polish space, and a point process $\Pi$ on $\Xi$ can be thought of as a probability measure on $\S$.  Let $\D \subset \Xi$ be a bounded open set. The decomposition $\Xi=\D \cup \D^c$ induces a factorization $\S=\S_{\inn} \times \S_{\out}$, where $\S_{\inn}$ and $\S_{\out}$ are respectively the spaces of  finite point configurations on $\D$ and locally finite point configurations on $\D^c$.  This immediately leads to the natural decomposition $\Upsilon=(\Upsilon_{\inn},\Upsilon_{\out})$ for any $\Upsilon \in \S$, and  consequently a decomposition of the point process $\Pi$ as $\Pi=(\Pi_{\inn},\Pi_{\out})$.

% We are now ready to formulate a rigorous definition of rigidity as follows.
% \begin{definition}
% \label{defrig}
%A measurable function $f_{\inn} : \S_{\inn} \rightarrow \C $ is said to be \textbf{rigid} with respect to the point process $X$ on $\S$ if there is a measurable function  $f_{\out}:\S_{\out} \rightarrow \C$ such that a.s. we have $f_{\inn}(X_{\inn})=f_{\out}(X_{\out})$.
%\end{definition}
%
% Of course, the phenomenon of rigidity is the most interesting in the case of point processes that have infinitely many points. For finite processes (of a given size), the points outside a domain $\D$ will determine the number of points inside $\D$, and in the usual case of the points having a joint density, these points inside $\D$ could be in almost any configuration in $\D$. However, such simplistic behaviour cannot be expected, and indeed, is not true for point processes of infinite size.
%
% The most common point process of infinite size, used as a model for many real world phenomena, is the Poisson point process. The most significant property of the Poisson process is the statistical independence of points in disjoint domains, and this property ensures that there is no ``rigidity'' of any sort for the Poisson process. However, for processes with non-trivial spatial correlation, the exploration of rigidity phenomena remains an interesting question. Among the most important natural examples of point processes of this kind are the bulk scaling limits of various random matrix ensembles, e.g. the sine kernel process in one dimension, or the Ginibre ensemble in two dimensions. Other significant ensembles include the zeroes of the standard planar Gaussian Analytic Function, abbreviated as the (standard planar) GAF on the complex plane, and the zeroes of the standard GAF on the hyperbolic plane.
%
% The underlying randomness in most of these processes comes from independent Gaussian random variables, and inspite of the non-trivial spatial correlations, it would be natural to expect a fair amount of regularity or smoothness in the conditional distributions (under spatial conditioning). For example, one might expect that the conditional distribution of the points inside a given domain $\D$ would be, a.s., mutually absolutely continuous with respect to a Poisson process on $\D$. However, it turns out that in many of these processes, such anticipated regularity is not true. On the contrary, the conditional distribution of the points inside $\D$ is highlly sinngular, in the sense that the support of the conditional measure is a singular subset of the ambient domain.
%
% In \cite{GP}, the authors studied rigidity phenomena with regard to the Ginibre ensemble and the standard planar GAF zero process. The Ginibre ensemble is the weak limit of the eigenvalues of non-Hermitian (complex) Gaussian random matrices. The standard planar GAF is the Gaussian power series \[f(z)=\sum_{k=0}^\infty \frac{\xi_k}{\sqrt{k!}}z^k,\] and the GAF zero process is the point process of zeroes of this random analytic function. For more details on these ensembles, we refer the reader to \cite{HKPV}.
%
% The study of rigidity phenomena in point processes has received some attention in the recent past; we mention here some of the works relevant to our study. In \cite{G-1}, it was shown that the sine kernel process (which arises as the bulk limit of Hermitian random matrix ensembles) exhibits rigidity in the number of points in a domain. Similar results were also established for a wide range of translation invariant determinantal point processes on $\Z$ (introduced by Lyons and Steif \cite{LySt}) that correspond to function spaces characterised by vanishing Fourier transform outside a given set. In \cite{OsSh}, Osada and Shirai showed that for the Ginibre ensemble, the Palm measures with respect to different point sets are mutually absolutely continuous if the conditioning set of points have the same cardinality, and are mutually absolutely continuous otherwise. Such dichotomy is similar in spirit to, and is, in fact, closely related with the rigidity phenomena under our consideration. For more on this theme, we refer the reader to the upcoming article \cite{G-2}.
%
% Rigidity phenomena have also been exploited to answer questions on point processes and stochastic geometry which are interesting in their own right. In \cite{G-1}, rigidity of the sine kernel process was exploited to answer a completeness question related to exponential functions coming from the point process. In \cite{GKP}, the authors used an understanding of the rigidity behaviour of the Ginibre ensemble and the standard planar GAF zero process obtained in
% \cite{GP} in order to study continuum percolation on these models. In particular, they showed the  existence of a non-trivial critical radius for percolation, and established the uniqueness of the infinite cluster in the supercritical regime. In \cite{Os}, an understanding of  quasi-Gibbs property, which has a somewhat similar  flavour to rigidity and tolerance, was used to define an infinite particle SDE for invariant dynamics on the Ginibre process. To execute a similar programme for invariant dynamics on the standard planar GAF zero process involves new challenges involving the higher level of rigidity in GAF, and is a topic of current research.
%
% In \cite{GP}, the authors showed that in the Ginibre ensemble, the points outside any bounded open set $\D$ determine a.s. the number of points inside $\D$, and in the GAF zero process, the points outside $\D$ determine the number and the sum of the points inside. If we think of the points as a particle system, then this can be described by saying that in the Ginibre ensemble, there is local conservation of mass, while in the standard planar GAF zero process, the mass as well as the centre of mass are locally conserved. Moreover, they showed that these are the ``only'' conservation laws in these ensembles, in a natural sense. To be precise, we quote the relevant theorems from \cite{GP}.
%
% In Theorems \ref{gin-1}-\ref{gaf-2} we denote the Ginibre ensemble by $\G$ and the GAF zero ensemble by $\F$. As before, $\D$ is a bounded open set in $\C$.

% In the case of the Ginibre ensemble, we prove that a.s.  the points outside $\D$ determine the number of points inside $\D$, and ``nothing more''.

%\begin{theorem}
% \label{gin-1}
%For the Ginibre ensemble, there is a measurable function $N:\S_{\out} \to \nat$ such that a.s. \[ \mathrm{ \ Number \ of \ points \ in \ } \G_{\inn} = N(\G_{\out})\hspace{3 pt}.\]
%\end{theorem}

%Since a.s. the length of $\uz$ equals $N(\G_{\out})$, we can assume that each measure $\rho(\uout,\cdot)$ is supported on $\D^{N({\uout})}$.

%
%\begin{theorem}
%\label{gin-2}
%For the Ginibre ensemble, $\P$-a.s. the measure $\rho({\G_{\out}},\cdot)$ and the Lebesgue measure $\el$ on $\D^{N(\G_{\out})}$ are mutually absolutely continuous.
%\end{theorem}

%In the case of the GAF zero process, we prove that the points outside $\D$ determine the number as well as the centre of mass (or equivalently, the sum) of the points inside $\D$, and ``nothing more''.

%\begin{theorem}
% \label{gaf-1}
%For the GAF zero ensemble, \newline
%\noindent
%(i)There is a measurable function $N:\S_{\out} \to \nat$ such that a.s.  \[ \mathrm{ \ Number \ of \ points \ in \ } \F_{\inn} = N(\F_{\out}).\]
%(ii)There is a measurable function $S:\S_{\out} \to \C$ such that a.s.  \[ \mathrm{ \ Sum \ of \ the \ points \ in \ } \F_{\inn} = S(\F_{\out}).\]
%\end{theorem}

%For a possible value $\uout$ of $\F_{\out}$, define the set of admissible vectors of inside points (obtained by considering all possible orderings of such inside point configurations) \[ \Sigma_{S({\uout})} := \{ \uz \in \D^{N({\uout})} : \sum_{j=1}^{N({\uout})} \z_j = S({\uout}) \}\] where $\uz=(\z_1,\cdots,\z_{N({\uout})})$.

%Since a.s. the length of $\uz$ equals $N({\uout})$, we can assume that each measure $\rho(\uout,\cdot)$ gives us the distribution of a random vector in  $\D^{N({\uout})}$ supported on $\Sigma_{S({\uout})}$.

%\begin{theorem}
%\label{gaf-2}
%For the GAF zero ensemble, $\P$-a.s. the measure $\rho(\F_{\out},\cdot)$ and the Lebesgue measure $\els$ on $\Sigma_{S(\F_{\out})}$ are mutually absolutely continuous.
%\end{theorem}

%Theorems \ref{gin-2} and \ref{gaf-2} lead to a natural definition of ``tolerance'' for point processes. Heuristically, this corresponds to the regularity of the spatially conditional measures, modulo local rigidity constraints. Before making a formal definition, let us recall the definition of linear statistics:
%\begin{definition}
% \label{linstat}
%Let $\Pi$ be a point proces on $\Xi$ and $\ph:\Xi \to \C$ be a measurable function. Then the linear statistics $\La(\ph)[\Pi]$ of $\Pi$ is defined to be the random variable \[\La(\ph)[\Pi]:=\int_\Xi \ph(z) d[\Pi](z).\]
%\end{definition}

%
%\begin{definition}
% \label{tolerance}
% Let $\Pi$ be a point process on a Riemannian manifold $\Xi$ with volume measure $\mu$. Let $\D \subset \Xi$ be a bounded open set, and let $\La(\Phi_0),\La(\Phi_1),\cdots,\La(\Phi_t)$ be rigid linear statistics of the point process $\Pi_\inn$ on $\D$, with $\Phi_0 \equiv 1$ and $\Phi_1,\cdots,\Phi_t:\D \rightarrow \C$ smooth functions.
%
% For an integer $m \ge 0$  and $\us:=(s_1,\cdots,s_t) \subset \C^t$, consider the submanifold of $\D^m$ \[\Sigma_{m,\us}:=\{ \uz=(\zeta_1,\cdots,\zeta_m) \in \D^m : \La(\Phi_j)[\delta_{\uz}]=s_j; 1 \le j \le t  \},\] where $\delta_{\uz}$ is the counting measure corresponding to the point set $\{\zeta_i\}_{i=1}^m$.
%
% Then $\Pi$ is said to be tolerant subject to  $\La(\Phi_0),\La(\Phi_1),\cdots,\La(\Phi_t)$ if the conditional distribution $\l(\Pi_\inn | \Pi_\out=\o \r)$ is mutually absolutely continuous with the point process of $\La(\Phi_0)[\Pi_\inn]=N(\o)$ points sampled independently from the submanifold $\Sigma_{N(\o),\us}$ (where $s_i=\La(\Phi_i)[\Pi_\inn]=S_i(\o), 1\le i \le t$) equipped with the restriction of the volume measure $\mu^{\otimes N(\o)}$.
%\end{definition}

%\begin{remark}
% One can generalise the above notion of tolerance by demanding constraints on more general functionals than linear statistics. For example, for a fixed positive integer $k$, one can consider a smooth function $\Psi:\D^k \to \C$ and demand that the functional $\La^{(k)}(\Psi):=\int \int \Psi d[\Pi_\inn]^{\otimes k}$ is rigid.
%\end{remark}

%Theorems \ref{gin-2} and \ref{gaf-2} can be phrased in terms tolerance as defined above. E.g., Theorem \ref{gin-2} can be rephrased by saying that for any bounded open set $\D$, the Ginibre ensemble  is tolerant subject to the number of points in $\D$.

%In view of these results, it is natural to ask whether there are point processes which exhibit higher levels of rigidity, in the sense that higher moments of the points inside $\D$ are also conserved. In a technical sense, we can formulate this question as follows.
%
%\begin{definition}
% \label{hie}
% We say that a point process $\Pi$ on $\C$ is rigid at level $k$ if the following conditions hold for every bounded open set $\D \subset \C$:
% \begin{itemize}
%  \item The linear statistics of $\Pi_\inn$ given by $\{\La(z^{j})\}_{j=0}^{k-1}$ are rigid.
%  \item $\Pi$ is tolerant subject to $\{\La(z^{j})\}_{j=0}^{k-1}$.
% \end{itemize}
%\end{definition}

%In terms of the last definition, we can say that the Ginibre ensemble is rigid at level 1 and the standard planar GAF zero process is rigid at level 2.
%
%Of course, we would like to consider ``natural'' models of point processes exhibiting higher levels of rigidity. As in, the models should not be toy examples engineered to precisely conform to such notions of rigid behaviour. One potential source of such toy models could be lattice perturbations, with the perturbations constrained so as to obtain rigidity at the desired level. However, even to obtain ``toy'' examples seems to be rather difficult, and we are not aware of any such models.
%
% In this paper, we answer the above question by introducing a family of point processes, indexed by a parameter $\a>0$, such that for different values of $\a$  there is a different rigidity behaviour. These are also Gaussian analytic functions, albeit with different scaling behaviour of the coefficients from the standard one. In fact, we show that there is a monotonicity in the rigid behaviour with respect to the parameter $\a$: for $\frac{1}{k} < \a \le \frac{1}{k-1}$ (where $k \ge 0$ is an integer), the resulting point process is rigid at level $k$. For the special case $\a=1/2$, we recover the standard planar GAF. We call this family of Gaussian analytic functions as $\a$-GAF, which we formally define as follows:
%
% \begin{definition}
%  For a real number $\a>0$, we define the $\a$-GAF \[f_\a(z)=\sum_{k=0}^\infty \frac{\xi_k}{(k!)^{\a/2}}z^k.\]
% \end{definition}

% This enables us to state
% \begin{theorem}
%  \label{hierig}
%  The $\a$-GAF zero process is rigid at level $k \ge 1$ whenever $\a \in (\frac{1}{k} , \frac{1}{k-1}]$.
% \end{theorem}

%%  It is natural to ask whether one can study continuum percolation on the $\a$-GAF zero processes on similar lines to \cite{GKP}. Letus mention prove existence of a (non-trivial) critical radius for continuum percolation on the $\a$-GAF zero process, and whether it is possible to establish uniqueness of the infinite cluster in the supercritical regime
%
% Another natural question which arises with regard to rigidity phenomena is the following. In a determinantal point process (henceforth abbreviated as d.p.p.) with a kernel $K$ and a background measure $\mu$, all information about the process is contained, in principle, in the pair $(K,\mu)$. So, it is natural to ask whether it is possible to read off information about the rigidity behaviour of determinantal processes by looking at their kernel. We provide a partial answer to this question by specifying conditions on the pair $(K,\mu)$ which mandate a certain rigidity behaviour of the determinantal process.
%
% To state this result, recall that the necessary and sufficient condition (due to Machchi and Soshnikov) for the pair $(K,\mu)$ to be the kernel and background measure of a determinantal point process is that $K$ gives rise to a non-negative contraction when looked upon in the natural way as the kernel of an integral operator acting on $L^2(\mu)$. Then we have the following connection between rigidity and the kernel:
%
% \begin{theorem}
%  \label{detrig}
%  Let $\Pi$ be a determinantal point process with kernel $K$ and background measure $\mu$. Then $\Pi$ exhibits rigidity in the number of points in a domain only if $K$ is a projection operator on $L^2(\mu)$.
% \end{theorem}

% It is an interesting question to ask whether converse of Theorem \ref{detrig} is true. In other words, if the kernel $K$ yields a projection operator on $L^2(\mu)$, then is the resulting determinantal process rigid (in terms of the number of points in a domain). However, such a statement is not true in complete generality. A counter-example is provided by the zeroes of the hyperbolic Gaussian analytic function of intensity 1. It is a determinantal point process whose kernel is the projection on to the Bargmann spacee of $L^2$ analytic functions on the unit disk. It has been shown to be insertion and deletion tolerant in \cite{HS}; in particular, it does not exhibit rigidity of the number of points in any domain. However, this is an example where the ambient space (the hyperbolic plane) is non-Euclidean, in particular it is non-amenable. This still leaves open the question of whether a determinantal point process on a Euclidean space given by a projection kernel is necessarily rigid (in terms of the number of points), or more generally, what can be said about the rigidity  properties of such point processes.
%
% In Section \ref{radialmeasures}, we consider determinantal point processes on $\C$ with a sesqui-holomorphic kernel $K(z,w)$ (that is holomorphic in $z$ and conjugate-holomorphic in $w$).  Further, we will assume that $\gamma$ is a radial measure with $\mu$ being the measure on the non-negative real line induced by $|Z|^2$ (where $Z  \sim \gamma$), that $\mu$ has all moments finite, and let \[c_j^{-1}= \int_0^\infty r^j d\mu(r).\] We will focus on the case where the kernel has the structure \[K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j .\] The last identity implies that $K$ is a reproducing kernel, projecting on to the subspace of $L^2(\gamma)$ gererated by the polynomials.

% This is an interesting family of d.p.p.-s (parametrized by the measure $\gamma$), encompassing the zeroes of the hyperbolic GAF with unit intensity on one hand (where $\gamma$ is the uniform measure on the unit disk), and the Ginibre ensemble on the the other (where $\gamma$ equals the standard Gaussian measure on the complex plane). It is known that the rigidity properties of these two ensembles are very different - while the hyperbolic GAF is tolerant to insertion and deletion of points (\cite{HS}), the Ginibre ensemble exhibits rigidity at level 1.
%
% We investiage this family of d.p.p.-s with respect to rigidity behavious. Interestingly, a rough dichotomy emerges - when $\gamma$ is compactly supported (along with some additional conditions), the d.p.p. does not exhibit rigidity, whereas, when $\gamma$ belongs to a fairly wide class of measures that have unbounded support (that includes the Gaussian and related measures), the d.p.p. is rigid at level 1. Technically, these conditions on the measures can be articulated in terms of the various moments of $\mu$.
%
% Before stating the theorems, we introduce some further notations. Let $\Gamma_j$ be the size biasing of $\mu$ of the order $j$; in other words, $\Gamma_j$ has a density which is proportional to $r^jd\mu(r)$. Let \[\mu_j:=\E[\Gamma_j]=c_j/c_{j+1},\] \[\sigma_j:=\E\l[\l(\frac{\Gamma_j}{\mu_j}-1\r)^2\r]=\l(\frac{\mu_{j+1}}{\mu_j}-1\r)\] and  \[\nu_j := \E\l[  \l(\frac{\Gamma_j}{\mu_j}-1\r)^4\r]= \l( \frac{\mu_{j+3}\mu_{j+2}\mu_{j+1}}{\mu_j} - 4 \frac{\mu_{j+2} \mu_{j+1}}{\mu_j^2} + 6 \frac{\mu_{j+1}}{\mu_j} -3 \r).\]
%
% In the setting described above, we can state the following theorems:
% \begin{theorem}
% \label{compact}
%Suppose that $\sum_{j=1}^{\infty}\sigma_j < \infty$. Then the process $\mathbb{X}$ does not exhibit rigidity of numbers.
%\end{theorem}
%
% and
%
% \begin{theorem}
% \label{dpprt}
%Let the measure $\mu$ be such that it satisfies the following growth conditions:
%\begin{itemize}
% \item $\sum_{j=1}^{\infty}\nu_j<\infty. $
% \item $\sum_{j=1}^{k} \mu_j^4 \nu_j= o(\mu_k^4).  $
%\end{itemize}
%Then the determinantal point process $\mathbb{X}$ is rigid with respect to the number of points in a bounded domain.
%If, in addition, we have the measure $\gamma$ absolutely continuous w.r.t. the Lebesgue measure on $\C$, and that for some integer $a \ge 1$
%\begin{itemize}
% \item $\sum_{j=1}^{\infty}\mu_j^{-a}<\infty$,
%\end{itemize}
%then the point process  $\mathbb{X}$ is in fact rigid at level 1.
%\end{theorem}

%\begin{remark}
% The assumption of absolute continuity on the measure $\gamma$ is somewhat superfluous, and is there purely to invoke the definition of tolerance, which rules out arbitrary measures. However, for rigidity at level 1, one can adopt a slightly wider notion of tolerance, by demanding that the point process inside a bounded open $\D$ is mutually absolutely continuous with respect to the point process of $N(\D)$ intependent points sampled from $d\gamma^{\otimes N(\D)}$. The proof of tolerance shows that this more general notion of tolerance is also valid in the case at hand.
%\end{remark}

%
%A key class of measures $\mu$ which satisfies the conditions in Theorem \ref{compact} is the one where we have the following asymptotic expansion for $m_j$:
%\[ \mu_j=A+\frac{B}{j} + O(1/j^2) .\]
%Included in this class of measures are all measures $\mu$ such that $\mu$ is compactly supported and has a positive density in a neighbourhood of the maximal end of its support, which incorporates the important case of uniform measures on disks.

%An important class of measures which satisfies the criteria in Theorem \ref{dpprt} are those which exhibit the following asymptotics, for some constants $C,A,\a$: \[\mu_j:=\E[\Gamma_j]=Cj^\a\l(1+\frac{A}{j} + O(\frac{1}{j^2})\r).\]
%In other words, we stipulate a power law for the means of the size biased measures $\Gamma_j$. This covers the case of all measures of the form $d\mu(r)=r^\beta e^{-r^\gamma}dr$, which includes the Ginibre ensemble.

%While Theorems \ref{compact} and \ref{dpprt} encompass the known and important examples of relevant d.p.p.-s, it would be definitely very interesting to sharpen the dichotomy presentes in these two theorems. In particular, would it be possible to extend this dichotomy and establish that it is indeed the compactness or the non-compactness of the measure $\gamma$ that determines the rigidity behaviour of the d.p.p.

%An interesting point process on $\R$ for which rigidity phenomena has been considered is the case of the sine kernel process. Indeed, it has been shown in \cite{G-I} that this point process has rigidity of the number points. It turns out that this is the only rigid statistic for the sine process, in other words, the sine process is rigid of order 1. The proof of tolerance, subject to the constraint on the number of points, is on similar lines to the proof of tolerance for the Ginibre ensemble in \cite{GP} and the proof of tolerance in Theorem \ref{dpprt}. Accordingly, we will address the proof in the supplementary note \cite{}. For now, we simply record the fact as:
%\begin{theorem}
% \label{sintol}
% The sine kernel process on $\R$ is rigid at level 1.
%\end{theorem}

%
%Finally, in Section \ref{lattice}, we consider the  point process obtained by Gaussian perturbations of $\Z$. For an i.i.d. perturbation of $\Z$, it can be shown that the resulting point process is rigid at level 1; for this the perturbing variable does not need to be Gaussian, finite variance is enough. This is similar to the situation for i.i.d. lattice perturbations of $\Z^2$. On the other hand, for i.i.d. perturbations in dimensions $d \ge 3$, it is known (\cite{PS}) that there is a phase transition in the variance of the perturbing Gaussian: there is a critical $\sigma_c$ such that for variance bigger than $\sigma_c^2$, the process is insertion tolerant (to be defined below), while for variance less than $\sigma_c^2$ it is rigid (at level 1). We call a point process $\X$ on a Euclidean space insertion tolerant, if, given any bounded domain $D$ and the point configuration  $ \X$ we can introduce a new point in $D$ and still remain in the support of $\X$.  In particular, this implies that there is no rigidity of numbers in $\X$.

%In dimension 1, when the tails of the Gaussians become progressively heavier, the rigidity phenomena presents an interesting study. If we posit a power law growth for the variances of the perturbations, we obtain a phase transition in the rigidity behaviour of Gaussian perturbations of $\Z$ as follows:

%\begin{theorem}
% \label{power}
% Consider the point process $\X$ on $\R$ which is the random point set given by $\{k+Z_k: k \in \Z, Z_k \text{ independent } N(0,\sigma_\beta(k)) \}$, where $\sigma_\beta(k) = |k|^\beta$. Then $\X$ is insertion tolerant if $\beta>1/2$, and is rigid (at level 1) if $\beta \le 1/2$.
%\end{theorem}

%


==> Revised manuscript/nonprojectiondpp.tex <==
\section{Proof of Theorem~\ref{detrig}: Non-projection determinantal processes are tolerant}
We first sketch the basic idea, and then move on to the proof. Consider a  kernel of the form $K(x,y)=\sum_{j\ge 1}\la_{j}\ph_{j}(x)\bar{\ph}_{j}(y)$ where $0\le \la_{j}\le 1$ and $\ph_{j}$ are orthonormal in $L^{2}(\mu)$. Let $I_{j}$ be independent Bernoulli random variables with $\P\{I_{j}=1\}=\la_{j}$, and define $K_{I}(x,y)=\sum_{j\ge 1}I_{j}\ph_{j}(x)\bar{\ph}_{j}(y)$. If we sample $I_{j}$s first and then a determinantal point process with kernel $K_{I}$, the resulting process is precisely the determinantal point process with kernel $K$ (see Thereom~4.5.3 in \cite{HKPV}). In particular, if $0<\la_{j}<1$ for at least one $j$, then the  number of points in the point process is a non-constant random variable,  or it is almost surely infinite. For the special case when the expected number of points $\sum_j\lambda_j<\infty$, this shows that rigidity fails even when $D=\Xi$ (also see   Lemma~\ref{lem:inclusion}).


%For the simple case when the expected number of points $\sum_j\lambda_j<\infty$, this shows that if we condition on $N_{D^c}(\Pi)=0$ (which happens with positive probability for large enough $D$), then $N_D(\Pi)$ cannot be determined. }

In general, $K$ (rather, its associated operator $\mathcal K$) may have a continuous spectrum and hence we cannot write an expansion as above. However, we can write the kernel $K$ as a convex combination of two projection kernels and extend the above idea to show that the determinantal process with kernel $K$ is a mixture of two determinantal processes. From this, we can deduce that the given determinantal process does not have rigidity of numbers. The essential observation is that the proof of Theorem~4.5.3 in \cite{HKPV} referred to above, does not require $\ph_{j}$s to be orthogonal.

%We fix a  Radon measure $\mu$ on $\Xi$ and express all joint intensities with respect to $\mu$. Suppose $L-K=\la\phi\phi^{*}$ where $K,L$ are hermitian, locally trace-class, sub-projection kernels and $\phi$ is a unit vector in $L^{2}(\mu)$. Assume that $\Pi_{K}$ 

%
%Even if we do not assume that $\phi$ is orthogonal to $K$, under some conditions we can construct DPP($L$) as a mixture of the determinantal point processes DPP($K$) and DPP($K+\phi \phi^{*}$).


\begin{proof}[Proof of Theorem \ref{detrig}]
Let $K$ be a locally trace-class, Hermitian, contraction kernel on $L^{2}(\Xi,\mu)$ which is not a projection. Then, the corresponding integral operator  $\mathcal K=\int_{0}^{1}\la dE(\la)$ where the projection-valued measure $E$ has the property that $E[\del,1-\del]\not=0$ for some $\del>0$. 

Let $f$ be in the range of $E[\del,1-\del]$ with $\|f\|^{2}=\del$ (norms in $L^{2}(\mu)$). Let 
\begin{align*}
L_{0}(x,y)=K(x,y)-\half f(x)\bar{f}(y)\;\;\;\mb{ and } \;\;\; L_{1}(x,y)=K(x,y)+ \half f(x)\bar{f}(y).
\end{align*} 
Let $\mathcal L_{0}$ and $\mathcal L_{1}$ be the associated operators.

Since $\mathcal K$ is locally of trace-class and Hermitian and $f\in L^{2}(\mu)$, it follows that $\mathcal L_{0}$ and $\mathcal L_{1}$ are also locally of trace-class and Hermitian. Further, by the choice of $f$, it follows that they are contraction kernels on $L^{2}(E,\mu)$, i.e., $0\le \mathcal L_{0}\le I$ and $0\le \mathcal L_{1}\le I$. To see this, let $P_{\del}$ denote the spectral projection $E[\del,1-\del]$ and let $f\otimes f^{*}$ denote the operator on $L^{2}(\mu)$ that maps $\psi$ to $\langle \psi,f \rangle f$. Then $f\otimes f^{*}\le \del P_{\del}$ (in the positive definite order) and $\del P_{\del}\le \mathcal K\le (1-\del)P_{\del}$. Therefore, 
\begin{align*}
\mathcal L_{0}=(K-\frac12 f\otimes f^{*})\ge\frac12 \del P_{\del}, \\
 \mathcal L_{1}=(K+\frac12 f\otimes f^{*})\le (1-\frac12 \del)P_{\del}.
\end{align*}
This shows that $\mathcal L_{0}$ and $\mathcal L_{1}$ are positive contractions and hence, by the theorem of Macchi and Soshnikov (see the discussion preceding the statement of Theorem~\ref{detrig}), there exist determinantal processes $\Pi_{0}$ and $\Pi_{1}$ with kernels $L_{0}$ and $L_{1}$, respectively.

By a result tracing back to Lyons, we may construct $\Pi_{0}$ and $\Pi_{1}$ on the same probability space such that every point of  $\Pi_{0}$ is also a point of $\Pi_{1}$, along with a  Bernoulli$(1/2)$ random variable $\xi$ that is independent of $\Pi_{0}$ and $\Pi_{1}$.  For Lyons' original result (applicable to the case when $\Xi$ is a countable set),  see Theorem~6.2 of \cite{Ly}. For  more recent versions that address the general case, we refer the reader to  \cite{Tripathi, Lyons-ICM}. The  result in the general setting can, in fact,  be obtained from Lyon's original result for the countable case via the so-called \textit{Goldman's transference principle} \cite{Go}.

 As $\mathcal L_{1}-\mathcal L_{0}=f\otimes f^{*}$ has rank one, in view of the above coupling there is at most one point in $\Pi_{1}$ that is not in $\Pi_{0}$. Define
\[
\Pi=\begin{cases}
\Pi_{0} &\mb{ if }\xi=0, \\ \Pi_{1} &\mb{ if }\xi=1.
\end{cases}
\]
We claim that $\Pi$ is a determinantal point process with kernel $K$. To show this, fix $k\ge 1$ and $x_{1},\ldots ,x_{k}\in E$ and let  $M=\l(L_{0}(x_{i},x_{j})\r)_{i,j\le k}$ and $\uu^{t}=(f(x_{1}),\ldots ,f(x_{k}))$. Then, $\l(L_{1}(x_{i},x_{j})\r)_{i,j\le k}=M+\uu \uu^{*}$. Hence, $\Pi$ has $k$-point intensity given by
\begin{align*}
p_{k}(x_{1},\ldots ,x_{k}) &= \half \det\l( L_{1}(x_{i},x_{j})\r)_{i,j\le k} + \half \det\l( L_{0}(x_{i},x_{j})\r)_{i,j\le k} \\
&= \frac12 \det(M+\uu \uu^{*})+\frac12 \det(M) \\
&= \half \det(M)\l(1+ \uu^{*} M^{-1} \uu \r) + \half \det(M)\\
&=  \det(M)\l(1+\half \uu^{*} M^{-1} \uu \r) \\
&= \det\l(M+\half \uu \uu^{*}\r)
\end{align*}
which is precisely  $\det(K(x_{i},x_{j}))_{i,j\le k}$. This proves the claim.

Now, there exists a pre-compact set $D$ such that $\P\{\Pi_{1}\setminus \Pi_{0} \subseteq D\}>0$. On this event, $\Pi_{0}, \Pi_{1},\Pi$, all agree on $D^{c}$ but inside $D$, $\Pi_{1}$ has one point more than $\Pi_{0}$. Condition on the configuration $\Pi_{D^{c}}$. Depending on the value of $\xi$, the number of points of $\Pi$ inside $D$ can take two different values, each with positive probability (for a positive probability of configurations outside $D$).  This proves that $\Pi$ cannot have rigidity of numbers.
\end{proof}



%We end this section with a formal definition of Palm measures of a point process. For a more detailed treatment, we refer the reader to \cite{Ka} Chapter 10 . 
%\begin{definition} \label{def:Palm}
%Let $\Pi$ be a point process on the space $X$,  let $\mathcal{S}$ denote the Polish space of all locally finite point configurations on $X$,  $\mathcal{B}(X)$ denote the Borel sigma field on $\mathcal{S}$ and $\rho_1$ denote the one-point intensity measure of $\Pi$. Let $F : X \times \mathcal{S} \mapsto \R$ be a test function. Then, for $s \in X$, the Palm measure  $\Pi_s$ at $s$ is defined by  
%$\E_\Pi \l[ \sum_{s \in \Pi} F(s,\Pi) \r] = \int_X \E_{\Pi_s} \l[  F(s,\Pi_s) \r] \mathrm{d}\rho_1(s)$.
%\end{definition}




%
%Indeed, if $P_\del$ denotes the the spectral projection $E[\del,1-\del]$ and $P_{\del'}$ the projection on to its orthogonal complement, then  for any $\psi \in L^2(\mu)$ we have \[ \langle \psi, L_0 \psi \rangle = \langle P_{\del'} \psi, K P_{\del'} \psi   \rangle + \langle P_{\del} \psi, \l(K - \frac{1}{2}ff^{*}\r) P_\del \psi \rangle.   \] By construction, $P_\del \l(K - \frac{1}{2}ff^{*}\r) P_\del \ge 0$ as an operator, since $f$ is in the range of $P_\del$ with norm $\del$, and $P_\del K P_\del \ge \del \text{Id}$. Hence the right hand side of the above display is non-negative, thereby proving that $L_0 \ge 0$ as an operator. Similarly, it can be seen that $L_1 \ge 0$.

%Let $\mathcal X_{0}$ and $\mathcal X_{1}$ be determinantal processes with kernels $L_{0}$ and $L_{1}$, respectively, coupled so that $\mathcal X_{0}\subseteq \mathcal X_{1}$. Let $\xi\sim \textbf{Ber}(1/2)$ be independent of $\mathcal X_{0}$ and $\mathcal X_{1}$. Then, define
%$$
%\mathcal X = \begin{cases} \mathcal X_{0} & \textbf{ if }\xi=0, \\ \mathcal X_{1} & \textbf{ if } \xi=1.\end{cases}
%$$
%We claim that $\mathcal X$ is determinantal with kernel $K$. To show this, fix $k\ge 1$ and $x_{1},\ldots x_{k}\in E$ and let  $M=\l(L_{0}(x_{i},x_{j})\r)_{i,j\le k}$ and $\u^{t}=(f(x_{1}),\ldots ,f(x_{k}))$. Then, $\mathcal X$ has $k$-point intensity given by
%\begin{align*}
%p_{k}(x_{1},\ldots ,x_{k}) &= \half \det\l( L_{1}(x_{i},x_{j})\r)_{i,j\le k} + \half \det\l( L_{0}(x_{i},x_{j})\r)_{i,j\le k} \\
%&= \half \det(M)\l(1+ \u^{*} M^{-1} \u \r) + \half \det(M)\\
%&=  \det(M)\l(1+\half \u^{*} M^{-1} \u \r) \\
%&= \det\l(M+\half \u \u^{*}\r)
%\end{align*}
%which is precisely  $\det(K(x_{i},x_{j}))_{i,j\le k}$. This proves the claim.

%Now, there exists a compact set $A$ such that $\P\{\mathcal X_{1} \setminus \mathcal X_{0} \subseteq A\}>0$. On this event, $\mathcal X_{0}, \mathcal X_{1},\mathcal X$, all agree on $A^{c}$ but the second one has one more point than the first inside $A$. Condition on the configuration $\mathcal X|_{A^{c}}$. Depending on the value of $\xi$, the number of points of $\mathcal X$ inside $A$ can take two different values, each with positive probability (for a positive probability of configurations outside $A$). 

%


==> Revised manuscript/nonprojectiondpp_1.tex <==
\section{Proof of Theorem~\ref{detrig}: Non-projection determinantal processes are tolerant}
We sketch the basic idea. Consider a  kernel of the form $K(x,y)=\sum_{j\ge 1}\la_{j}\ph_{j}(x)\bar{\ph}_{j}(y)$ where $0\le \la_{j}\le 1$ and $\ph_{j}$ are orthonormal in $L^{2}(\mu)$. Let $I_{j}$ be independent Bernoulli random variables with $\P\{I_{j}=1\}=\la_{j}$, and define $K_{I}(x,y)=\sum_{j\ge 1}I_{j}\ph_{j}(x)\bar{\ph}_{j}(y)$. If we sample $I_{j}$s first and then a determinantal point process with kernel $K_{I}$, the resulting process is precisely the determinantal point process with kernel $K$ (see Thereom~4.5.3 in \cite{HKPV}). In particular, if $0<\la_{j}<1$ for at least one $j$, then the  number of points in the point process is a non-constant random variable.

In general, $K$ (rather, its associated operator $\mathcal K$) may have a continuous spectrum and hence we cannot write an expansion as above. However, we can write the kernel $K$ as a convex combination of two projection kernels and extend the above idea to show that the determinantal process with kernel $K$ is a mixture of two determinantal processes. From this, we can deduce that the given determinantal process does not have rigidity of numbers. The essential observation is that the proof of Theorem~4.5.3 in \cite{HKPV} referred to above, does not require $\ph_{j}$s to be orthogonal.

%We fix a  Radon measure $\mu$ on $\Xi$ and express all joint intensities with respect to $\mu$. Suppose $L-K=\la\phi\phi^{*}$ where $K,L$ are hermitian, locally trace-class, sub-projection kernels and $\phi$ is a unit vector in $L^{2}(\mu)$. Assume that $\Pi_{K}$ 

%
%Even if we do not assume that $\phi$ is orthogonal to $K$, under some conditions we can construct DPP($L$) as a mixture of the determinantal point processes DPP($K$) and DPP($K+\phi \phi^{*}$).


\begin{proof}[Proof of Theorem \ref{detrig}]
Let $K$ be a locally trace-class, Hermitian, contraction kernel on $L^{2}(\Xi,\mu)$ which is not a projection. Then, the corresponding integral operator  $\mathcal K=\int_{0}^{1}\la dE(\la)$ where the projection-valued measure $E$ has the property that $E[\del,1-1\del]\not=0$ for some $\del>0$. 

Let $f$ be in the range of $E[\del,1-\del]$ with $\|f\|^{2}=\del$ (norms in $L^{2}(\mu)$). Let 
\begin{align*}
L_{0}(x,y)=K(x,y)-\half f(x)\bar{f}(y)\;\;\;\mb{ and } \;\;\; L_{1}(x,y)=K(x,y)+ \half f(x)\bar{f}(y).
\end{align*} 
Let $\mathcal L_{0}$ and $\mathcal L_{1}$ be the associated operators.

Since $\mathcal K$ is locally of trace-class and Hermitian and $f\in L^{2}(\mu)$, it follows that $\mathcal L_{0}$ and $\mathcal L_{1}$ are also locally of trace-class and Hermitian. Further, by the choice of $f$, it follows that they are contraction kernels on $L^{2}(E,\mu)$, i.e., $0\le \mathcal L_{0}\le I$ and $0\le \mathcal L_{1}\le I$. To see this, let $P_{\del}$ denote the spectral projection $E[\del,1-\del]$ and let $f\otimes f^{*}$ denote the operator on $L^{2}(\mu)$ that maps $\psi$ to $\langle \psi,f \rangle f$. Then $f\otimes f^{*}\le \del P_{\del}$ (in the positive definite order) and $\del P_{\del}\le \mathcal K\le (1-\del)P_{\del}$. Therefore, 
\begin{align*}
\mathcal L_{0}=(K-\frac12 f\otimes f^{*})\ge\frac12 \del P_{\del}, \\
 \mathcal L_{1}=(K+\frac12 f\otimes f^{*})\le (1-\frac12 \del)P_{\del}.
\end{align*}
This shows that $\mathcal L_{0}$ and $\mathcal L_{1}$ are positive contractions and hence, by the theorem of Macchi and Soshnikov (see the discussion preceding the statement of Theorem~\ref{detrig}), there exist determinantal processes $\Pi_{0}$ and $\Pi_{1}$ with kernels $L_{0}$ and $L_{1}$, respectively.

By a result of Lyons (see Theorem~6.2 of \cite{Ly} for the case when $\Xi$ is a countable set), we may construct $\Pi_{0}$ and $\Pi_{1}$ on the same probability space such that every point of  $\Pi_{0}$ is also a point of $\Pi_{1}$. As $\mathcal L_{1}-\mathcal L_{0}=f\otimes f^{*}$ has rank one, there is at most one point in $\Pi_{1}$ that is not in $\Pi_{0}$. along with a  Bernoulli$(1/2)$ random variable $\xi$ that is independent of $\Pi_{0}$ and $\Pi_{1}$. Define
\[
\Pi=\begin{cases}
\Pi_{0} &\mb{ if }\xi=0, \\ \Pi_{1} &\mb{ if }\xi=1.
\end{cases}
\]
We claim that $\Pi$ is a determinantal point process with kernel $K$. To show this, fix $k\ge 1$ and $x_{1},\ldots ,x_{k}\in E$ and let  $M=\l(L_{0}(x_{i},x_{j})\r)_{i,j\le k}$ and $\uu^{t}=(f(x_{1}),\ldots ,f(x_{k}))$. Then, $\l(L_{1}(x_{i},x_{j})\r)_{i,j\le k}=M+\uu \uu^{*}$. Hence, $\Pi$ has $k$-point intensity given by
\begin{align*}
p_{k}(x_{1},\ldots ,x_{k}) &= \half \det\l( L_{1}(x_{i},x_{j})\r)_{i,j\le k} + \half \det\l( L_{0}(x_{i},x_{j})\r)_{i,j\le k} \\
&= \frac12 \det(M+\uu \uu^{*})+\frac12 \det(M) \\
&= \half \det(M)\l(1+ \uu^{*} M^{-1} \uu \r) + \half \det(M)\\
&=  \det(M)\l(1+\half \uu^{*} M^{-1} \uu \r) \\
&= \det\l(M+\half \uu \uu^{*}\r)
\end{align*}
which is precisely  $\det(K(x_{i},x_{j}))_{i,j\le k}$. This proves the claim.

Now, there exists a pre-compact set $D$ such that $\P\{\Pi_{1}\setminus \Pi_{0} \subseteq D\}>0$. On this event, $\Pi_{0}, \Pi_{1},\Pi$, all agree on $D^{c}$ but inside $D$, $\Pi_{1}$ has one point more than $\Pi_{0}$. Condition on the configuration $\Pi_{D^{c}}$. Depending on the value of $\xi$, the number of points of $\Pi$ inside $D$ can take two different values, each with positive probability (for a positive probability of configurations outside $D$).  This proves that $\Pi$ cannot have rigidity of numbers.
\end{proof}
%
%Indeed, if $P_\del$ denotes the the spectral projection $E[\del,1-\del]$ and $P_{\del'}$ the projection on to its orthogonal complement, then  for any $\psi \in L^2(\mu)$ we have \[ \langle \psi, L_0 \psi \rangle = \langle P_{\del'} \psi, K P_{\del'} \psi   \rangle + \langle P_{\del} \psi, \l(K - \frac{1}{2}ff^{*}\r) P_\del \psi \rangle.   \] By construction, $P_\del \l(K - \frac{1}{2}ff^{*}\r) P_\del \ge 0$ as an operator, since $f$ is in the range of $P_\del$ with norm $\del$, and $P_\del K P_\del \ge \del \text{Id}$. Hence the right hand side of the above display is non-negative, thereby proving that $L_0 \ge 0$ as an operator. Similarly, it can be seen that $L_1 \ge 0$.

%Let $\mathcal X_{0}$ and $\mathcal X_{1}$ be determinantal processes with kernels $L_{0}$ and $L_{1}$, respectively, coupled so that $\mathcal X_{0}\subseteq \mathcal X_{1}$. Let $\xi\sim \textbf{Ber}(1/2)$ be independent of $\mathcal X_{0}$ and $\mathcal X_{1}$. Then, define
%$$
%\mathcal X = \begin{cases} \mathcal X_{0} & \textbf{ if }\xi=0, \\ \mathcal X_{1} & \textbf{ if } \xi=1.\end{cases}
%$$
%We claim that $\mathcal X$ is determinantal with kernel $K$. To show this, fix $k\ge 1$ and $x_{1},\ldots x_{k}\in E$ and let  $M=\l(L_{0}(x_{i},x_{j})\r)_{i,j\le k}$ and $\u^{t}=(f(x_{1}),\ldots ,f(x_{k}))$. Then, $\mathcal X$ has $k$-point intensity given by
%\begin{align*}
%p_{k}(x_{1},\ldots ,x_{k}) &= \half \det\l( L_{1}(x_{i},x_{j})\r)_{i,j\le k} + \half \det\l( L_{0}(x_{i},x_{j})\r)_{i,j\le k} \\
%&= \half \det(M)\l(1+ \u^{*} M^{-1} \u \r) + \half \det(M)\\
%&=  \det(M)\l(1+\half \u^{*} M^{-1} \u \r) \\
%&= \det\l(M+\half \u \u^{*}\r)
%\end{align*}
%which is precisely  $\det(K(x_{i},x_{j}))_{i,j\le k}$. This proves the claim.

%Now, there exists a compact set $A$ such that $\P\{\mathcal X_{1} \setminus \mathcal X_{0} \subseteq A\}>0$. On this event, $\mathcal X_{0}, \mathcal X_{1},\mathcal X$, all agree on $A^{c}$ but the second one has one more point than the first inside $A$. Condition on the configuration $\mathcal X|_{A^{c}}$. Depending on the value of $\xi$, the number of points of $\mathcal X$ inside $A$ can take two different values, each with positive probability (for a positive probability of configurations outside $A$). 

%


==> Revised manuscript/perturbedlattice.tex <==
\section{Perturbed lattice in one dimension}
\label{lattice}
Consider $\Pi=\{X_{k} \ : \ k\in \Z\}$ where $X_{k}\sim N(k,\sigma_{k}^{2})$ are independent random variables. We want to consider the special case of $\sigma_{k}^{2}=k^{2\beta}$ and understand the issue of rigidity and tolerance, depending on the parameter $\beta$.

\underline{${\beta>1/2: }$}

For simplicity of notation, we work with perturbed $\N$, i.e., $\{X_{k}\text{ such that } k\ge 1\}$. The proof for the case of $\Z$ (instead of $\N$) is similar. Let $\mu=\mathcal L(X_{1},X_{2},\ldots)$ and $\nu=\mathcal L(X_{2},X_{3},\ldots)$, where by the notation $\mathcal{L}(\underline{Y})$ we denote the law of the random sequence $\underline{Y}$. We claim that $\mu$ and $\nu$ are mutually absolutely continuous and hence, the process $\Pi$ is insertion tolerant (that is, given any bounded domain $D$ and the point configuration  $ \Pi$ we can introduce a new point in $D$ and still remain in the support of $\Pi$). In particular, this implies that there is no rigidity of numbers in $\Pi$. To see this, note that the function mapping the sequence $(X_1,X_2,\cdots,\infty)$ to the point set $\{X_1,X_2\cdots,\infty\}$ is measurable, hence $\mu \equiv \nu$ implies $\Pi \equiv \widetilde{\Pi}$ (where $\widetilde{\Pi}$ is the point process corresponding to $(X_2,\cdots,\infty)$), hence these have the same support. But by a trivial coupling, $\Pi$ contains one more point than the corresponding realization of $\widetilde{X}$, which (being a Gaussian perturbation of $1$) could be inside any given interval in $\R$ with positive probability . Since the distributions of $\Pi$ and $\widetilde{X}$ have the same support, we conclude that the point process $\Pi$ is insertion tolerant in the sense described above.

To compare $\mu$ and $\nu$, we will invoke Kakutani's Dichotomy Theorem. Fix $k$ and let $\mu=k$, $\mu'=k+1$, $\sigma=k^{\beta}$ and $\sigma'=(k+1)^{\beta}$. Then, the Radon-Nikodym derivative of $X_{k}$ to $X_{k+1}$ is
\begin{align*}
f_{k}(x) &= \frac{\sigma'}{\sigma}\exp\l\{-\half\l[\frac{(x-\mu)^{2}}{\sigma^{2}}-\frac{(x-\mu')^{2}}{\sigma'^{2}} \r]\r\}.
\end{align*}
Therefore,
\begin{align*}
\int \sqrt{f_{k}}d\nu &= \sqrt{\frac{\sigma'}{\sigma}}\frac{1}{\sigma'\sqrt{2\pi}}\int \exp\l\{-\frac{1}{4}\l[\frac{(x-\mu)^{2}}{\sigma^{2}}-\frac{(x-\mu')^{2}}{\sigma'^{2}} \r]\r\} \exp\l\{-\half \frac{(x-\mu')^{2}}{\sigma'^{2}}\r\} dx \\
&= \frac{1}{\sqrt{\sigma\sigma'} \sqrt{2\pi}} \int \exp\l\{-\frac{1}{4}\l[\frac{(x-\mu)^{2}}{\sigma^{2}}+\frac{(x-\mu')^{2}}{\sigma'^{2}} \r]\r\} dx \\
&= \frac{1}{\sqrt{\sigma\sigma'} \sqrt{2\pi}} \int \exp\l\{-\frac{1}{4\sigma^{2}\sigma'^{2}}(ax^{2}+bx+c)\r\}dx
\end{align*}
where $a=\sigma^{2}+\sigma'^{2}$, $b=-2\mu\sigma'^{2}-2\mu'\sigma^{2}$ and $c=\mu^{2}\sigma'^{2}+\mu'^{2}\sigma^{2}$. Note that $\int e^{-\half(Ax^{2}+Bx+C)}dx = \sqrt{\frac{2\pi}{A}}e^{(B^{2}-4AC)/2A}$. In our case, $A=a/2\sigma^{2}\sigma'^{2}$, $B=b/2\sigma^{2}\sigma'^{2}$ and $C=c/2\sigma^{2}\sigma'^{2}$ and hence
\begin{align*}
\int \sqrt{f_{k}}d\nu &= \frac{1}{\sqrt{\sigma\sigma'}\sqrt{2\pi}}\frac{\sqrt{2\pi}\sqrt{2\sigma^{2}\sigma'^{2}}}{\sqrt{a}}\exp\l\{-\frac{(\mu-\mu')^{2}}{\sigma^{2}+\sigma'^{2}}\r\} \\
&= \sqrt{\frac{2\sigma\sigma'}{\sigma^{2}+\sigma'^{2}}}\exp\l\{-\frac{(\mu-\mu')^{2}}{\sigma^{2}+\sigma'^{2}}\r\} \\
&= \sqrt{1-\frac{(\sigma-\sigma')^{2}}{\sigma^{2}+\sigma'^{2}}}\exp\l\{-\frac{(\mu-\mu')^{2}}{\sigma^{2}+\sigma'^{2}}\r\}.
\end{align*}
Plugging the values of $\mu=k$, $\sigma=k^{\beta}$ etc., we get
\begin{align*}
\int \sqrt{f_{k}}d\nu &= \sqrt{1-O\l(\frac{1}{k^{2}}\r)}\exp\l\{-O\l(\frac{1}{k^{2\beta}}\r)\r\}
\end{align*}
from which it immediately follows that $\prod_{k}(\int \sqrt{f_{k}}d\nu) >0$. By Kakutani's Theorem, $\mu \equiv \nu$.

% [{\bf Remark}: It appears that the martingale is not $L^{p}$ bounded for any $p>1$ and so I could not bypass Kakutani's theorem to get a direct proof of uniform integrability. It is crucial here that we got $1-O(k^{-2})$ and not $1-O(k^{-1})$].

% Similar calculation ought to show that $\nu\ll \mu$ (xxneed to check $\prod \int\sqrt{1/f_{k}}d\mu$, check thisxx).



\underline{${\beta \le 1/2: }$}

For a compactly supported test function $h$, let $h_{L}(x)=h(x/L)$. Let $\sigma^{2}(h_{L})=\Var(\sum_{x\in \Pi}h_{L}(x))=\sum_{k\in \Z}\Var(h_{L}(X_{k}))$. We shall consider $h $ to be a  non-negative Lipschitz function compactly supported on $[-1,1]$ such that $h \equiv 1$ in a neighbourhood of the origin, and $\|h\|_\infty =1$. Then, $|h_{L}(x)-h_{L}(y)|\le \kappa(h) |x-y|/L$, where $\kappa(h)$ is the Lipschitz constant of $h$. Hence we have
$$
\Var(h_{L}(X_{k}))=\half \E[(h_{L}(X_{k})-h_{L}(Y_{k}))^{2}] \le \frac{\kappa(h)^2}{2L^{2}}\E[(X_{k}-Y_{k})^{2}]=\kappa(h)^2\frac{\sigma_{k}^{2}}{2L^{2}}.
$$
We use this bound for $|k|\le 10L$ and get
\begin{align}\label{eq:boundforupto10L}
\sum_{|k|\le 10L}\Var(h_{L}(X_{k})) \le \frac{\kappa(h)^2}{L^{2}}\sum_{k=1}^{10L}k^{2\beta}  \lesssim \kappa(h)^2 L^{-1+2\beta}.
\end{align}

 For $|k|>10L$, we note that $h_{L}(X_{k})-h_{L}(Y_{k})=0$ unless one of $X_{k}$ or $Y_{k}$ falls in the interval $[-L,L]$. In any case, the difference is bounded by $1$, because we have $0 \le h(x) \le 1$ for any $x$. Hence (for simplicity of notation, let $k$ be positive),
$$
\Var(h_{L}(X_{k}))=\half \E[(h_{L}(X_{k})-h_{L}(Y_{k}))^{2}] \le \P\{|X_{k}-k|\ge k-L\}\le e^{-(k-L)^{2}/2\sigma_{k}^{2}}.
$$
For $k>10L$, we see that $(k-L)^{2}\ge k^{2}/4$ while $\sigma_{k}^{2}=k^{2\beta}\le k$ and hence
\begin{align}\label{eq:boundbeyond10L}
\sum_{|k|>10L}\Var(h_{L}(X_{k})) \le e^{-L/10}.
\end{align}
From \eqref{eq:boundforupto10L} and \eqref{eq:boundbeyond10L} we see that $\sigma^{2}(h_{L})\le C \kappa(h)^2 L^{-1+2\beta}$ (for large enough $L$, depending on $h$).

Suppose we want to prove that the number of points of $\Pi$ in a bounded interval $D \subset \R$ is rigid. For $\eps>0$, we define $h_\eps$ as $\Psi_\eps$ in the proof of Theorem \ref{dpprt} in Section \ref{dpprtproof}. It is easy to see that, for large enough $L$ (depending on $\eps$), $\sigma^{2}(h_{L}) \le c\eps^2$. We can again invoke Theorem 6.2 from \cite{GP} to show that we have the desired rigidity of the number of points in $D$.
%  which goes to zero as $L\to \infty$, by the assumption that $\beta<\half$.

Now fix any interval $[-A,A]$ and condition on $\Pi\cap[-A,A]^{c}$. Find $L$ large enough so that $\sigma^{2}(h_{L})<\eps^{3}$. Coupled with Theorem 6.2 in \cite{GP}, this suffices to establish that the number of points in $A$ is rigid.
% is very small, and then we can predict $\sum_{x\in \Pi\cap[-A,A]}h_{L}(x)$ to an accuracy of $\eps$, with probability at least $1-\eps$. Also, $\sum_{x\in \Pi\cap[-A,A]}h_{L}(x)$ converges to $|\Pi\cap[-A,A]|$ as $L\to \infty$. Thus, we get rigidity for number of points.

%
% \underline{$\mathbf{\beta=\frac{1}{2}: }$}
%
% Again we show rigidity of the number of points in a domain. But the test statistic $h(x)=(1-x)_{+}$ is not good enough since $\sigma^{2}(h_{L})$ is asymptotically a positive constant. Instead, we need statistics whose variance can be made arbitrarily small. For this, fix $p>0$ and let $h(x)=(1-x)_{+}^{p}$. The difference comes in our estimate of $\Var(h_{L}(X_{k}))$ for $|k|<10L$. In that case, if we use the approximate bound  $|h_{L}(X_{k})-h_{L}(Y_{k})|\le |h_{L}'(k)||X_{k}-Y_{k}|$ (xxnot quite right, cannot put the derivative at $k$ but at another point.... An argument needed but should be easyxx) we get $\Var(h_{L}(X_{k}))\le |h_{L}'(k)|^{2} \sigma_{k}^{2}= \frac{\sigma_{k}^{2}}{L^{2}}\l(1-\frac{|k|}{L}\r)_{+}^{2p-2}$. This gives the bound (recall that $\sigma_{k}^{2}=k$)
% $$
% \sum_{|k|\le 10L}\Var(h_{L}(X_{k})) \lesssim \frac{1}{L^{2}}\sum_{k=1}^{L}k\l(1-\frac{k}{L}\r)^{2p-2} \approx \int_{0}^{1}x(1-x)^{2p-2}dx = \frac{1}{2p(2p-1)}.
% $$
% Thus, by choosing $p$ large, and then taking $L$ large, we can make the variance as small as we like. The rest of the argument goes through.

\underline{Strong tolerance for $\beta \le 1/2$:}

By looking at the random sequence $(X_1,X_2,\cdots,\infty)$, we notice that for each realization of the random sequence, the points that occur inside any bounded interval $A$ have a joint density (coming from the Gaussians). Hence could be in any other possible locations in $A$ (w.r.t. the Lebesgue measure) with positive probability density. This completes the proof for $\beta  \ge 1/2$.
%Hence, for $\beta \ge 1/2$, the point process $\Pi$ is rigid at level 1.



% \end{document} 

==> Revised manuscript/rig.tex <==
% \documentclass[11pt]{article}
% \usepackage{amsmath,amsthm,amsfonts,amssymb,mathrsfs,bm,graphicx,amscd,epsfig,psfrag,verbatim,hyperref}
% \usepackage[usenames]{color}
% \usepackage{fancyhdr}
% \oddsidemargin	0.635cm
% \textwidth	15.3cm
% \topmargin	-1cm
% \textheight	23cm
% \parindent	10pt
% \parskip 	\bigskipamount
% % \usepackage{graphicx}
% % \usepackage{amscd}
% % \usepackage{amsmath}
% % \usepackage{amsfonts}
% % \usepackage{yfonts}
% % \usepackage{psfrag}
% % \usepackage{amssymb}
% % \usepackage{verbatim}
% % \usepackage{comment}
%
% %%%%%%%%%%%THEOREMS%%%%%%%%%%%
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{property}{Property}[section]
% \newtheorem{remark}{Remark}[section]
% \newtheorem{example}{Example}[section]
% \newtheorem{definition}{Definition}
% \newtheorem{claim}{Claim}
% \newtheorem{question}{Question}
% \newtheorem{notation}{Notation}
% %%%%%%%%%%%LETTERS%%%%%%%%%%%
% \def\a{{\alpha}}
% \def\N{\mathbb{N}}
% \def\Z{\mathbb{Z}}
% \def\Q{\mathbb{Q}}
% \def\R{\mathbb{R}}
% \def\C{\mathbb{C}}
% \def\E{\mathbb{E}}
% \def\P{\mathbb{P}}
% \def\e{\eilon}
% \def\d{\delta}
% \def\Pi{\Pi}
% \def\F{\mathcal{F}}
% \def\p{\mathcal{P}}
% \def\L{\Delta}
% \def\g{\Gamma}
% \def\gm{\gamma}
% \def\t{\theta}
% \def\la{\lambda}
% \def\k{\mathbb{K}}
% \def\D{\mathcal{D}}
% \def\e{\eilon}
% \def\A{\mathcal{A}}
% \def\o{\omega}
% \def\z{\zeta}
% \def\ze{\mathcal{Z}}
% \def\c{\mathcal{C}}
% \def\fa{f_{\alpha}}
% \def\e{\mathcal{E}}
% \def\h{\mathcal{H}}
% \def\b{\mathcal{B}}
% \def\el{\gamma}
% \def\ph{\varphi}
% \def\S{\mathcal{S}}
% \def\T{\mathcal{T}}
% \def\ja{(j!)^{\alpha}}
% \def\jh{(j!)^{\alpha/2}}
% \def\js{(j!)^{\alpha/2}}
% \def\I{\mathcal{I}}
% \def\k{\kappa}
% \def\u{\Upsilon}
% \def\ovl{\overline}
% \def\uz{\underline{\zeta}}
% \def\uout{\Upsilon_{\out}}
% \def\out{\mathrm{out}}
% \def\iin{\mathrm{in}}
% \def\els{\gamma_{\Sigma}}
% \def\ol{\overline}
% \def\var{\mathrm{Var}}
% \def\wt{\widetilde}
% \def\del{\delta}
% %\def\L{\Lambda}
% %\def\K{\mathcal{K}}
% %\def\H{\mathcal{H}}
% %\def\u{\mathbf{u}}
% %\def\v{\mathbf{v}}
% %\def\w{\wedge}
% \renewcommand{\l}[0]{\left }
% \renewcommand{\r}[0]{\right}
% \renewcommand{\qedsymbol}{$\blacksquare$}
% % \renewcommand{\x}[0]{\lfloor}
% % \renewcommand{\y}[0]{\rfloor}
% \makeatletter
% \renewcommand*{\@cite@ofmt}{\hbox}
% \makeatother
%
% \begin{document}
\section{Determinantal processes with radial intensity measures}
\label{radialmeasures}
% In this section, we will consider determinantal point processes on $\C$ with kernel \[K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j \] and background measure $\gamma$. Further, we will assume that $\gamma$ is a radial measure with $\mu$ being the measure on the non-negative real line induced naturally by $\gamma$, and \[c_j^{-1}= \int_0^\infty r^j d\mu(r).\] The last identity implies that $K$ is a reproducing kernel, projecting on to the subspace of $L^2(\gamma)$ gererated by the polynomials.

In this section, we will prove Theorems \ref{compact} and \ref{dpprt}. We will take up these proofs in two separate subsections. We recall the relevant notations from Section \ref{introduction}, and introduce some additional notation by setting $\Pi_n$ to be the d.p.p. generated by the $(K_n,\gamma)$, where $K_n$ is the truncated kernel given by \[K_n(z,w)=\sum_{j=0}^{n} c_j z^j\ol{w}^j.\] In our further considerations, we will use the concept of Palm measures. Roughly speaking, the Palm measure of a point process at the origin is the law of point process conditioned to contain the origin. The precise definition is given below. For a more detailed treatment, we refer the reader to chapter~10 of \cite{Ka} or chapter~3  of \cite{bbkbook}. 
%We include a formal definition of Palm measures at the end of the present section.

\begin{definition} \label{def:Palm}
Let $\Pi$ be a point process on the space $X$,  let $\mathcal{S}$ denote the Polish space of all locally finite point configurations on $X$,  $\mathcal{B}(X)$ denote the Borel sigma field on $\mathcal{S}$ and $\rho_1$ denote the one-point intensity measure of $\Pi$. Let $F : X \times \mathcal{S} \mapsto \R$ be a test function. Then, for $s \in X$, the Palm measure  $\Pi_s$ at $s$ is defined by  
$\E_\Pi \l[ \sum_{s \in \Pi} F(s,\Pi) \r] = \int_X \E_{\Pi_s} \l[  F(s,\Pi_s) \r] \mathrm{d}\rho_1(s)$.
\end{definition}

For a determinantal process  with kernel $K$, and any $s\in \Xi$ with $K(s,s)>0$, the Palm measure at $s$ exists and is again a determinantal process with kernel
\[
K_s(x,y)=K(x,y)-\frac{K(x,s)K(s,y)}{K(s,s)}.
\]
See Theorem~1.7 in \cite{shiraitakahashi}.

\subsection{Proof of Theorem \ref{compact}}
% Let, as before, $\Pi$ be a d.p.p. with kernel $K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j $ and background measure $\gamma$. Further assume that $\gamma$ is a radial measure with $\mu$ being the measure on the positive real line induced naturally by $\gamma$, and $c_j^{-1}= \int_0^\infty r^j d\mu(r)$, so that $K$ is a reproducing kernel, projecting on to the subspace of $L^2(\gamma)$ gererated by the polynomials.
% Let $\Gamma_j$ be the size biasing of $\mu$ of the order $j$; in other words, $\Gamma_j$ has a density which is proportional to $r^jd\mu(r)$. Let \[\mu_j:=\E[\Gamma_j]=c_j/c_{j+1}\] and \[\sigma_j:=\E\l[\l(\frac{\Gamma_j}{\mu_j}-1\r)^2\r]=\l(\frac{\mu_{j+1}}{\mu_j}-1\r).\]

% In this set up, we prove:
% \begin{theorem}
% Suppose the moment sequence $\{\mu_j\}_{j=1}^{\infty}$ satisfy $\sum_{j=1}^{\infty}\sigma_j < \infty$. Then the process $\Pi$ does not exhibit rigidity of numbers.
% \end{theorem}

% \begin{remark}
% \end{remark}

\begin{proof}
 We will show that $\Pi$ and the Palm measure of $\Pi$ at the origin can be coupled so that they are equal with positive probability. This will show that, with positive probability, a point can suitably be removed or added to $\Pi$ without detection, establishing that there cannot be rigidity of the number of points. In fact, we show that the Palm measure $\wt{\Pi}_n$ of $\Pi_n$ at the origin and $\Pi_{n-1}$ can be coupled so that they are equal with a positive probability, that stays bounded away from 0 as $n \to \infty$. Then, using the fact that $\Pi_n \to \Pi$ and $\wt{\Pi}_n \to \wt{\Pi}$ weakly, we can draw the desired conclusion about $\Pi$.

 Note that the process $\Pi_n$ is determinantal with kernel $K_n$ and hence contains $n+1$ points,  almost surely. The joint density of  the points of $\Pi_n$ (when placed in uniform random order)  is given by \[p_n(z_1,\cdots,z_{n+1})=C c_0 c_1 \cdots c_n |\Delta(z_1,\cdots,z_{n+1})|^2,\] where $\Delta(z_1,\cdots,z_{n+1})$ is, as usual, the Vandermonde determinant formed by $z_1,\cdots,z_{n+1}$. The Palm measure $\wt{\Pi}_n$ of $\Pi_n$ at the origin is a determinantal point process with background measure $\gamma$ and kernel given by $\wt{K}_n(z,w)=K_n(z,w)-c_0$. Thus, $\wt{\Pi}_n$ has a density given by $\wt{p}_n(z_1,\cdots,z_n)=C c_1 \cdots c_n|z_1|^2\cdots|z_n|^2  |\Delta(z_1,\cdots,z_n)|^2$. Then the Radon Nikodym derivative of $\wt{\Pi}_n$ w.r.t. $\Pi_{n-1}$ is given by \[\t_n(z_1,\cdots,z_n)=\frac{\wt{p}_n(z_1,\cdots,z_n)}{p_{n-1}(z_1,\cdots,z_n)}= c_n |z_1|^2 \cdots |z_n|^2.\]

 The maximal probability, under any coupling of $\wt{\Pi}_n$ and $\Pi_{n-1}$, that the coupled random variables are equal is $\E_{\Pi_{n-1}}\l[ \t_n(z_1,\cdots,z_n) \wedge 1  \r]$. Therefore, our goal is to show that $\E_{\Pi_{n-1}}\l[ \t_n(z_1,\cdots,z_n) \wedge 1  \r]$ is bounded away from 0 as $n \to \infty$. One can then take a subsequential weak limit of the finite dimensional couplings and obtain a coupling of $\Pi$ and $\wt{\Pi}$ with the desired property. We will show that, under the growth assumption on the moments as described in the statement of the theorem, $  \t_n(z_1,\cdots,z_n)= c_n |z_1|^2 \cdots |z_n|^2 \to Z$ a.s., where $Z>0$ with positive probability. 
 
To this end, we consider $W$ to be a random variable distributed according to the probability measure $\mu(\cdot)/\mu(\C)$. Then we set $\Gamma_1 = |W|^2$, and each $\Gamma_k$ is a size-biased version of $\Gamma_{k-1}$, i.e. the corresponding probability measures satisfy $d \Gamma_k = \frac{c_k}{c_{k-1}} d \Gamma_{k-1}$. Theorem Theorem~4.7.1 in \cite{HKPV} essentially states that, if $(z_1,\ldots,z_n) \sim \Pi_{n-1}$, then  $\{|z_i|^2\}_{i=1}^n$ has the same distribution as $\{|\Gamma_i|\}_{i=1}^n$, where the $\Gamma_i$-s are independent copies of the random variables described above. 
 

Thus, observe that we can write, using Theorem~4.7.1 in \cite{HKPV},
 \[c_n |z_1|^2 \cdots |z_n|^2 =  c_0 \prod_{i=1}^n \frac{|z_i|^2}{(c_{i-1}/c_i)} =  c_0 \prod_{j=1}^n\frac{\Gamma_j}{\mu_j}= c_0  \prod_{j=1}^n\l(1+\l(\frac{\Gamma_j}{\mu_j}-1\r)\r),\] where $\Gamma_j$-s are independent copies of the size biased random variables. discussed above. 
 
 Thus, it suffices to show that $\l|\sum_{j=1}^{\infty}\l(\frac{\Gamma_j}{\mu_j}-1\r) \r|<\infty$. By the Kolmogorov's Two Series Theorem (c.f. \cite{Durrett} Chap. 2), this will be true if  $\sum_{j=1}^{\infty}\mathrm{Var}\l(\frac{\Gamma_j}{\mu_j}-1\r) <\infty$. This is exactly the condition \[\sum_{j=1}^{\infty}\l( \frac{\mu_{j+1}}{\mu_j} -1 \r) < \infty.\] This is precisely growth criterion laid out in the statement of the theorem.
 \end{proof}


\subsection{Proof of Theorem \ref{dpprt}}
\label{dpprtproof}
% \label{invpowersgin}
% Let, as before, $\Pi$ be a d.p.p. with kernel $K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j $ and background measure $\gamma$. Further assume that $\gamma$ is a radial measure with $\mu$ being the measure on the positive real line induced naturally by $\gamma$, and $c_j^{-1}= \int_0^\infty r^j d\mu(r)$, so that $K$ is a reproducing kernel, projecting on to the subspace of $L^2(\gamma)$ gererated by the polynomials. Let $\Pi_n$ be the d.p.p. generated by the $(K_n,\gamma)$, where $K_n$ is the truncated kernel given by $K(z,w)=\sum_{j=0}^{n} c_j z^j\ol{w}^j .$


% Let $B(0;r)$ denote the disk of radius $r$ centred at the origin. Let $\Gamma_j$ be the size biasing of $\mu$ of the order $j$; in other words, $\Gamma_j$ has a density which is proportional to $r^jd\mu(r)$. Set \[\nu_j := \E\l[  \l(\frac{\Gamma_j}{\mu_j}-1\r)^4\r]= \l( \frac{\mu_{j+3}\mu_{j+2}\mu_{j+1}}{\mu_j} - 4 \frac{\mu_{j+2} \mu_{j+1}}{\mu_j^2} + 6 \frac{\mu_{j+1}}{\mu_j} -3 \r).\]

% \begin{remark}
%  An important class of measures which satisfies this criterion is those which exhibit the following asymptotics, for some constants $C,A,\a$: \[\mu_j:=\E[\Gamma_j]=Cj^\a\l(1+\frac{A}{j} + O(\frac{1}{j^2})\r).\]
% In other words, we stipulate a power law for the means of the size biased measures $\Gamma_j$. This covers the case of all measures of the form $d\mu(r)=r^\beta e^{-r^\gamma}dr$, which includes the Ginibre ensemble.
% \end{remark}

We begin by recalling that   $\Pi$ is the d.p.p. generated by the $(K,\gamma)$, where $K$ is the  kernel given by \[K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j.\] On the other hand,
$\Pi_n$ is the d.p.p. generated by the $(K_n,\gamma)$, where $K_n$ is the truncated kernel given by \[K_n(z,w)=\sum_{j=0}^{n} c_j z^j\ol{w}^j.\] The sequence of d.p.p.-s $\{\Pi_n\}_{n \ge 0}$ converges to the d.p.p. $\Pi$ in the sense of convergence of point processes (\cite{DV}).


We will study the variance of linear statistics of $\Pi$ and $\Pi_n$, and show that under certain conditions on the coefficients, the variance of linear statistics remains bounded even as the scaling factor goes to infinity. 
Invoking a result in \cite{GP} (c.f. Theorem 6.1 therein; for a statement see Theorem \ref{thm:GP} in Section \ref{sec:thiswillberewritten}), this would be enough to guarantee the rigidity of the number of points of $\Pi$ in any bounded open set. For a more detailed discussion on this matter, we refer the reader to the Proof of Theorem \ref{dpprt} later in this section. 

To prove Theorem \ref{dpprt}, we will first state and prove an estimate on the variance of linear statistics of $\Pi$.

\begin{proposition}
\label{est}
Let $\varphi$ be a compactly supported Lipschitz function, supported inside the disk $B(0;r)$ with Lipschitz constant $\kappa(\varphi)$. Let $\varphi_R(z):=\varphi(z/R)$. Suppose  that the growth conditions in the statement of Theorem \ref{dpprt} hold.

Then we have 
\begin{equation} \label{estimate} 
\mathrm{Var} \l(\int\varphi_R(z)\, d[\Pi_n](z)\r)\le B \kappa(\varphi)^2 + C \|\varphi\|^2_\infty \rho(R),
\end{equation} 
where $B,C$ are positive numbers and $\rho(R)$ is a quantity that $\to 0$ as $R \to \infty$, uniformly in $n$ and $\varphi$.
The same conclusion holds for $\Pi$ in place of $\Pi_n$.
\end{proposition}



To prove Proposition \ref{est}, we will make use of a general fact about determinantal point processes:
\begin{lemma}
\label{varlinst}
Let $\Pi$ be a determinantal point process with Hermitian kernel $K$. Let $K$ be a reproducing kernel with respect to its background measure $\gamma$, i.e., $K(x,y)= \int K(x,z)K(z,y)\, \mathrm{d}\gamma(z)$ for all $x,y$. Let $\varphi, \psi$ be  compactly supported continuous functions.  Then we have
\[\mathrm{Cov} \l( \int \varphi \, d\Pi, \int \psi \, d\Pi \r) = \frac{1}{2}\iint (\varphi(z) - \varphi (w)) \overline{(\psi(z)-\psi(w))}|K(z,w)|^2 \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w).\]
\end{lemma}


\begin{proof} [\textbf{Proof of Proposition \ref{est}}]
We give the proof when $r=1$, from here the general case is obtained by scaling, because any function $\varphi$ supported on $B(0;r)$ is equal to the scaling $\Phi_r$ of some function $\Phi$ supported on $B(0;1)$ and having the same continuity and differentiability properties as $\varphi$. Notice that $(\Phi_r)_R=\Phi_{rR}$, so the result for $\varphi$ can be deduced from the result for $\Phi$. In what follows we deal with $\Pi_n$, the result for $\Pi$ follows, for instance, from taking limits as $n \to \infty$ for the result for $\Pi_n$.

Using Lemma \ref{varlinst}, we have \[\text{Var} \l(\int \varphi_R(z)\, d[\Pi_n](z) \r)= \frac{1}{2} \iint {|\varphi_R(z)-\varphi_R(w)|^2|K_n(z,w)|^2\, \mathrm{d}\gamma(z)\, \mathrm{d}\gamma(w)}\]
where $\gamma$ is the background measure.
Now, \[|\varphi_R(z)-\varphi_R(w)|^2 = |\varphi(z/R)-\varphi(w/R)|^2 \le \frac{1}{R^2}\kappa(\varphi)^2|z-w|^2. \]
Therefore, it suffices to bound the integral $\int_{A(R)} |\varphi_R(z)-\varphi_R(w)|^2 |K_n(z,w)|^2 \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w)$ on the set \[A(R):= \{ (z,w) : \min\{|z|, |w|\} \le R \} \] because outside $A(R)$, we have $\varphi_R(z)=\varphi_R(w)=0$.  

Thus, we may write
\begin{align*}
& \int_{A(R)} |\varphi(z/R)-\varphi(w/R)|^2 |K_n(z,w)|^2 \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w) \\ 
\le & \frac{\kappa(\varphi)^2}{R^2} \int_{A_1(R)} |z-w|^2 |K_n(z,w)|^2 \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w) + \|\varphi\|_\infty^2 \int_{A_2(R)} |K_n(z,w)|^2 \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w) 
\numberthis \label{eq:A1-A2}
\end{align*}
where, for  $a \ge 2$, we set \[A_1(R)=\{ |z|\le aR, |w| \le aR \} \text{ and } A_2(R)=\{ |z|\le R, |w| \ge aR \} \cup \{ |w|\le R, |z| \ge aR \}. \]

% We first address the case of $A_2(R)$. By symmetry, it suffices to bound the integral over the region $\{ |z|\le R, |w| \ge aR \}$. In this region, $||z|-|w|| \ge (a-1)R$, and $|K_n(z,w)|^2 e^{-|z|^2-|w|^2} \le e^{-||z|-|w||^2}$. The integral is bounded from above by \[\frac{1}{\pi^2}\int_{|z| \le R} \l( \int_{|w| \ge aR} (|z|+|w|)^2 \, \mathrm{d}\gamma(w)\r)  \mathrm{d}\gamma(z)   .\]
% It is not hard to see that the inner integral is $O(R^2e^{-R^2})$ Integrating over $|z|\le R$ gives another factor of $R^2$, so the total contribution is $o(1)$ as $R \to \infty$.

In \eqref{eq:A1-A2}, the integral over $A_1(R)$ will provide an upper bound of $B \kappa(\varphi)^2$, whereas the integral over $A_2(R)$ will be controlled by a quantity of the form $\|\varphi\|^2_\infty \rho(R)$, where 
$\rho(R) \to 0$ as $R \to \infty$, uniformly in $n$ and $\varphi$. The bounds for these two integrals will be taken up in Propositions \ref{prop:A1} and \ref{prop:A2} respectively.

Combining \eqref{eq:A1-A2} with Propositions \ref{prop:A1} and \ref{prop:A2}, we obtain the desired estimate on the variance of linear statistics as stated in Proposition \ref{est}.
\end{proof}

\begin{proposition}  \label{prop:A1}
Consider the integral 
\[ I_1(R,\varphi) := \frac{\kappa(\varphi)^2}{R^2} \int_{A_1(R)} |z-w|^2 |K_n(z,w)|^2 \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w)\] as in \eqref{eq:A1-A2}.
Then we have
\[ I_1(R,\varphi) \le  B \kappa(\varphi)^2 \]
for some positive number $B$.
\end{proposition}

\begin{proof}
We begin with
\begin{align*}
&\int_{A_1(R)} |z-w|^2 |K_n(z,w)|^2\, \mathrm{d}\gamma(z) \mathrm{d}\gamma(w)
\\& = \int \bigg( |z|^2-z\bar{w}-\bar{z}w+|w|^2 \bigg) \l(\sum_{j=0}^{n-1}c_j( z\bar{w})^j\r) \l(\sum_{j=0}^{n-1} c_j( \bar{z}w)^j\r) \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w). \numberthis \label{eq:integral}
\end{align*}
Now, we integrate the $|z-w|^2$ part term by term. Due to the radial symmetry of $\gamma$, only some specific terms from $|K_n(z,w)|^2$ contribute. For example, when we integrate the $|z|^2$ term in $|z-w|^2$, only the ${\displaystyle c_j (z\bar{w})^j c_j (\bar{z}w)^j}$,$0\le j\le n-1$ terms in the expanded expression for $|K_n(z,w)|^2$ contribute. When we integrate $z\bar{w}$, only the ${\displaystyle c_j(z\bar{w})^{j}c_{j+1} (\bar{z}w)^{j+1} }$,$0\le j\le{n-2}$ terms provide non-zero contributions. Due to symmetry between $z$ and $w$, it is enough to bound the contribution from $(|z|^2 - z \overline{w})$ by  $O(R^2)$, with the constant in the $O$ being independent of $n$.
% \newline

In what follows, we will denote by $\mu$ the measure on $\R_+$ obtained by the push forward of the measure $\gamma$ from $\C$ to $\R_+$ under the map $z \mapsto |z|^2$.

$\bullet$ \underline{$|z|^2$ term: }

Let us introduce the change of variables  by $x=|z|^2$ and $y=|w|^2$. Then the contribution in the above integral \eqref{eq:integral} coming from \[ c_j (z\bar{w})^jc_j (\bar{z}w)^j\] can be written as \[ \int_0^{a^2R^2} \int_0^{a^2R^2} c_j x^{j+1} c_j y^{j} d\mu(x)d\mu(y). \] So, the total contribution due to all such terms, ranging from $j=0,\cdots,n-1$ is \[ \sum_{j=0}^{n-1}  \l( \int_0^{a^2 R^2} c_j x^{j+1} d\mu(x) \r) \l( \int_0^{a^2 R^2} c_{j+1} y^{j}d\mu(y) \r). \]
% \newpage

$\bullet$
 \underline{$z\bar{w}$ term: }

As above, the contribution coming from the \[ c_j(z\bar{w})^{j}c_{j+1}(\bar{z}w)^{j+1} \] is given by \[ \int_0^{a^2R^2} \int_0^{a^2R^2}c_j x^{j+1} c_{j+1} y^{j+1}d\mu(x)d\mu(y).  \] Therefore the total contribution from $0\le j\le{n-2}$ is
\[\sum_{j=0}^{n-2} \l( \int_0^{a^2 R^2} c_j  x^{j+1} d\mu(x) \r) \l( \int_0^{a^2R^2} c_{j+1} y^{j+1} d\mu(y) \r).\]

Recall that ${\displaystyle c_j x^jd\mu(x)}$ is a probability density, denote the corresponding random variable by $\Gamma_{j+1}$ (it may be seen that the random variable $\Gamma_j$ defined here, and that introduced in the proof of Theorem \ref{compact} are the same, using Theorem 4.7.1 in \cite{HKPV}; however, we do not require this fact for our arguments in this subsection). 

The contribution due to the $|z|^2$ term is ${ \displaystyle \sum_{j=0}^{n-1} \E[\Gamma_{j+1}{1\hskip-4pt{\rm 1}}_{(\Gamma_{j+1}\le a^2R^2)}]\P[\Gamma_{j+1}\le a^2R^2]}$ and that due to the $z\bar{w}$ term is
${ \displaystyle \sum_{j=0}^{n-2} \E[\Gamma_{j+1}{1\hskip-4pt{\rm 1}}_{(\Gamma_{j+1}\le a^2R^2)}]\P[\Gamma_{j+2}\le a^2R^2] }$.

$\bullet$ \underline{Combining the terms:}
The difference between the above two terms can be written as:
\begin{equation}
 \label{qty}
 \E[\Gamma_{n}{1\hskip-4pt{\rm 1}}_{(\Gamma_{n}\le a^2R^2)}]\P[\Gamma_{n}\le a^2R^2]+\sum_{j=1}^{n-1}\E[\Gamma_j{1\hskip-4pt{\rm 1}}{(\Gamma_j\le a^2R^2)}]\bigg(\P[\Gamma_j\le a^2R^2]-\P[\Gamma_{j+1}\le a^2R^2] \bigg).
\end{equation}
All the expectations in the above are $\le a^2R^2$, and $\P[\Gamma_j\le a^2R^2] \ge \P[\Gamma_{j+1}\le a^2R^2]$ because $\Gamma_{j+1}$ stochastically dominates $\Gamma_j$ (this is true because  a random variable is stochastically dominated by its size biasing). 

Therefore the absolute value of \eqref{qty}, by a telescopic sum, is bounded above by 
\begin{align*}
& \E[\Gamma_{n}{1\hskip-4pt{\rm 1}}_{(\Gamma_{n}\le a^2R^2)}]\P[\Gamma_{n}\le a^2R^2]+\sum_{j=1}^{n-1}\E[\Gamma_j{1\hskip-4pt{\rm 1}}{(\Gamma_j\le a^2R^2)}]\bigg(\P[\Gamma_j\le a^2R^2]-\P[\Gamma_{j+1}\le a^2R^2] \bigg) \\
\le & a^2R^2 \P[\Gamma_1\le a^2R^2] \\
\le & a^2R^2. \numberthis \label{eq:qty-1}
\end{align*}



%$\bullet$ \underline{$|w|^2$ term: } This term is treated on similar lines to the $|z|^2$ term.


$\bullet$ Finally, we  recall the definition of $I_1(R,\varphi)$ and combine with \eqref{eq:qty-1} to complete the proof of the proposition.


\end{proof}


\begin{proposition} \label{prop:A2}
Let 
\[I_2(R,\varphi):=)\|\varphi\|_\infty^2 \int_{A_2(R)} |K_n(z,w)|^2 \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w)   \]
and set
\begin{equation} \label{suffcond} 
\rho(R):= \sum_{j=0}^n \P\l[\Gamma_j \le R^2\r] \P\l[ \Gamma_j \ge a^2R^2 \r]. 
\end{equation}
Then $I_2(R,\varphi) \le C \|\varphi\|^2_\infty \rho(R)$ for some positive number $C$ and, furthermore, $\rho(R) \to 0$ uniformly in $n, \varphi$ as $R \to \infty$.
\end{proposition}

\begin{proof}
We proceed with our analysis of $I_2(R,\varphi)$ as in the proof of Proposition \ref{prop:A1}. In this vein, we write, 
\begin{align}  
 \|\varphi\|_\infty^2 \int_{A_2(R)}&  |K_n(z,w)|^2\, \mathrm{d}\gamma(z) \mathrm{d}\gamma(w) \nonumber \\
 &= \|\varphi\|_\infty^2 \int_{A_2(R)} \l(\sum_{j=0}^{n-1}c_j( z\bar{w})^j\r) \l(\sum_{j=0}^{n-1} c_j( \bar{z}w)^j\r) \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w). \label{eq:integral-1}
\end{align}

Due to the radial symmetry of $\gamma$, only some specific terms from $|K_n(z,w)|^2$ contribute to the above integral. To be more specific, only the ${\displaystyle c_j (z\bar{w})^j c_j (\bar{z}w)^j}$,$0\le j\le n-1$ terms in the expanded expression for $|K_n(z,w)|^2$ contribute. 

%When we integrate $z\bar{w}$, only the ${\displaystyle c_j(z\bar{w})^{j}c_{j+1} (\bar{z}w)^{j+1} }$,$0\le j\le{n-2}$ terms provide non-zero contributions. Due to symmetry between $z$ and $w$, it is enough to bound the contribution from $(|z|^2 - z \overline{w})$ by  $O(R^2)$, with the constant in the $O$ being independent of $n$.
% \newline

As in the proof of Proposition \ref{prop:A1}, we will denote by $\mu$ the measure on $\R_+$ obtained by the push forward of the measure $\gamma$ from $\C$ to $\R_+$ under the map $z \mapsto |z|^2$.

Thus, we may rewrite the right hand side of \eqref{eq:integral-1} as 
\begin{align*}  
& \int \l(\sum_{j=0}^{n-1}c_j( z\bar{w})^j\r) \l(\sum_{j=0}^{n-1} c_j( \bar{z}w)^j\r) \, \mathrm{d}\gamma(z) \, \mathrm{d}\gamma(w) \\
= &  \sum_{j=0}^{n-1} \l( \int_0^{ R^2} c_j  x^j d\mu(x) \r) \l( \int_{a^2R^2}^{\infty} c_{j} y^{j} d\mu(y) \r) + \sum_{j=0}^{n-1} \l(   \int_{a^2R^2}^{\infty} c_j  x^j d\mu(x) \r) \l( \int_0^{ R^2} c_{j} y^{j} d\mu(y) \r)
\numberthis \label{eq:integral-2}
\end{align*}
Due to reasons of symmetry,  the two terms on the right hand side of \eqref{eq:integral-2} are equal, and we need estimate only one of them. 

We recall from the proof of Proposition \ref{prop:A1} the random variable $\Gamma_{j+1}$, which corresponds to the probability measure on $\R_+$ given by $c_j x^j d\mu(x)$. As such, we may write
\[\rho(R) : =  \sum_{j=0}^{n-1} \l( \int_0^{ R^2} c_j  x^j d\mu(x) \r) \l( \int_{a^2R^2}^{\infty} c_{j} y^{j} d\mu(y) \r) = \sum_{j=0}^n \P\l[\Gamma_j \le R^2\r] \P\l[ \Gamma_j \ge a^2R^2 \r]. \] It suffices, therefore, to show that $\rho(R) \to 0$ uniformly in $n, \varphi$ as $R \to \infty$.
% (for another sufficient criterion, see Remark \ref{rem:alt_crit} at the end of this proof).   


% Another important class of measures is one where we have, for some constants $C,\a,A$, the mean $\mu_j:=\E[\Gamma_j]=Cj^\a\l(1+\frac{A}{j} + O(\frac{1}{j^2})\r)$.
% In other words, we stipulate a power law for the means of the size biased measures $\Gamma_j$. This covers the case of all measures of the form $d\mu(r)=r^\beta e^{-r^\gamma}dr$, which includes the Ginibre ensemble.

%To see this, we aim to show that \eqref{suffcond} is $O(1)$ as $R \to \infty$. 
We consider the $\Gamma_j$-s in two groups: $J_1:=\{ j| \mu_j \le 2 R^2\}$ and $J_2:=\{j| \mu_j > 2 R^2\}$. Let $j_*:=\max\{j|j\in J_1\}$. Clearly,
\begin{align*}  \rho(R) = & \sum_{j=0}^n \P\l[\Gamma_j \le R^2\r] \P\l[ \Gamma_j \ge a^2R^2 \r] \\ \le & \l( \sum_{j \in J_1} \P\l[ \Gamma_j \ge a^2R^2 \r] \r) + \l( \sum_{j \in J_2} \P\l[ \Gamma_j \le R^2 \r] \r). \end{align*}
Observe that, for any $j$ we have
 \[ \E[\Gamma_j]=\mu_j; \quad  \mathrm{Var}\l( \Gamma_j/\mu_j \r)= \l( \frac{\mu_{j+1}}{\mu_j}-1 \r)\] 
 and 
 \begin{equation} \label{eq:nu_j}
 \E\l[\l(\frac{\Gamma_j}{\mu_j}-1\r)^4\r] =\l( \frac{\mu_{j+3}\mu_{j+2}\mu_{j+1}}{\mu_j^3} - 4 \frac{\mu_{j+2} \mu_{j+1}}{\mu_j^2} + 6 \frac{\mu_{j+1}}{\mu_j} -3 \r) = \nu_j .
 \end{equation} 
 %It can be checked that the asymptotics on $\mu_j$ implies \[\E\l[\l(\frac{X}{\E[X]}-1\r)^4\r] \le C_\a /j^2. \]  

By  Chebyshev-type  inequality, we have 
\begin{align*} 
& \P\l[ \Gamma_j \ge a^2R^2  \r] \le \frac{\E\l( \Gamma_j/\mu_j -1 \r)^4}{(a^2R^2/\mu_j -1)^4}  \\ 
& \Rightarrow \sum_{j \in J_1} \P\l[ \Gamma_j \ge a^2R^2  \r] \le \sum_{j \in J_1}  \frac{\E\l( \Gamma_j/\mu_j -1 \r)^4}{(a^2R^2/\mu_j -1)^4}. 
\end{align*} 

We recall that $a \ge 2$, so that $\frac{a^2}{2} \ge 2$. 
 For $j \in J_1$ (recall that $J_1:=\{ j| \mu_j \le 2 R^2\}$), we have $\frac{a^2R^2}{\mu_j} \ge \frac{a^2}{2} \ge 2 ~\forall j \in J_1$. Since $|x-1|\ge x/2 ~\forall x \ge 2$, we deduce that  
    $|\frac{a^2R^2}{\mu_j}-1|\ge  \frac{a^2R^2}{2 \mu_j} \forall j \in J_1 $.  
    
Combining with \eqref{eq:nu_j}, We may therefore conclude that for each $j \in J_1$ we have    \[  \frac{\E\l( \Gamma_j/\mu_j -1 \r)^4}{(a^2R^2/\mu_j -1)^4} \le c \cdot  \mu_j^4\nu_j  \big/ (a^2R^2)^4 \] for some constant $c>0$. 
    
    Hence we have, for some constant $C>0$,
\begin{align*} & \sum_{j \in J_1} \P\l[ \Gamma_j \ge a^2R^2  \r] \\ & \le C \cdot \frac{1}{(a^2R^2)^4}\sum_{j \in J_1} \mu_j^4\nu_j \\ & =  C \cdot \frac{\mu_{j_*}^4}{(a^2R^2)^4}\frac{1}{\mu_{j_*}^4} \l\{ \sum_{j \le j_*} \mu_j^4\nu_j\r\} . \end{align*}
Notice that, by definition of $J_1$, we have $\frac{\mu_{j_*}^4}{(a^2R^2)^4} \le 16/a^8$.  By our assumption on the moment sequence, $\l\{ \sum_{j \le j_*} \mu_j^4\nu_j\r\}=o(\mu_{j_*}^4)$ as $j_* \to \infty$, i.e. as $R \to \infty$ (since $\mu_j \to \infty$ as $j \to \infty$). 

% Equivalently, as $R \to \infty$,
% \begin{align*} & \sum_{j \in J_1} \P\l[ \Gamma_j \ge a^2R^2  \r] \\  & \le \sum_{j \in J_1} \frac{\mu_j^2}{a^4R^4} \l( \mu_{j+1}/\mu_j -1 \r) \\ & \le C \frac{\sum_{j \in J_1}\mu_j^2/j}{a^4R^4} \\ & \le  C \frac{\sum_{j \in J_1} j^{2\a-1}}{a^4R^4} \\ & \le C j_*^{2\a}/a^4R^4, \end{align*}  where $j_*=\max\{j| j \in J_1 \}$.
% But by definition of $j_*$, we have $j_*^\a \le C bR^2 $, so as $R \to \infty$ we have \[\sum_{j \in J_1} \P\l[ \Gamma_j \ge a^2R^2  \r]=O(1).\]
% To bound the sum over $j \in J_2$, we use the following version of the second moment inequality: for $0<\t<1$ and a random variable $X>0$,
% \[ \P[ X \ge \t \E[X] ] \ge \frac{(1-\t)^2 \E[X]^2 }{ \mathrm{Var}[X] + (1-\t)^2 \E[X]^2 } . \] Equivalently, \[ \P[X /\E[X] \ge \t  ] \ge \frac{(1-\t)^2  }{ \mathrm{Var}[X/\E[X]] + (1-\t)^2 } . \] Therefore \[ \P[X /\E[X] < \t  ] \le 1- \frac{(1-\t)^2  }{ \mathrm{Var}[X/\E[X]] + (1-\t)^2 } = \frac{\mathrm{Var}[X/\E[X]]}{ \mathrm{Var}[X/\E[X]] + (1-\t)^2 } \]
% Combining all of these, we see that  $\text{Var} \l(\int \varphi_R(z)\, d[\Pi_n](z)\r)$ is bounded by  ${ \displaystyle \l(1/R^2 \r)2 \kappa(\varphi)^2 a^2 R^2=C(\varphi)}$. It is clear that $C(\varphi)$ depends on $\varphi$ only through $\kappa(\varphi)$.

On the other hand,  we note for $j \in J_2$ that we have
 \[ \P\l[\Gamma_j \le R^2\r] \le \frac{\E\l( \Gamma_j/\mu_j -1 \r)^4}{(R^2/\mu_j -1)^2} . \]
 Since $\mu_j \ge 2R^2$, we have $|\frac{R^2}{\mu_j}-1|\ge \frac{1}{2}$. As a result, we have \[ \sum_{j \in J_2} \P\l[ \Gamma_j \le R^2  \r] \le C \sum_{j \in J_2} \E\l( \Gamma_j/\mu_j -1 \r)^4  = C \sum_{j > j_*} \nu_j,\] which $\to 0$ as $j_* \to \infty$ (equivalently, as $R \to \infty$) by our assumption on the moment sequence $\{\nu_j\}_j$.

Thus, $\sum_{j=0}^n \P\l[\Gamma_j \le R^2\r] \P\l[ \Gamma_j \ge a^2R^2 \r] \to 0$ as $R \to \infty$, uniformly in $n$ and $\varphi$. This completes the proof of the proposition. 

\end{proof}


%\begin{remark} \label{rem:alt_crit}
%Another sufficient condition is that $\int_{a^2 R^2} |K(z,w)|^2 d\mu(w) \to 0$ uniformly on $\{|z| \le R\}$, in the sense that \[ \l( \sup_{|z|\le R} \int_{a^2 R^2}^{\infty} |K(z,w)|^2 d\gamma(w) \r) \to_{R \to \infty} 0.\] This criterion can be particularly helpful when we have an alternate expression for $K$ that enables us to perform estimates when $|z-w|$ is large. This is indeed the case with the important example of the Ginibre ensemble.
%\end{remark}

We are now ready to complete the proof of Theorem \ref{dpprt}.

\begin{proof}[Proof of Theorem \ref{dpprt}]
 Let $D$ be a bounded open set in $\C$. We will first establish the rigidity of the number of points in $D$.

 To do so, for any $\eps>0$, we will construct a function $\Psi_{\eps}$ with the following properties:
 \begin{itemize}
  \item $\Psi_{\eps} \equiv 1$ on $D$
  \item $\| \Psi_{\eps} \|_\infty \le 1$
  \item $\kappa(\Psi_\eps) < \sqrt{\eps}$.
\end{itemize}
Then, considering the dilations $(\Psi^{\eps})_R$, we get via Proposition \ref{est} that  for large enough $R$ we have
\begin{itemize}
  \item $(\Psi_{\eps})_R \equiv 1$ on $D$
  \item $\| (\Psi_{\eps})_R \|_\infty \le 1$
  \item $\Var\l( \int (\Psi^{\eps})_R d[\Pi] \r) < C \eps $.
\end{itemize}
Appealing to Theorem 6.1 in \cite{GP}, we deduce that the number of points in $D$ is rigid.

Let $r_0$ denote the radius of the disk $D$. We construct the function $\Psi_{\eps}$ as follows:
\[\Psi_{\eps}(r) = \begin{cases}
                           1 & \text{ for $0\le r \le r_0$}, \\
                           -\eps \log r + \eps \log r_0 +1  & \text{ for $r_0 \le r \le r_0\exp(1/\eps)$}, \\
                           0 & \text{ for $r \ge r_0\exp(1/\eps)$ }.
                          \end{cases}
  \]
It is a simple computation to check that $\Psi_{\eps}$ defined above has the desired properties.

%For the tolerance of the points in $D$, subject to the constraint on the number of points, we will mention the crucial point here and refer the reader to the accompanying note \cite{GK} for the details. It turns out that the estimate \ref{estimate} for $\Pi_n$-s, coupled with the additions moment assumption in the statement of our theorem, is enough to establish that the inverse power sums \[\l( \sum_{z \in \Pi_n \cap \D^c} \frac{1}{z^k} \r)\] is bounded above in expectation. Exploiting this as a crucial fact, and employing the techniques introduced in \cite{GP} to deal with the Ginibre ensemble, it can be shown that $\Pi$ is rigid of order 1.
\end{proof}




% \begin{thebibliography}{9}
%
% \bibitem[GhPe12]{GP}
%   S. Ghosh, Y. Peres, \emph{Rigidity and Tolerance in point processes: Gaussian zeroes and Ginibre eigenvalues}, http://arxiv.org/abs/1211.2381, Duke Mathematical Journal (to appear).
%
% \bibitem[HKPV10]{HKPV}
% J.B. Hough, M.Krishnapur, Y.Peres, B.Virag, \emph{Zeros of Gaussian Analytic Functions and Determinantal Point Processes}, A.M.S., 2010.
%
% \end{thebibliography}


% \end{document}


==> introduction.tex <==


 \section{Introduction}
 \label{introduction}
 The study of rigidity phenomena in random point sets has attracted a fair amount of attention in the recent past. To put it informally, ``rigidity'' refers to a phenomenon where, for a bounded domain $\D$ in the ambient space, the points of the set outside $\D$ determine, almost surely, certain properties of the points inside. In other words, we consider spatial conditioning in the random point set, and ``rigidity'' broadly refers to singularities appearing in the conditional distribution of the points inside $\D$ given the locations of those outside.
 
 We take this opportunity to provide a rigorous formulation of the phenomenon of ``rigidity'', on similar lines to \cite{GP}. Let us first describe the set-up in which we will work, and introduce some fundamental notions. A (simple) point process $\Pi$ is a random locally finite point configuration on some metric space $\Xi$ that is equipped with a regular Borel measure $\mu$. A point process can equivalently be looked upon as a random counting measure, with atoms corresponding to the points. For more details on point processes, we refer the reader to \cite{DV} and \cite{Ka}. The space $\S$ of locally finite point configurations on $\Xi$ is a Polish space, and a point process $\Pi$ on $\Xi$ can be thought of as a probability measure on $\S$.  Let $\D \subset \Xi$ be a bounded open set. The decomposition $\Xi=\D \cup \D^c$ induces a factorization $\S=\S_{\inn} \times \S_{\out}$, where $\S_{\inn}$ and $\S_{\out}$ are respectively the spaces of  finite point configurations on $\D$ and locally finite point configurations on $\D^c$.  This immediately leads to the natural decomposition $\Upsilon=(\Upsilon_{\inn},\Upsilon_{\out})$ for any $\Upsilon \in \S$, and  consequently a decomposition of the point process $\Pi$ as $\Pi=(\Pi_{\inn},\Pi_{\out})$. 

 We are now ready to formulate a rigorous definition of rigidity as follows. 
 \begin{definition}
 \label{defrig}
A measurable function $f_{\inn} : \S_{\inn} \rightarrow \C $ is said to be \textbf{rigid} with respect to the point process $X$ on $\S$ if there is a measurable function  $f_{\out}:\S_{\out} \rightarrow \C$ such that a.s. we have $f_{\inn}(X_{\inn})=f_{\out}(X_{\out})$.
\end{definition}
 
 Of course, the phenomenon of rigidity is the most interesting in the case of point processes that have infinitely many points. For finite processes (of a given size), the points outside a domain $\D$ will determine the number of points inside $\D$, and in the usual case of the points having a joint density, these points inside $\D$ could be in almost any configuration in $\D$. However, such simplistic behaviour cannot be expected, and indeed, is not true for point processes of infinite size. 
 
 The most common point process of infinite size, used as a model for many real world phenomena, is the Poisson point process. The most significant property of the Poisson process is the statistical independence of points in disjoint domains, and this property ensures that there is no ``rigidity'' of any sort for the Poisson process. However, for processes with non-trivial spatial correlation, the exploration of rigidity phenomena remains an interesting question. Among the most important natural examples of point processes of this kind are the bulk scaling limits of various random matrix ensembles, e.g. the sine kernel process in one dimension, or the Ginibre ensemble in two dimensions. Other significant ensembles include the zeroes of the standard planar Gaussian Analytic Function, abbreviated as the (standard planar) GAF on the complex plane, and the zeroes of the standard GAF on the hyperbolic plane. 
 
 The underlying randomness in most of these processes comes from independent Gaussian random variables, and inspite of the non-trivial spatial correlations, it would be natural to expect a fair amount of regularity or smoothness in the conditional distributions (under spatial conditioning). For example, one might expect that the conditional distribution of the points inside a given domain $\D$ would be, a.s., mutually absolutely continuous with respect to a Poisson process on $\D$. However, it turns out that in many of these processes, such anticipated regularity is not true. On the contrary, the conditional distribution of the points inside $\D$ is highlly sinngular, in the sense that the support of the conditional measure is a singular subset of the ambient domain.
  
 In \cite{GP}, the authors studied rigidity phenomena with regard to the Ginibre ensemble and the standard planar GAF zero process. The Ginibre ensemble is the weak limit of the eigenvalues of non-Hermitian (complex) Gaussian random matrices. The standard planar GAF is the Gaussian power series \[f(z)=\sum_{k=0}^\infty \frac{\xi_k}{\sqrt{k!}}z^k,\] and the GAF zero process is the point process of zeroes of this random analytic function. For more details on these ensembles, we refer the reader to \cite{HKPV}.
 
 The study of rigidity phenomena in point processes has received some attention in the recent past; we mention here some of the works relevant to our study. In \cite{G-1}, it was shown that the sine kernel process (which arises as the bulk limit of Hermitian random matrix ensembles) exhibits rigidity in the number of points in a domain. Similar results were also established for a wide range of translation invariant determinantal point processes on $\Z$ (introduced by Lyons and Steif \cite{LySt}) that correspond to function spaces characterised by vanishing Fourier transform outside a given set. In \cite{OsSh}, Osada and Shirai showed that for the Ginibre ensemble, the Palm measures with respect to different point sets are mutually absolutely continuous if the conditioning set of points have the same cardinality, and are mutually absolutely continuous otherwise. Such dichotomy is similar in spirit to, and is, in fact, closely related with the rigidity phenomena under our consideration. For more on this theme, we refer the reader to the upcoming article \cite{G-2}. 
 
 Rigidity phenomena have also been exploited to answer questions on point processes and stochastic geometry which are interesting in their own right. In \cite{G-1}, rigidity of the sine kernel process was exploited to answer a completeness question related to exponential functions coming from the point process. In \cite{GKP}, the authors used an understanding of the rigidity behaviour of the Ginibre ensemble and the standard planar GAF zero process obtained in 
 \cite{GP} in order to study continuum percolation on these models. In particular, they showed the  existence of a non-trivial critical radius for percolation, and established the uniqueness of the infinite cluster in the supercritical regime. In \cite{Os}, an understanding of  quasi-Gibbs property, which has a somewhat similar  flavour to rigidity and tolerance, was used to define an infinite particle SDE for invariant dynamics on the Ginibre process. To execute a similar programme for invariant dynamics on the standard planar GAF zero process involves new challenges involving the higher level of rigidity in GAF, and is a topic of current research.
  
 In \cite{GP}, the authors showed that in the Ginibre ensemble, the points outside any bounded open set $\D$ determine a.s. the number of points inside $\D$, and in the GAF zero process, the points outside $\D$ determine the number and the sum of the points inside. If we think of the points as a particle system, then this can be described by saying that in the Ginibre ensemble, there is local conservation of mass, while in the standard planar GAF zero process, the mass as well as the centre of mass are locally conserved. Moreover, they showed that these are the ``only'' conservation laws in these ensembles, in a natural sense. To be precise, we quote the relevant theorems from \cite{GP}.
 
 In Theorems \ref{gin-1}-\ref{gaf-2} we denote the Ginibre ensemble by $\G$ and the GAF zero ensemble by $\F$. As before, $\D$ is a bounded open set in $\C$. 

 In the case of the Ginibre ensemble, we prove that a.s.  the points outside $\D$ determine the number of points inside $\D$, and ``nothing more''. 

\begin{theorem}
 \label{gin-1}
For the Ginibre ensemble, there is a measurable function $N:\S_{\out} \to \nat$ such that a.s. \[ \mathrm{ \ Number \ of \ points \ in \ } \G_{\inn} = N(\G_{\out})\hspace{3 pt}.\]
\end{theorem}

Since a.s. the length of $\uz$ equals $N(\G_{\out})$, we can assume that each measure $\rho(\uout,\cdot)$ is supported on $\D^{N({\uout})}$.


\begin{theorem}
\label{gin-2}
For the Ginibre ensemble, $\P$-a.s. the measure $\rho({\G_{\out}},\cdot)$ and the Lebesgue measure $\el$ on $\D^{N(\G_{\out})}$ are mutually absolutely continuous.
\end{theorem}

In the case of the GAF zero process, we prove that the points outside $\D$ determine the number as well as the centre of mass (or equivalently, the sum) of the points inside $\D$, and ``nothing more''. 

\begin{theorem}
 \label{gaf-1}
For the GAF zero ensemble, \newline
\noindent
(i)There is a measurable function $N:\S_{\out} \to \nat$ such that a.s.  \[ \mathrm{ \ Number \ of \ points \ in \ } \F_{\inn} = N(\F_{\out}).\]
(ii)There is a measurable function $S:\S_{\out} \to \C$ such that a.s.  \[ \mathrm{ \ Sum \ of \ the \ points \ in \ } \F_{\inn} = S(\F_{\out}).\]
\end{theorem}

For a possible value $\uout$ of $\F_{\out}$, define the set of admissible vectors of inside points (obtained by considering all possible orderings of such inside point configurations) \[ \Sigma_{S({\uout})} := \{ \uz \in \D^{N({\uout})} : \sum_{j=1}^{N({\uout})} \z_j = S({\uout}) \}\] where $\uz=(\z_1,\cdots,\z_{N({\uout})})$.

Since a.s. the length of $\uz$ equals $N({\uout})$, we can assume that each measure $\rho(\uout,\cdot)$ gives us the distribution of a random vector in  $\D^{N({\uout})}$ supported on $\Sigma_{S({\uout})}$.

\begin{theorem}
\label{gaf-2}
For the GAF zero ensemble, $\P$-a.s. the measure $\rho(\F_{\out},\cdot)$ and the Lebesgue measure $\els$ on $\Sigma_{S(\F_{\out})}$ are mutually absolutely continuous.
\end{theorem}

Theorems \ref{gin-2} and \ref{gaf-2} lead to a natural definition of ``tolerance'' for point processes. Heuristically, this corresponds to the regularity of the spatially conditional measures, modulo local rigidity constraints. Before making a formal definition, let us recall the definition of linear statistics: 
\begin{definition}
 \label{linstat}
Let $\Pi$ be a point proces on $\Xi$ and $\ph:\Xi \to \C$ be a measurable function. Then the linear statistics $\La(\ph)[\Pi]$ of $\Pi$ is defined to be the random variable \[\La(\ph)[\Pi]:=\int_\Xi \ph(z) d[\Pi](z).\] 
\end{definition}


\begin{definition}
 \label{tolerance}
 Let $\Pi$ be a point process on a Riemannian manifold $\Xi$ with volume measure $\mu$. Let $\D \subset \Xi$ be a bounded open set, and let $\La(\Phi_0),\La(\Phi_1),\cdots,\La(\Phi_t)$ be rigid linear statistics of the point process $\Pi_\inn$ on $\D$, with $\Phi_0 \equiv 1$ and $\Phi_1,\cdots,\Phi_t:\D \rightarrow \C$ smooth functions. 
 
 For an integer $m \ge 0$  and $\us:=(s_1,\cdots,s_t) \subset \C^t$, consider the submanifold of $\D^m$ \[\Sigma_{m,\us}:=\{ \uz=(\zeta_1,\cdots,\zeta_m) \in \D^m : \La(\Phi_j)[\delta_{\uz}]=s_j; 1 \le j \le t  \},\] where $\delta_{\uz}$ is the counting measure corresponding to the point set $\{\zeta_i\}_{i=1}^m$.
 
 Then $\Pi$ is said to be tolerant subject to  $\La(\Phi_0),\La(\Phi_1),\cdots,\La(\Phi_t)$ if the conditional distribution $\l(\Pi_\inn | \Pi_\out=\o \r)$ is mutually absolutely continuous with the point process of $\La(\Phi_0)[\Pi_\inn]=N(\o)$ points sampled independently from the submanifold $\Sigma_{N(\o),\us}$ (where $s_i=\La(\Phi_i)[\Pi_\inn]=S_i(\o), 1\le i \le t$) equipped with the restriction of the volume measure $\mu^{\otimes N(\o)}$.
\end{definition}

\begin{remark}
 One can generalise the above notion of tolerance by demanding constraints on more general functionals than linear statistics. For example, for a fixed positive integer $k$, one can consider a smooth function $\Psi:\D^k \to \C$ and demand that the functional $\La^{(k)}(\Psi):=\int \int \Psi d[\Pi_\inn]^{\otimes k}$ is rigid.  
\end{remark}

Theorems \ref{gin-2} and \ref{gaf-2} can be phrased in terms tolerance as defined above. E.g., Theorem \ref{gin-2} can be rephrased by saying that for any bounded open set $\D$, the Ginibre ensemble  is tolerant subject to the number of points in $\D$.

In view of these results, it is natural to ask whether there are point processes which exhibit higher levels of rigidity, in the sense that higher moments of the points inside $\D$ are also conserved. In a technical sense, we can formulate this question as follows.
 
\begin{definition}
 \label{hie}
 We say that a point process $\Pi$ on $\C$ is rigid at level $k$ if the following conditions hold for every bounded open set $\D \subset \C$:
 \begin{itemize}
  \item The linear statistics of $\Pi_\inn$ given by $\{\La(z^{j})\}_{j=0}^{k-1}$ are rigid.
  \item $\Pi$ is tolerant subject to $\{\La(z^{j})\}_{j=0}^{k-1}$.
 \end{itemize}
\end{definition}

In terms of the last definition, we can say that the Ginibre ensemble is rigid at level 1 and the standard planar GAF zero process is rigid at level 2.
 
Of course, we would like to consider ``natural'' models of point processes exhibiting higher levels of rigidity. As in, the models should not be toy examples engineered to precisely conform to such notions of rigid behaviour. One potential source of such toy models could be lattice perturbations, with the perturbations constrained so as to obtain rigidity at the desired level. However, even to obtain ``toy'' examples seems to be rather difficult, and we are not aware of any such models.
 
 In this paper, we answer the above question by introducing a family of point processes, indexed by a parameter $\a>0$, such that for different values of $\a$  there is a different rigidity behaviour. These are also Gaussian analytic functions, albeit with different scaling behaviour of the coefficients from the standard one. In fact, we show that there is a monotonicity in the rigid behaviour with respect to the parameter $\a$: for $\frac{1}{k} < \a \le \frac{1}{k-1}$ (where $k \ge 0$ is an integer), the resulting point process is rigid at level $k$. For the special case $\a=1/2$, we recover the standard planar GAF. We call this family of Gaussian analytic functions as $\a$-GAF, which we formally define as follows:
 
 \begin{definition}
  For a real number $\a>0$, we define the $\a$-GAF \[f_\a(z)=\sum_{k=0}^\infty \frac{\xi_k}{(k!)^{\a/2}}z^k.\]
 \end{definition}

 This enables us to state
 \begin{theorem}
  \label{hierig}
  The $\a$-GAF zero process is rigid at level $k \ge 1$ whenever $\a \in (\frac{1}{k} , \frac{1}{k-1}]$. 
 \end{theorem}

%  It is natural to ask whether one can study continuum percolation on the $\a$-GAF zero processes on similar lines to \cite{GKP}. Letus mention prove existence of a (non-trivial) critical radius for continuum percolation on the $\a$-GAF zero process, and whether it is possible to establish uniqueness of the infinite cluster in the supercritical regime 
 
 Another natural question which arises with regard to rigidity phenomena is the following. In a determinantal point process (henceforth abbreviated as d.p.p.) with a kernel $K$ and a background measure $\mu$, all information about the process is contained, in principle, in the pair $(K,\mu)$. So, it is natural to ask whether it is possible to read off information about the rigidity behaviour of determinantal processes by looking at their kernel. We provide a partial answer to this question by specifying conditions on the pair $(K,\mu)$ which mandate a certain rigidity behaviour of the determinantal process.
 
 To state this result, recall that the necessary and sufficient condition (due to Machchi and Soshnikov) for the pair $(K,\mu)$ to be the kernel and background measure of a determinantal point process is that $K$ gives rise to a non-negative contraction when looked upon in the natural way as the kernel of an integral operator acting on $L^2(\mu)$. Then we have the following connection between rigidity and the kernel:
 
 \begin{theorem}
  \label{detrig}
  Let $\Pi$ be a determinantal point process with kernel $K$ and background measure $\mu$. Then $\Pi$ exhibits rigidity in the number of points in a domain only if $K$ is a projection operator on $L^2(\mu)$.
 \end{theorem}

 It is an interesting question to ask whether converse of Theorem \ref{detrig} is true. In other words, if the kernel $K$ yields a projection operator on $L^2(\mu)$, then is the resulting determinantal process rigid (in terms of the number of points in a domain). However, such a statement is not true in complete generality. A counter-example is provided by the zeroes of the hyperbolic Gaussian analytic function of intensity 1. It is a determinantal point process whose kernel is the projection on to the Bargmann spacee of $L^2$ analytic functions on the unit disk. It has been shown to be insertion and deletion tolerant in \cite{HS}; in particular, it does not exhibit rigidity of the number of points in any domain. However, this is an example where the ambient space (the hyperbolic plane) is non-Euclidean, in particular it is non-amenable. This still leaves open the question of whether a determinantal point process on a Euclidean space given by a projection kernel is necessarily rigid (in terms of the number of points), or more generally, what can be said about the rigidity  properties of such point processes. 
 
 In Section \ref{radialmeasures}, we consider determinantal point processes on $\C$ with a sesqui-holomorphic kernel $K(z,w)$ (that is holomorphic in $z$ and conjugate-holomorphic in $w$).  Further, we will assume that $\gamma$ is a radial measure with $\mu$ being the measure on the non-negative real line induced by $|Z|^2$ (where $Z  \sim \gamma$), that $\mu$ has all moments finite, and let \[c_j^{-1}= \int_0^\infty r^j d\mu(r).\] We will focus on the case where the kernel has the structure \[K(z,w)=\sum_{j=0}^{\infty} c_j z^j\ol{w}^j .\] The last identity implies that $K$ is a reproducing kernel, projecting on to the subspace of $L^2(\gamma)$ gererated by the polynomials.   

 This is an interesting family of d.p.p.-s (parametrized by the measure $\gamma$), encompassing the zeroes of the hyperbolic GAF with unit intensity on one hand (where $\gamma$ is the uniform measure on the unit disk), and the Ginibre ensemble on the the other (where $\gamma$ equals the standard Gaussian measure on the complex plane). It is known that the rigidity properties of these two ensembles are very different - while the hyperbolic GAF is tolerant to insertion and deletion of points (\cite{HS}), the Ginibre ensemble exhibits rigidity at level 1. 
 
 We investiage this family of d.p.p.-s with respect to rigidity behavious. Interestingly, a rough dichotomy emerges - when $\gamma$ is compactly supported (along with some additional conditions), the d.p.p. does not exhibit rigidity, whereas, when $\gamma$ belongs to a fairly wide class of measures that have unbounded support (that includes the Gaussian and related measures), the d.p.p. is rigid at level 1. Technically, these conditions on the measures can be articulated in terms of the various moments of $\mu$.
 
 Before stating the theorems, we introduce some further notations. Let $\Gamma_j$ be the size biasing of $\mu$ of the order $j$; in other words, $\Gamma_j$ has a density which is proportional to $r^jd\mu(r)$. Let \[\mu_j:=\E[\Gamma_j]=c_j/c_{j+1},\] \[\sigma_j:=\E\l[\l(\frac{\Gamma_j}{\mu_j}-1\r)^2\r]=\l(\frac{\mu_{j+1}}{\mu_j}-1\r)\] and  \[\nu_j := \E\l[  \l(\frac{\Gamma_j}{\mu_j}-1\r)^4\r]= \l( \frac{\mu_{j+3}\mu_{j+2}\mu_{j+1}}{\mu_j} - 4 \frac{\mu_{j+2} \mu_{j+1}}{\mu_j^2} + 6 \frac{\mu_{j+1}}{\mu_j} -3 \r).\]
 
 In the setting described above, we can state the following theorems:
 \begin{theorem}
 \label{compact}
Suppose that $\sum_{j=1}^{\infty}\sigma_j < \infty$. Then the process $\mathbb{X}$ does not exhibit rigidity of numbers.
\end{theorem}
 
 and 
 
 \begin{theorem}
 \label{dpprt}
Let the measure $\mu$ be such that it satisfies the following growth conditions:
\begin{itemize}
 \item $\sum_{j=1}^{\infty}\nu_j<\infty. $
 \item $\sum_{j=1}^{k} \mu_j^4 \nu_j= o(\mu_k^4).  $
\end{itemize}
Then the determinantal point process $\mathbb{X}$ is rigid with respect to the number of points in a bounded domain. 
If, in addition, we have the measure $\gamma$ absolutely continuous w.r.t. the Lebesgue measure on $\C$, and that for some integer $a \ge 1$ 
\begin{itemize}
 \item $\sum_{j=1}^{\infty}\mu_j^{-a}<\infty$, 
\end{itemize}
then the point process  $\mathbb{X}$ is in fact rigid at level 1.
\end{theorem}

\begin{remark}
 The assumption of absolute continuity on the measure $\gamma$ is somewhat superfluous, and is there purely to invoke the definition of tolerance, which rules out arbitrary measures. However, for rigidity at level 1, one can adopt a slightly wider notion of tolerance, by demanding that the point process inside a bounded open $\D$ is mutually absolutely continuous with respect to the point process of $N(\D)$ intependent points sampled from $d\gamma^{\otimes N(\D)}$. The proof of tolerance shows that this more general notion of tolerance is also valid in the case at hand. 
\end{remark}


A key class of measures $\mu$ which satisfies the conditions in Theorem \ref{compact} is the one where we have the following asymptotic expansion for $m_j$:
\[ \mu_j=A+\frac{B}{j} + O(1/j^2) .\]
Included in this class of measures are all measures $\mu$ such that $\mu$ is compactly supported and has a positive density in a neighbourhood of the maximal end of its support, which incorporates the important case of uniform measures on disks.

An important class of measures which satisfies the criteria in Theorem \ref{dpprt} are those which exhibit the following asymptotics, for some constants $C,A,\a$: \[\mu_j:=\E[\Gamma_j]=Cj^\a\l(1+\frac{A}{j} + O(\frac{1}{j^2})\r).\]
In other words, we stipulate a power law for the means of the size biased measures $\Gamma_j$. This covers the case of all measures of the form $d\mu(r)=r^\beta e^{-r^\gamma}dr$, which includes the Ginibre ensemble. 

While Theorems \ref{compact} and \ref{dpprt} encompass the known and important examples of relevant d.p.p.-s, it would be definitely very interesting to sharpen the dichotomy presentes in these two theorems. In particular, would it be possible to extend this dichotomy and establish that it is indeed the compactness or the non-compactness of the measure $\gamma$ that determines the rigidity behaviour of the d.p.p.

An interesting point process on $\R$ for which rigidity phenomena has been considered is the case of the sine kernel process. Indeed, it has been shown in \cite{G-I} that this point process has rigidity of the number points. It turns out that this is the only rigid statistic for the sine process, in other words, the sine process is rigid of order 1. The proof of tolerance, subject to the constraint on the number of points, is on similar lines to the proof of tolerance for the Ginibre ensemble in \cite{GP} and the proof of tolerance in Theorem \ref{dpprt}. Accordingly, we will address the proof in the supplementary note \cite{}. For now, we simply record the fact as:
\begin{theorem}
 \label{sintol}
 The sine kernel process on $\R$ is rigid at level 1.
\end{theorem}


Finally, in Section \ref{lattice}, we consider the  point process obtained by Gaussian perturbations of $\Z$. For an i.i.d. perturbation of $\Z$, it can be shown that the resulting point process is rigid at level 1; for this the perturbing variable does not need to be Gaussian, finite variance is enough. This is similar to the situation for i.i.d. lattice perturbations of $\Z^2$. On the other hand, for i.i.d. perturbations in dimensions $d \ge 3$, it is known (\cite{PS}) that there is a phase transition in the variance of the perturbing Gaussian: there is a critical $\sigma_c$ such that for variance bigger than $\sigma_c^2$, the process is insertion tolerant (to be defined below), while for variance less than $\sigma_c^2$ it is rigid (at level 1). We call a point process $\X$ on a Euclidean space insertion tolerant, if, given any bounded domain $D$ and the point configuration  $ \X$ we can introduce a new point in $D$ and still remain in the support of $\X$.  In particular, this implies that there is no rigidity of numbers in $\X$.

In dimension 1, when the tails of the Gaussians become progressively heavier, the rigidity phenomena presents an interesting study. If we posit a power law growth for the variances of the perturbations, we obtain a phase transition in the rigidity behaviour of Gaussian perturbations of $\Z$ as follows:

\begin{theorem}
 \label{power}
 Consider the point process $\X$ on $\R$ which is the random point set given by $\{k+Z_k: k \in \Z, Z_k \text{ independent } N(0,\sigma_\beta(k)) \}$, where $\sigma_\beta(k) = |k|^\beta$. Then $\X$ is insertion tolerant if $\beta>1/2$, and is rigid (at level 1) if $\beta \le 1/2$.
\end{theorem}




==> nonprojectiondpp_1.tex <==
\section{Proof of Theorem~\ref{detrig}: Non-projection determinantal processes are tolerant}
We sketch the basic idea. Consider a  kernel of the form $K(x,y)=\sum_{j\ge 1}\la_{j}\ph_{j}(x)\bar{\ph}_{j}(y)$ where $0\le \la_{j}\le 1$ and $\ph_{j}$ are orthonormal in $L^{2}(\mu)$. Let $I_{j}$ be independent Bernoulli random variables with $\P\{I_{j}=1\}=\la_{j}$, and define $K_{I}(x,y)=\sum_{j\ge 1}I_{j}\ph_{j}(x)\bar{\ph}_{j}(y)$. If we sample $I_{j}$s first and then a determinantal point process with kernel $K_{I}$, the resulting process is precisely the determinantal point process with kernel $K$ (see Thereom~4.5.3 in \cite{HKPV}). In particular, if $0<\la_{j}<1$ for at least one $j$, then the  number of points in the point process is a non-constant random variable.

In general, $K$ (rather, its associated operator $\mathcal K$) may have a continuous spectrum and hence we cannot write an expansion as above. However, we can write the kernel $K$ as a convex combination of two projection kernels and extend the above idea to show that the determinantal process with kernel $K$ is a mixture of two determinantal processes. From this, we can deduce that the given determinantal process does not have rigidity of numbers. The essential observation is that the proof of Theorem~4.5.3 in \cite{HKPV} referred to above, does not require $\ph_{j}$s to be orthogonal.

%We fix a  Radon measure $\mu$ on $\Xi$ and express all joint intensities with respect to $\mu$. Suppose $L-K=\la\phi\phi^{*}$ where $K,L$ are hermitian, locally trace-class, sub-projection kernels and $\phi$ is a unit vector in $L^{2}(\mu)$. Assume that $\Pi_{K}$ 

%
%Even if we do not assume that $\phi$ is orthogonal to $K$, under some conditions we can construct DPP($L$) as a mixture of the determinantal point processes DPP($K$) and DPP($K+\phi \phi^{*}$).


\begin{proof}[Proof of Theorem \ref{detrig}]
Let $K$ be a locally trace-class, Hermitian, contraction kernel on $L^{2}(\Xi,\mu)$ which is not a projection. Then, the corresponding integral operator  $\mathcal K=\int_{0}^{1}\la dE(\la)$ where the projection-valued measure $E$ has the property that $E[\del,1-1\del]\not=0$ for some $\del>0$. 

Let $f$ be in the range of $E[\del,1-\del]$ with $\|f\|^{2}=\del$ (norms in $L^{2}(\mu)$). Let 
\begin{align*}
L_{0}(x,y)=K(x,y)-\half f(x)\bar{f}(y)\;\;\;\mb{ and } \;\;\; L_{1}(x,y)=K(x,y)+ \half f(x)\bar{f}(y).
\end{align*} 
Let $\mathcal L_{0}$ and $\mathcal L_{1}$ be the associated operators.

Since $\mathcal K$ is locally of trace-class and Hermitian and $f\in L^{2}(\mu)$, it follows that $\mathcal L_{0}$ and $\mathcal L_{1}$ are also locally of trace-class and Hermitian. Further, by the choice of $f$, it follows that they are contraction kernels on $L^{2}(E,\mu)$, i.e., $0\le \mathcal L_{0}\le I$ and $0\le \mathcal L_{1}\le I$. To see this, let $P_{\del}$ denote the spectral projection $E[\del,1-\del]$ and let $f\otimes f^{*}$ denote the operator on $L^{2}(\mu)$ that maps $\psi$ to $\langle \psi,f \rangle f$. Then $f\otimes f^{*}\le \del P_{\del}$ (in the positive definite order) and $\del P_{\del}\le \mathcal K\le (1-\del)P_{\del}$. Therefore, 
\begin{align*}
\mathcal L_{0}=(K-\frac12 f\otimes f^{*})\ge\frac12 \del P_{\del}, \\
 \mathcal L_{1}=(K+\frac12 f\otimes f^{*})\le (1-\frac12 \del)P_{\del}.
\end{align*}
This shows that $\mathcal L_{0}$ and $\mathcal L_{1}$ are positive contractions and hence, by the theorem of Macchi and Soshnikov (see the discussion preceding the statement of Theorem~\ref{detrig}), there exist determinantal processes $\Pi_{0}$ and $\Pi_{1}$ with kernels $L_{0}$ and $L_{1}$, respectively.

By a result of Lyons (see Theorem~6.2 of \cite{Ly} for the case when $\Xi$ is a countable set), we may construct $\Pi_{0}$ and $\Pi_{1}$ on the same probability space such that every point of  $\Pi_{0}$ is also a point of $\Pi_{1}$. As $\mathcal L_{1}-\mathcal L_{0}=f\otimes f^{*}$ has rank one, there is at most one point in $\Pi_{1}$ that is not in $\Pi_{0}$. along with a  Bernoulli$(1/2)$ random variable $\xi$ that is independent of $\Pi_{0}$ and $\Pi_{1}$. Define
\[
\Pi=\begin{cases}
\Pi_{0} &\mb{ if }\xi=0, \\ \Pi_{1} &\mb{ if }\xi=1.
\end{cases}
\]
We claim that $\Pi$ is a determinantal point process with kernel $K$. To show this, fix $k\ge 1$ and $x_{1},\ldots ,x_{k}\in E$ and let  $M=\l(L_{0}(x_{i},x_{j})\r)_{i,j\le k}$ and $\uu^{t}=(f(x_{1}),\ldots ,f(x_{k}))$. Then, $\l(L_{1}(x_{i},x_{j})\r)_{i,j\le k}=M+\uu \uu^{*}$. Hence, $\Pi$ has $k$-point intensity given by
\begin{align*}
p_{k}(x_{1},\ldots ,x_{k}) &= \half \det\l( L_{1}(x_{i},x_{j})\r)_{i,j\le k} + \half \det\l( L_{0}(x_{i},x_{j})\r)_{i,j\le k} \\
&= \frac12 \det(M+\uu \uu^{*})+\frac12 \det(M) \\
&= \half \det(M)\l(1+ \uu^{*} M^{-1} \uu \r) + \half \det(M)\\
&=  \det(M)\l(1+\half \uu^{*} M^{-1} \uu \r) \\
&= \det\l(M+\half \uu \uu^{*}\r)
\end{align*}
which is precisely  $\det(K(x_{i},x_{j}))_{i,j\le k}$. This proves the claim.

Now, there exists a pre-compact set $D$ such that $\P\{\Pi_{1}\setminus \Pi_{0} \subseteq D\}>0$. On this event, $\Pi_{0}, \Pi_{1},\Pi$, all agree on $D^{c}$ but inside $D$, $\Pi_{1}$ has one point more than $\Pi_{0}$. Condition on the configuration $\Pi_{D^{c}}$. Depending on the value of $\xi$, the number of points of $\Pi$ inside $D$ can take two different values, each with positive probability (for a positive probability of configurations outside $D$).  This proves that $\Pi$ cannot have rigidity of numbers.
\end{proof}
%
%Indeed, if $P_\del$ denotes the the spectral projection $E[\del,1-\del]$ and $P_{\del'}$ the projection on to its orthogonal complement, then  for any $\psi \in L^2(\mu)$ we have \[ \langle \psi, L_0 \psi \rangle = \langle P_{\del'} \psi, K P_{\del'} \psi   \rangle + \langle P_{\del} \psi, \l(K - \frac{1}{2}ff^{*}\r) P_\del \psi \rangle.   \] By construction, $P_\del \l(K - \frac{1}{2}ff^{*}\r) P_\del \ge 0$ as an operator, since $f$ is in the range of $P_\del$ with norm $\del$, and $P_\del K P_\del \ge \del \text{Id}$. Hence the right hand side of the above display is non-negative, thereby proving that $L_0 \ge 0$ as an operator. Similarly, it can be seen that $L_1 \ge 0$.

%Let $\mathcal X_{0}$ and $\mathcal X_{1}$ be determinantal processes with kernels $L_{0}$ and $L_{1}$, respectively, coupled so that $\mathcal X_{0}\subseteq \mathcal X_{1}$. Let $\xi\sim \textbf{Ber}(1/2)$ be independent of $\mathcal X_{0}$ and $\mathcal X_{1}$. Then, define
%$$
%\mathcal X = \begin{cases} \mathcal X_{0} & \textbf{ if }\xi=0, \\ \mathcal X_{1} & \textbf{ if } \xi=1.\end{cases}
%$$
%We claim that $\mathcal X$ is determinantal with kernel $K$. To show this, fix $k\ge 1$ and $x_{1},\ldots x_{k}\in E$ and let  $M=\l(L_{0}(x_{i},x_{j})\r)_{i,j\le k}$ and $\u^{t}=(f(x_{1}),\ldots ,f(x_{k}))$. Then, $\mathcal X$ has $k$-point intensity given by
%\begin{align*}
%p_{k}(x_{1},\ldots ,x_{k}) &= \half \det\l( L_{1}(x_{i},x_{j})\r)_{i,j\le k} + \half \det\l( L_{0}(x_{i},x_{j})\r)_{i,j\le k} \\
%&= \half \det(M)\l(1+ \u^{*} M^{-1} \u \r) + \half \det(M)\\
%&=  \det(M)\l(1+\half \u^{*} M^{-1} \u \r) \\
%&= \det\l(M+\half \u \u^{*}\r)
%\end{align*}
%which is precisely  $\det(K(x_{i},x_{j}))_{i,j\le k}$. This proves the claim.

%Now, there exists a compact set $A$ such that $\P\{\mathcal X_{1} \setminus \mathcal X_{0} \subseteq A\}>0$. On this event, $\mathcal X_{0}, \mathcal X_{1},\mathcal X$, all agree on $A^{c}$ but the second one has one more point than the first inside $A$. Condition on the configuration $\mathcal X|_{A^{c}}$. Depending on the value of $\xi$, the number of points of $\mathcal X$ inside $A$ can take two different values, each with positive probability (for a positive probability of configurations outside $A$). 

%

